A New Approach to Post-Quantum Non-Malleability

We provide the first $\mathit{constant}$-$\mathit{round}$ construction of post-quantum non-malleable commitments under the minimal assumption that $\mathit{post}$-$\mathit{quantum}$ $\mathit{one}$-$\mathit{way}$ $\mathit{functions}$ exist. We achieve the standard notion of non-malleability with respect to commitments. Prior constructions required $\Omega(\log^*\lambda)$ rounds under the same assumption. We achieve our results through a new technique for constant-round non-malleable commitments which is easier to use in the post-quantum setting. The technique also yields an almost elementary proof of security for constant-round non-malleable commitments in the classical setting, which may be of independent interest. When combined with existing work, our results yield the first constant-round quantum-secure multiparty computation for both classical and quantum functionalities $\mathit{in}$ $\mathit{the}$ $\mathit{plain}$ $\mathit{model}$, under the $\mathit{polynomial}$ hardness of quantum fully-homomorphic encryption and quantum learning with errors.

==> sections/STOC-comments.tex <==
%!TEX root = ../main.tex
\section{STOC'23 Comments}
\label{sec:STOC-comments}

In this section, we have included the original comments verbatim from STOC'23 for reference, with only typographical edits made for readability in LaTeX. At the end of each review, we include our response in {\color{Plum} purple} text.


\subsection{Review A}

\para{Paper Summary.}
The research aims to construct a constant-round post-quantum commitment scheme under the assumption of a quantum one-way function. The approach that is taken is to construct a Small-Tag, One-Sided, Synchronous commitment scheme and prove that it is non-malleable using quantum-friendly techniques. Then, using the existing techniques, one can remove the one-sided restriction to achieve post-quantum secure Small-Tag, Synchronous commitment scheme. Later, the authors construct a post-quantum secure Small-Tag, Asynchronous commitment scheme. And finally, they apply an existing compiler to construct full-fledged post-quantum non-malleable commitment. Lastly, they use their result to construct constant-round post-quantum multiparty computation. The paper is well-written with good explanation of difficulties and their corresponding solutions.

The summary of Small-Tag, One-Sided, Synchronous commitment construction is as follows:
\begin{enumerate}
	\item 
	The receiver sends a random bitstring $\beta$ to the committer
\item
The committer commits to his message using $\beta$ and Naor's commitment
\item
The receiver sends the image of some random inputs to a one-way function: call them $y_i$s
\item
The receiver invokes a witness-indistinguishable proof of knowledge (WIPoK1) to show he knows at least a pre-image for one of $y_i$
\item
The committer invokes a WIPoK2 to show that either he knows an opening to the commitment value in the step 2 or he knows a pre-image for one of $y_i$
\end{enumerate}
If all the verifications hold, the committer opens the commitment later.

\para{Comments for Author:} I have a concern regarding the Small-Tag, One-Sided, Synchronous commitment construction. A comment: since the adversary in the middle is computationally restricted, maybe argument of knowledge is enough instead of proof of knowledge in the protocol.

\subpara{Concern:} The (high-level) concern regarding the non-malleability proof (of construction above) is the fact that author(s) do not use zero-knowledge proof of knowledge instead of WIPoK2. I am not totally convinced the proof will go through with a WIPoK2 protocol. My high-level argument is that the adversary in the middle may learn about the actual committed message in the step 5. Note that the witness-indistinguishability of WIPoK2 may not help because the adversary is aware of the fact that the PPT committer does not know a pre-image of the one-way function. Therefore, the committer should prove that he knows the opening for the commitment value in the step 2. Now since you use Naor's commitment, only with a negligible probability, there exists another witness (opening). (When there is only one witness, a protocol that sends the witness itself is witness indistinguishable and not zero-knowledge of course.) In other words, I do not see how witness indistinguishability prevents the adversary from learning about the message and randomness. Below, I give a detailed strategy for the adversary:
\begin{itemize}
	\item Strategy: The adversary in the middle honestly forwards the value $\beta$. After receiving the commitment $C=(c_, \ldots, c_n)$ in the step 2, if $\beta_i$ (the $i$-th bit of $\beta$) is 0, it forwards $c_i$ to the receiver, otherwise, if $\beta_i$ is 1, it forwards $c_i \xor 1$ to the receiver. Looking at the definition of Naor's commitment, assuming that the committer commits to a bit $b$ in the step 2 using a randomness $r$, the adversary changes it to a commitment to the value $1-b$ using the same randomness $r$. Now in the step 5, the adversary receives a proof of knowledge of $(b,r)$ from the committer. I am not quite sure the witness indistinguishability prevents the adversary to construct a valid proof for $(\bar{b}, r)$ to send to the receiver. One may argue that with proof of knowledge property of WIPoK2 (right), we can extract $\bar{b}$ (and therefore $b$) and this contradicts the hiding property of the commitment scheme. However, this might be a false argument since the leakage is happening in the protocol WIPoK2 (left) and not in the commitment scheme.
\end{itemize}

\subpara{Some comments:}  Better to explain more the definition of post-quantum non-malleable commitment (Definition 7). It is not clear if the adversary's output is restricted to be classical or the adversary is allowed to output a quantum state at the end. (If quantum outputs are allowed, how indistinguishability is defined over two quantum ensembles.) Typo in page 35, Machine $G_i'$: perhaps prime is missing in the description.

{\color{Plum}
\para{Our Response:} The situation the reviewer is concerned about is exactly what we describe in the last paragraph on \Cpageref{para:rebutal} that starts with ``To implement this idea, ....''

In short, our solution for this issue is to prove a statement that has two independent witnesses; WI implies WH (Witness Hiding) in such settings. Furthermore, if one of these witnesses can be extracted from an earlier part of the protocol, it can be used in a hybrid argument to get rid of the other witness (which ensures that it cannot be leaked by the WIPOK). We do exactly this in hybrid game $\mcal{G}_i$ shown in \Cref{figure:one-sided:tech-overview:Gi}. In $\mcal{G}_i$, we extract some $x_j$ from the left WIPoK1, and use the extracted $x_j$ as the ``trapdoor'' witness to finish the left WIPoK2, thus eliminating the need for witness $(m,r)$. This ensures that the left WIPoK2 is independent of $(m,r)$ and therefore it cannot leak $(m,r)$ to $M$. 


\para{In more detail:} Our eventual goal is to prove non-malleability in the real man-in-the-middle (MIM) execution. We choose to reduce it to the hiding property of the left Naor's commitment. But to construct such a reduction, we first need to make sure that the left WIPoK2 is independent of the left Naor's commitment, i.e., in the left WIPoK2, we cannot use the committed value and randomness anymore because in the reduction we are about to build, the left Naor's commitment will come from an {\bf external} challenger. This is the issue the reviewer refers to in 
%``learn about the committed value and its corresponding randomness used in c from WIPoK2-left.'' 
``the leakage is happening in the protocol WIPoK2 (left) and not in the commitment scheme.''

We address this issue by ensuring that the left WIPOK2 does not depend on the left Naor's commitment as follows. We define a hybrid game $\mcal{G}_i$ where the left WIPoK2 is executed using the extracted $x_j$. We then prove the main technical lemma \Cref{lem:tech-overview:main}, which very roughly says:
\begin{itemize}
\item
In $\mcal{G}_i$, the value extracted from the right WIPoK2 is indeed $\tilde{m}$.
\end{itemize}
The proof of this \Cref{lem:tech-overview:main} is where the main technical difficulty lies and where our {\em distributional pigeon-hole argument} applies.

With this lemma, we manage to finish the reduction from non-malleability to the left Naor's hiding by embedding the (Naor-hiding) challenger's commitment in the first two messages of game $\mcal{G}_i$ and checking the value $w'$ extracted from the right WIPoK2. This is done on \Cpageref{para:rebuttal-3} in the part starts with ``{\bf Completing the Proof of Non-Malleability}''. Importantly, this reduction makes use of $\mcal{G}_i$ (instead of the real MIM execution), for which the issue that concerns the reviewer does not appear. In particular, the attacking strategy suggested by the reviewer can be ruled out as follows. In $\mcal{G}_i$, simply run the knowledge extractor for the right WIPoK2. \Cref{lem:tech-overview:main} ensures that the extracted value is the right-side committed message $\tilde{m}$, which is the $(\bar{b}, r)$ as in the reviewer's example. Therefore, if the $\bar{b}$ is related to the $b$ in the reviewer's example, then it necessarily breaks the hiding property of Naor's commitment.
}


\subsection{Review B}
\para{Paper Summary:} This work constructs constant round post-quantum non-malleable commitments from polynomial hardness of post-quantum one-way functions. Prior to this work, constant round protocol required super-polynomial hardness and only $\omega(1)$ round protocol was known from polynomial hardness. Additionally, plugging the construction in a known compiler results in the first constant round secure multi-party computation protocol from only polynomial hardness of quantum FHE and quantum LWE.

The construction follows the general template of first building a weaker form of non-malleable commitment and then bootstrapping it to full fledged non-malleability. The main technical ideas are in building a polynomial-sized family of commitment schemes that is one-sided non-malleable w.r.t.\ synchronous man-in-the-middle adversaries. Then, this this weaker form of non-malleable is bootstrapped to an exponential-sized family of commitment schemes that is two-sided non-malleable w.r.t.\ asynchronous man-in-the-middle adversaries using known ideas.

The challenge in non-malleability is to extract the value MIM adversary is committing in the right interaction. To be able to reduce non-malleability to underlying hardness assumptions, it is important that the extraction happens in a way that doesn't disturb the security of the left interaction (referred to as robustness in the paper). Such an extraction in the classical setting is done via rewinding the adversary but is much more nuanced in the quantum setting due to the no-cloning theorem. The one-sided non-malleable commitment is carefully designed to create imbalance among the left and right interactions such that it is possible to rewind even a quantum adversary. At a high level, to achieve this the authors leverage the imbalance among the two interactions and then by relying on pigeon-hole principle are able to build an adversary which can be rewound and extracted from without distributing the hiding of the left interaction. Implementing this intuition requires a lot of care.


\subpara{Strengths:} the paper introduces new technical ideas to deal with extraction from quantum adversaries, the ideas behind the one-sided protocol are beautiful and likely to find more applications. The paper is very well written and I especially appreciated authors' effort to make the introduction readable to a wider audience while also proving insights into the challenges in proving non-malleability (1.1 is excellent).

\subpara{Audience:} The construction of one-sided commitment might appeal to a wider audience but, as with other papers in the area, the rest of the paper might only be for experts.

{\color{Plum}
\para{Our Response:} Regarding suitability, we would like to mention that STOC and FOCS have been an important venue for advancing the research on non-malleable commitments. Indeed, the introduction of the problem \cite{STOC:DolDwoNao91} and subsequent efforts in obtaining optimized constructions in various aspects (e.g., \cite{FOCS:Barak02,STOC:PasRos05,STOC:LinPas09,FOCS:Wee10,STOC:Goyal11,STOC:LinPas11,FOCS:GLOV12,FOCS:GRRV14,STOC:GoyPanRic16,FOCS:LinPasSon17,FOCS:KhuSah17,FOCS:GoyRic19}) have led to valuable contributions to theoretical cryptography which have been welcome by the STOC/FOCS audience. Also, it has been demonstrated multiple times in the literature that non-malleable commitments play a central role for efficient MPC in both stand-alone and composable settings, which is a topic of general TCS interest. Thus, we are confident that our findings are appropriate for STOC/FOCS audience.
}

\subsection{Review C}

\para{Paper Summary:} This paper constructs post-quantum non-malleable commitments from post-quantum one-way functions in constant rounds. Previous works require $\log^*(n)$ rounds.

This is achieved through the following steps:
\begin{itemize}
	\item a quantum-friendly protocol against synchronous adversaries with $\log(n)$ tags.
\item
using standard techniques to make it secure against synchronous adversaries.
\item
using a tag-amplification post-quantum compiler from previous work.
\end{itemize}
A corollary is a constant round post-quantum MPC from similar assumptions to those known but in their polynomially hard, rather than subexponentially hard, version.

\para{Comments for Author:} In terms of techniques it seems that the heart of the result is (a one-sided version of) the synchronous protocol. Here there is a very nice idea of relating the tag to the number of witnesses in a proven trapdoor statement. As far as I know (and as the writeup reflects) this idea is new. Beyond that the main enabler for these results in terms of quantum techniques is the results of CCY and LMS that gave epsilon-simulatable extraction.

Overall, I think that this is a solid result in the area of post-quantum crypto, which would definitely be accepted to crypto venues. I'm not sure that it crosses the bar for FOCS/STOC though. There's a nice idea here, but I can't say that the result is surprising or constitutes a breakthrough given CCY and LMS.

{\color{Plum}
\para{Our Response:} 
We would like to clarify the role of CCY/LMS in light of the following in Review C: ``There's a nice idea here, but I can't say that the result is surprising or constitutes a breakthrough given CCY and LMS.''

CCY/LMS only helps in improving the assumptions but they play {\em no role} in obtaining constant rounds. We emphasize that the problem of constant-round post-quantum (PQ) non-malleable commitments is challenging (and open before our work) {\em even if we relax the minimal assumption of PQ-OWFs to any standard quantum polynomial hardness assumptions}. Indeed, there seems no way to use CCY/LMS with any of the existing techniques to solve this problem despite recent attempts in published works, such as \cite{EC:ABGKM21} and \cite{BLS21}. This is because non-malleability (in particular, constant rounds) requires {\em fundamentally different} techniques than ZK (note that CCY/LMS are about improving PQ-ZK). Advances in PQ-ZK do not directly translate to reducing rounds in non-malleable protocols. Indeed, a constant-round PQ-ZK (under QLWE+QFHE) has been known for a while \cite{STOC:BitShm20} (which is before CCY/LMS), but it did not yield constant-round PQ non-malleable commitments; Emergence of CCY/LMS does not change the picture either. 

On the contrary, it is actually the techniques proposed in our work that make CCY/LMS a useful tool in this setting to get a constant round construction.




\iffalse
%Bottom line is that it is a hard problem to solve that requires a new insight. It cannot be solved by just cleverly using known techniques with a new PQ-ZK protocol such as CCY/LMS or even BS20. Our work introduces an original technique to finally obtain a constant-round PQ-NMC.

%that enables the construction of constant round PQ-NMC (under any reasonable polynomial assumption).


====

This is true even for Bitansky-Shmueli \cite{STOC:BitShm20} (which is {\em fully} ZK, as opposed to CCY which is only $\epsilon$-ZK).
We could have also plugged \cite{STOC:BitShm20} in our framework (instead of \cite{cryptoeprint:2021:1516}) to get the result under QLWE+QFHE. This would, in principle, solve the main problem of constant-round post-quantum non-malleable commitment (NMC) without relying on CCY/LMS.

\fi


% To see this clearly, recall that CCY/LMS construct a weak form of PQZK (in particular, CCY construct $\epsilon$-PQZK and LMS construct PQZK under a new type of black-box simulator), both assuming PQ-OWFs. So let's assume for simplicity that we in fact have standard PQZK. Can we then use it to get a {\em constant-round} PQ non-malleable commitments (NMC)? In other words, does constant round PQZK imply constant round PQ-NMC under similar assumptions?\fi

% Several prior works, \cite{EC:ABGKM21} and \cite{BLS21}, have attempted to answer the above question without success. This is because non-malleability (in particular, constant rounds) requires {\em fundamentally different} techniques than ZK. Advances in ZK do not directly translate to reducing rounds in non-malleable protocols. They only help with improving the assumptions. It is worth noting that a constant-round PQ-ZK (under QLWE+QFHE) has been known for a while \cite{STOC:BitShm20}, but it did not yield a constant round PQ-NMC construction. Emergence of CCY/LMS also does not change that.

% Bottom line is that it is a hard problem to solve that requires a new insight. It cannot be solved by just cleverly using known techniques with a new PQ-ZK protocol such as CCY/LMS or even BS20.


\iffalse
CCY/LMS only helps in improving the assumptions but they play {\em no role} in obtaining constant rounds. We emphasize that the problem of constant-round post-quantum non-malleable commitments was open {\em even if we relax the minimal assumption of post-quantum OWFs to any standard quantum polynomial hardness assumptions}. Indeed, there seems no way of using CCY/LMS with any of the existing techniques to solve this problem despite recent attempts in published works, such as \cite{EC:ABGKM21} and \cite{BLS21}. This is true even for Bitansky-Shmueli \cite{STOC:BitShm20} (which is {\em fully} ZK, as opposed to CCY which is only $\epsilon$-ZK).
We could have also plugged \cite{STOC:BitShm20} in our framework (instead of \cite{cryptoeprint:2021:1516}) to get the result under QLWE+QFHE. This would, in principle, solve the main problem of constant-round post-quantum non-malleable commitment (NMC) without relying on CCY/LMS. A new approach seems essential to solve this problem. But such approaches are not easy to come by. 

It took 15-20 years to find them in the classical case, and none of them work in the post-quantum case. As discussed toward the end of \Cpageref{pageref:why-quantum-friendly}, the main challenge of this problem is to design a robust simulatable extraction structure in constant rounds. Before the current submission, it was unclear how this could be done in the post-quantum setting, {\em even with the CCY/LMS lemma or \cite{STOC:BitShm20} in hand}.


\fi
}


==> sections/old-small-tag-quantum.tex <==
%!TEX root = ../main.tex
\section{Small-Tag, One-sided, Synchronous, Post-Quantum Setting}\label{sec:small-tag-one-sided-sync-pq}
In this section, we prove that \Cref{prot:one-sided:classical} is post-quantumly secure if we rely on post-quantum building-blocks. 
Similarly to the classical case in \Cref{sec:small-tag-one-sided-sync-classical}, we present the construction assuming the existence of post-quantum {\em injective} OWFs.  
The assumption can be relaxed to  {\em any} OWFs by an appropriate modification to the protocol similarly to the classical case.  
Since this is exactly the same as that in the classical setting, which is explained in \Cref{sec:removing-injectivity}, we do not repeat it in this section. 

Our construction is based on the following building blocks:
%We need the following building blocks:
\begin{itemize}
\item
A post-quantum {\em injective} OWF $f$; 
\item
Naor's commitment $\Com$ that is implemented with a post-quantum OWF.\footnote{In this way, the Naor's commitment is statistically-binding and {\em post-quantumly} computationally-hiding.};
\item
A post-quantum witness-indistinguishable argument of knowledge with $\epsilon$-close emulation $\WIAoK$ %with knowledge error $\kappa(\secpar) = \negl(\secpar)$ 
(as per \Cref{def:PQWIAoK}). 
\end{itemize}

\begin{ProtocolBox}[label={prot:one-sided:pq}]{Small-Tag One-Sided Synchronous Post-Quantum NMCom \textnormal{$\langle C, R\rangle^{\msf{OneSided}-\msf{pq}}_{\msf{tg}}$}}
The tag space is defined to be $[2n]$ where $n$ is a polynomial on $\secpar$. Let $t \in [2n]$ be the tag for the following interaction. Let $m$ be the message to be committed to. \red{Why $2n$ instead of $n$?}

\para{Commit Stage:}
\begin{enumerate}
\item\label[Step]{item:one-sided:pq:step:Naor-rho}
Receiver $R$ samples and sends the first message $\gamma$ for Naor's commitment; 
\item\label[Step]{item:one-sided:pq:step:committing}
Committer $C$ commits to $m$ using the second message of Naor's commitment. Formally, $C$ samples a random tape $r$ and sends $\msf{com} = \Com_\gamma(m;r)$;
\item\label[Step]{item:one-sided:pq:step:OWFs}
$R$ computes $\Set{y_i = f(x_i)}_{i \in [t]}$ with $x_i \pick \bits^\secpar$ for each $i \in [t]$. $R$ sends $Y = (y_1, \ldots, y_t)$ to $C$;
\item\label[Step]{item:one-sided:pq:step:WIAoK:1}
{\bf (WIAoK-1.)} $R$ and $C$ execute an instance of $\WIAoK$ where $R$ proves to $C$ that he ``knows'' a pre-image of some $y_i$ contained in $Y$ (defined in \Cref{item:one-sided:pq:step:OWFs}). Formally, $R$ proves that $Y \in \Lang^t_f$, where \begin{equation}\label[Language]{eq:one-sided:pq:Lang:OWF}
\Lang^t_f \coloneqq \Set{(y_1, \ldots, y_t)~|~\exists (i, x_i) ~s.t.~ i \in [t] \wedge y_i = f(x_i)}.
\end{equation}
Note that $R$ uses $(1,x_1)$ as the witness when executing this $\WIAoK$.
\item\label[Step]{item:one-sided:pq:step:WIAoK:2}
{\bf (WIAoK-2.)} $C$ and $R$ execute an instance of $\WIAoK$ where $C$ proves to $R$ that he ``knows'' {\em either} the message committed in $\msf{com}$ (defined in \Cref{item:one-sided:pq:step:committing}), {\em or} a pre-image of some $y_i$ contained in $Y$ (defined in \Cref{item:one-sided:pq:step:OWFs}). Formally, $C$ proves that $(\msf{com}, Y) \in \Lang_\gamma \vee \Lang^t_f$, where $\Lang_\gamma \vee \Lang^t_f$ denotes the  OR-composed language (as per \Cref{def:OR-Comp}), $\Lang^t_f$ was defined in \Cref{eq:one-sided:pq:Lang:OWF} and 
\begin{equation}\label[Language]{eq:one-sided:pq:Lang:Com}
\Lang_\gamma\coloneqq \Set{\msf{com} ~|~ \exists (m, r)~s.t.~ \msf{com} = \Com_\gamma(m;r)}.
\end{equation}
Note that $C$ uses the $(m, r)$ defined in \Cref{item:one-sided:pq:step:committing} as the witness when executing this $\WIAoK$.
\end{enumerate}
\para{Decommit Stage:} 
$C$ sends $(m, r)$. $R$ accepts if $\msf{com} = \Com_\gamma(m;r)$, and rejects otherwise.
\end{ProtocolBox}

Remark that the above protocol is exactly the same as \Cref{prot:one-sided:pq} except that we use WIAoK instead of WIPoK and and assume post-quantum security for all  building-blocks.
Completeness, post-quantum computational hiding, and statistical binding hold similarly to the classical case in \Cref{sec:small-tag-one-sided-sync-classical}. 

\if0
Formally, we prove the following theorem.
\begin{theorem}
\Cref{prot:one-sided:classical} is a one-sided non-malleable commitment
scheme secure against synchronous QPT adversaries when the building blocks satisfies the following requirements:
\begin{itemize}
\item
	Naor's commitment is implemented with a post-quantum OWF.\footnote{In this way, the Naor's commitment is statistically-binding and {\em post-quantumly} computationally-hiding.}
\item
The injective OWF $f$ is a post-quantum one-way function
\item
The WIAoK satisfies \red{give the definition and Cref to it}
\end{itemize} 
\end{theorem}
\fi 


\subsection{Proving Non-Malleability}
\label{one-sided:pq:non-malleability:proof}

\begin{theorem}\label{thm:one-sided:pq:non-malleability}
The commitment scheme $\langle C, R\rangle^{\msf{OneSided}-\msf{pq}}_{\msf{tg}}$ in \Cref{prot:one-sided:pq} is a one-sided non-malleable commitment scheme secure against synchronous QPT adversaries.
\end{theorem}	
In the rest of this section, we write $\langle C, R \rangle$ to mean $\langle C, R\rangle^{\msf{OneSided}-\msf{pq}}_{\msf{tg}}$ for notational simplicity. 

We prove \Cref{thm:one-sided:pq:non-malleability} in \Cref{one-sided:pq:non-malleability:proof,sec:one-sided:pq:core-lemma:proof,lem:small-tag:proof:se:proof:pq,sec:lem:small-tag:proof:se:proof:K:proof:pq,sec:lem:bound:Ki:proof:pq}.
The proof follows the same template used in \Cref{one-sided:non-malleability:proof:classical}.
Almost all steps in the proof of \Cref{thm:one-sided:non-malleability} are directly translated into the post-quantum setting. The only exception is the proof of \Cref{lem:small-tag:proof:se} (whose post-quantum counterpart is \Cref{lem:small-tag:proof:se:pq}) where we amplify the extractor $\mcal{K}$ to the simulation-extractor $\mcal{SE}$ by rewinding. Since we cannot rewind quantum algorithms in general, we rely on an alternative argument based on the extract-and-simulate lemma~(\Cref{lem:extract_and_simulate}).


We use the same notation as in the proof of \Cref{thm:one-sided:non-malleability}, with the only difference that now the adversaries are QPT machines (instead of PPT machines). It is worth noting that the honest committer and receiver are still classical (i.e., PPT) machines. 
%We add a short bar on top of the games/machines that is the quantum counterpart of their classical version in \Cref{sec:small-tag-one-sided-sync-classical}.

\para{Game $H^{\mcal{M}_\secpar}(\secpar,m,\rho_\secpar)$:\label{gameH:description:pq}} This game is identical to the classical counterpart defined on \Cpageref{gameH:description}, except that $\mcal{M} = \Set{\mcal{M}_\secpar, \rho_\secpar}_{\secpar\in \Naturals}$ now is a QPT machine.
That is, this is the man-in-the-middle execution of the commit stage of the $\langle C, R \rangle$ defined in \Cref{prot:one-sided:pq}, where the left committer commits to $m$ and $\mcal{M}$'s non-uniform advice is $\rho_\secpar$. 
The output of $H^{\mcal{M}_\secpar}(m,\rho_\secpar)$ is again defined to be $(\OUT_{\mcal{M}}, \tilde{\tau}, b)$, where $\OUT_{\mcal{M}}$ is the (quantum) output of $\mcal{M}_\secpar(\rho_\secpar)$ at the end of this game, $\tilde{\tau}$ consists of the \Cref{item:one-sided:pq:step:Naor-rho,item:one-sided:pq:step:committing} messages in the right session, and $b \in \Set{\top, \bot}$ is the honest receiver's decision.

\para{Notation.} 
\xiao{Provide more explanation of notation. In particular, the MIM game for QPT adversaries are denoted as $\bar{\msf{mim}}^{\mcal{M}_\secpar}_{\langle C, R \rangle}(m, \rho_\secpar)$. See \Cref{def:NMCom:pq}.}\takashi{Is the following okay?}

Recall that the man-in-the middle game for a QPT adversary $\mcal{M}$ is denoted by $\bar{\msf{mim}}^{\mcal{M}_\secpar}_{\langle C, R \rangle}(m, \rho_\secpar)$ as defined in \Cref{def:NMCom:pq}. 
Remark that ``$\cind$'' refers to {\em quantum} computational indistinguishability throughout this section.

For any $(\OUT_{\mcal{M}}, \tilde{\tau}, b)$ in the support of $H^{\mcal{M}_\secpar}(\secpar,m,z)$, we define $\msf{val}_b(\tilde{\tau})$ similarly to the classical case, i.e., 
$$
\msf{val}_b(\tilde{\tau}) \coloneqq 
\begin{cases}
\msf{val}(\tilde{\tau}) & b = \top\\
\bot & b = \bot
\end{cases},
$$
where $\msf{val}(\tilde{\tau})$ denote the value statistically-bounded in \Cref{item:one-sided:pq:step:Naor-rho,item:one-sided:pq:step:committing} of the right session.


Similarly to \Cref{eq:classical:mim-H}, we have
\begin{align}
\big\{\bar{\msf{mim}}^{\mcal{M}_\secpar}_{\langle C, R \rangle}(m, \rho_\secpar)\big\} \idind \big\{\big(\OUT, \msf{val}_b(\tilde{\tau})\big): (\OUT, \tilde{\tau}, b) \gets H^{\mcal{M}_\secpar}(m,\rho_\secpar) \big\},
\end{align}
where both ensembles are indexed by $\secpar \in \Naturals$ and $m \in \bits^{\ell(\secpar)}$.

Then, similarly to \Cref{eq:classical:H:m-0:m-1}, the post-quantum non-malleability can be reduced to establishing the following equation:
\begin{align*}
&\big\{\big(\OUT^0, \msf{val}_{b^0}(\tilde{\tau}^0)\big): (\OUT^0, \tilde{\tau}^0, b^0) \gets H^{\mcal{M}_\secpar}(m_0,\rho_\secpar) \big\} \\
\cind ~& 
\big\{\big(\OUT^1, \msf{val}_{b^1}(\tilde{\tau}^1)\big): (\OUT^1, \tilde{\tau}^1, b^1) \gets H^{\mcal{M}_\secpar}(m_1,\rho_\secpar) \big\} \numberthis \label{eq:classical:H:m-0:m-1:pq},
\end{align*}
where both ensembles are indexed by $\secpar \in \Naturals$ and $(m_0, m_1) \in \bits^{\ell(\secpar)} \times \bits^{\ell(\secpar)}$.

\para{Proof by Contradiction.} Similarly to \Cref{eq:one-sided:proof:contra-assump}, we assume for contradiction that there are a (possibly non-uniform) QPT distinguisher $\mcal{D} = \Set{\mcal{D}_\secpar, \sigma_\secpar}_{\secpar \in \Naturals}$ and a function $\delta(\secpar) = 1/\poly(\secpar)$ such that for infinitely many $\secpar \in \Naturals$, it holds that
\begin{equation}\label[Inequality]{eq:one-sided:pq:proof:contra-assump}
\bigg|\Pr[\mcal{D}_\secpar\big(\OUT^0, \msf{val}_{b^0}(\tilde{\tau}^0); \sigma_\secpar\big)=1] - \Pr[\mcal{D}_\secpar\big(\OUT^1, \msf{val}_{b^1}(\tilde{\tau}^1); \sigma_\secpar\big)=1] \bigg|\ge 3 \cdot \delta(\secpar),
\end{equation}
where the first probability is taken over the random procedure $(\OUT^0, \tilde{\tau}^0, b^0) \gets H^{\mcal{M}_\secpar}(m_0,\rho_\secpar)$, %\xiao{Should I say ``and the randomness due to the measurement performed by $\mcal{D}_\secpar$ if any''}, 
and the second probability is taken over the random procedure $(\OUT^1, \tilde{\tau}^1, b^1) \gets H^{\mcal{M}_\secpar}(m_1,\rho_\secpar)$ (and the randomness due to the measurement performed by $\mcal{D}_\secpar$ if any for both probabilities).

Then, we show the following \Cref{lem:one-sided:pq:proof:core}, which should be understood as the quantum counterpart of \Cref{lem:one-sided:proof:core}. 
\begin{lemma}\label{lem:one-sided:pq:proof:core}
For the above $\delta(\secpar)$,
there exits a hybrid $G$ such that for any QPT $\mcal{M}=\Set{\mcal{M}_\secpar, \rho_\secpar}_{\secpar\in \Naturals}$, the following holds
\begin{enumerate}
\item\label[Property]{item:lem:one-sided:pq:proof:core:1}
$\big\{(\OUT^0, \Val^0):(\OUT^0, \Val^0) \gets G^{\mcal{M}_\secpar}(\secpar,m_0,\rho_\secpar) \big\} \cind \big\{(\OUT^1, \Val^1):(\OUT^1, \Val^1) \gets G^{\mcal{M}_\secpar}(\secpar,m_1,\rho_\secpar) \big\}$,
where both ensembles are indexed by $\secpar \in \Naturals$ and $(m_0, m_1) \in \bits^{\ell(\secpar)} \times \bits^{\ell(\secpar)}$.
\item\label[Property]{item:lem:one-sided:pq:proof:core:2}
\begingroup\fontsize{9.5pt}{0}\selectfont
$\big\{(\OUT^{G}, \Val^{G}):(\OUT^{G}, \Val^{G}) \gets G^{\mcal{M}_\secpar}(\secpar,m,\rho_\secpar) \big\}
\sind_{\delta(\secpar)} 
\big\{\big(\OUT^{H}, \msf{val}_{b^{H}}(\tilde{\tau}^{H})\big): (\OUT^{H}, \tilde{\tau}^{H}, b^{H}) \gets H^{\mcal{M}_\secpar}(\secpar,m,\rho_\secpar) \big\}$,
\endgroup  
where both ensembles are indexed by $\secpar \in \Naturals$ and $m \in \bits^{\ell(\secpar)}$.
\end{enumerate}
\end{lemma}

It is easy to see that if \Cref{lem:one-sided:pq:proof:core} is true, it contradicts our assumption in \Cref{eq:one-sided:pq:proof:contra-assump}. Therefore, it will finish the proof of non-malleability. Indeed, this lemma is the most technically involved part. We prove it in \Cref{sec:one-sided:pq:core-lemma:proof}.


\subsection{Proof of \Cref{lem:one-sided:pq:proof:core}}
\label{sec:one-sided:pq:core-lemma:proof}

In \Cref{hybrid:H:reinterpretation:pq}, we provide a new but equivalent interpretation of the game $H^{\mcal{M}}(\secpar, m, \rho_\secpar)$.
\begin{AlgorithmBox}[label={hybrid:H:reinterpretation:pq}]{Re-interpretation of Game \textnormal{$H^{\mcal{M}_\secpar}(\secpar, m, \rho_\secpar)$}}
Game $H^{\mcal{M}_\secpar}(\secpar, m, \rho_\secpar)$ can be split into the following stages:
\begin{enumerate}
\item \label[Stage]{hybrid:H:reinterpretation:1:pq}
{\bf Prefix Generation:}
First, execute \Cref{item:one-sided:pq:step:Naor-rho,item:one-sided:pq:step:committing} of the man-in-the-middle game of \Cref{prot:one-sided:classical}---it plays as the honest committer in the left committing to $m$ and the honest receiver in the right session, with $\mcal{M}_\secpar(\rho_\secpar)$ being the man-in-the-middle adversary.

\subpara{Notation:} Let $\msf{st}_{\mcal{M}}$ denote the state of $\mcal{M}$ at the end of \Cref{item:one-sided:pq:step:committing}; let $\msf{st}_C$  (resp.\ $\msf{st}_R$) denote the state of the honest committer (resp.\ receiver) at the end of \Cref{item:one-sided:pq:step:committing}; let $\tilde{\tau}$ denote the tuple $(\tilde{\gamma}, \tilde{\msf{com}})$\footnote{Recall that $\tilde{\gamma}$ and  $\tilde{\msf{com}}$ are the \Cref{item:one-sided:pq:step:Naor-rho,item:one-sided:pq:step:committing} messages in the right session; they constitutes an execution of Naor's commitment.}. In terms of notation, we denote the execution of this stage by 
\begin{equation}\label[Expression]{expression:hybrid:H:prefix:pq}
(\msf{st}_{\mcal{M}},  \msf{st}_C, \msf{st}_R, \tilde{\tau})\gets H^{\mcal{M}_\secpar}_{\msf{pre}}(\secpar, m, \rho_\secpar).
\end{equation}
We will call the tuple $(\msf{st}_{\mcal{M}},  \msf{st}_C, \msf{st}_R, \tilde{\tau})$ the {\em prefix} and denote it by $\msf{pref}$. It is worth noting that this $\msf{pref}$ contains all the information such that a QPT machine can ``complete'' the remaining execution of $H^{\mcal{M}_\secpar}(\secpar, m, \rho_\secpar)$ starting from $\msf{pref}$.

\item \label[Stage]{stage:hybrid:H:remainder:pq}
{\bf The Remainder:}
Next, it simply resumes from where the {\bf Prefix Generation} stage stops, to finish the remaining steps of the man-in-the-middle execution $H^{\mcal{M}_\secpar}(\secpar, m, \rho_\secpar)$.

\subpara{Notation:} We introduce the following notations to describe this stage. Define a QPT machine $\Adv$ that takes as input $(\msf{st}_{\mcal{M}}, \tilde{\tau})$; Machine $\mcal{A}$ is supposed to run the residual strategy of $\mcal{M}_\secpar$ starting from $\msf{st}_{\mcal{M}}$. Also, define a QPT machine $\mcal{B}$ that takes as input $(\msf{st}_C, \msf{st}_R, \tilde{\tau})$; Machine $\mcal{B}$ is supposed to run the residual strategies of the honest committer $C$ and receiver $R$, starting from 
$\msf{st}_C$ and $\msf{st}_R$ respectively\footnote{Note that it is not necessary to give $\tilde{\tau}$ as common input to these parties; indeed, it can be included in their respective internal states. We choose to make $\tilde{\tau}$ explicit only to match the syntax of \Cref{lem:extract_and_simulate}.}. With the above notations, we can denote the execution of the remaining steps of $H^{\mcal{M}_\secpar}(\secpar, m,z)$ by
\begin{equation}\label[Expression]{expression:hybrid:H:remainder:pq}
(\OUT_\mcal{A}, b)\gets \langle \mcal{A}(\msf{st}_{\mcal{M}}), \mcal{B}(\msf{st}_C, \msf{st}_R) \rangle(1^\secpar, \tilde{\tau}),
\end{equation}
where $\OUT_\mcal{A}$ is the output of $\mcal{A}$, and $b \in \Set{\bot, \top}$ is the output of the honest receiver $R$ (in the right), indicating if the man-in-the-middle's commitment (i.e., the right session) is accepted ($b = \top$) or not ($b = \bot$). (We remark that $\OUT_\Adv$ is nothing but the man-in-the-middle $\mcal{M}$'s final output.)

\item
{\bf Output:} It outputs the tuple $(\OUT_\Adv, \tilde{\tau}, b)$.  
\end{enumerate}
\end{AlgorithmBox}

%\xiao{Say that this is the major lemma for this proof. }
We prove the following lemma. which is the counterpart of \Cref{lem:small-tag:proof:se}. 
\begin{lemma}\label{lem:small-tag:proof:se:pq}
Let $H^{\mcal{M}_\secpar}_{\msf{pre}}(\secpar, m, \rho_\secpar)$, $\mcal{A}$, $\mcal{B}$ be as defined in \Cref{hybrid:H:reinterpretation:pq}.
There exists a QPT machine $\mcal{SE}$ (the simulation-extractor) such that for any $(\msf{st}_{\mcal{M}},  \msf{st}_C, \msf{st}_R, \tilde{\tau})$ in the support of $H^{\mcal{M}_\secpar}_{\msf{pre}}(\secpar, m, \rho_\secpar)$, any noticeable $\epsilon(\secpar)$, it holds that
\begin{align*}
& \big\{ (\OUT_{\mcal{SE}}, \msf{Val}_{\mcal{SE}}) : (\OUT_{\mcal{SE}}, \msf{Val}_{\mcal{SE}}, b_{\mcal{SE}}) \gets \SimExt^{\A(\msf{st}_{\mcal{M}})}(1^\secpar,1^{\epsilon^{-1}},\tilde{\tau})\big\}_{\secpar\in \Naturals} \\
\sind_{\epsilon(\secpar)} ~&
\big\{\big(\OUT_\mcal{A}, \msf{val}_b(\tilde{\tau})\big) : (\OUT_\mcal{A}, b) \gets \langle \mcal{A}(\msf{st}_{\mcal{M}}), \mcal{B}(\msf{st}_C, \msf{st}_R) \rangle(1^\secpar, \tilde{\tau})\big\}_{\secpar\in \Naturals} 
\end{align*} 
\end{lemma}
\Cref{lem:small-tag:proof:se:pq} is the main technical lemma for the current proof of \Cref{lem:one-sided:pq:proof:core}. We present its proof in \Cref{lem:small-tag:proof:se:proof:pq}. In the following, we finish the proof of \Cref{lem:one-sided:pq:proof:core}  assuming that \Cref{lem:small-tag:proof:se:pq} is true.


Now, we are ready to present the description of $G$.
\begin{AlgorithmBox}[label={hybrid:G:pq}]{Hybrid \textnormal{${G}^{\mcal{M}_\secpar}(\secpar, m, \rho_\secpar)$}}
This hybrid proceeds as follows:
\begin{enumerate}
\item
{\bf Prefix Generation:}
This stage is identical to \Cref{hybrid:H:reinterpretation:1:pq} of $H^{\mcal{M}_\secpar}(\secpar, m, \rho_\secpar)$. Formally, it executes 
$$(\msf{st}_{\mcal{M}},  \msf{st}_C, \msf{st}_R, \tilde{\tau}) \gets H^{\mcal{M}_\secpar}_{\msf{pre}}(\secpar, m, \rho_\secpar),$$
where $H^{\mcal{M}_\secpar}_{\msf{pre}}(\secpar, m, \rho_\secpar)$ is defined in \Cref{hybrid:H:reinterpretation:1:pq} of \Cref{hybrid:H:reinterpretation:pq}.
\item
{\bf The Remainder:}
Define $\mcal{A}$ in the same way as in \Cref{stage:hybrid:H:remainder:pq} of $H^{\mcal{M}_\secpar}(\secpar, m, \rho_\secpar)$. With this $\mcal{A}$  and the prefix $(\msf{st}_{\mcal{M}},  \msf{st}_C, \msf{st}_R, \tilde{\tau})$ from the previous stage, ${G}^{\mcal{M}}(\secpar, m, \rho_\secpar)$ invokes the $\mcal{SE}$ prescribed in \Cref{lem:small-tag:proof:se}. Formally, it does the following:
$$(\OUT_{\mcal{SE}}, \msf{Val}_{\mcal{SE}}, b_{\mcal{SE}}) \gets \SimExt^{\A(\msf{st}_{\mcal{M}})}(1^\secpar,1^{\delta^{-1}},\tilde{\tau}),$$
where the $\delta$ is the statistical distance that we want to show for \Cref{item:lem:one-sided:pq:proof:core:2} of \Cref{lem:one-sided:pq:proof:core}.

\item
{\bf Output:}
% $G^{\mcal{M}_\secpar}(m,\gamma_\secpar)$ sets $\OUT_{G}\coloneqq \OUT_{\mcal{SE}}$ and $ \msf{Val}_{G}\coloneqq \msf{Val}_{\mcal{SE}}$, and 
It outputs $(\OUT_{\mcal{SE}}, \msf{Val}_{\mcal{SE}})$.\footnote{Note that $b_{\mcal{SE}}$ is not included in the output of $G$. Indeed, $b_{\mcal{SE}}$ is not important for the current machine $G^{\mcal{M}}(\secpar, m, \rho_\secpar)$. We choose to include it in the output of $\SimExt^{\A(\msf{st}_{\mcal{M}})}(1^\secpar,1^{\delta^{-1}},\tilde{\tau})$ only for notational convenience when we define/prove properties about $\mcal{SE}$ itself.}
\end{enumerate}
\end{AlgorithmBox}

\para{Proving \Cref{item:lem:one-sided:pq:proof:core:1} of \Cref{lem:one-sided:pq:proof:core}.} Observe that hybrid $G^{\mcal{M}}(\secpar, m, \rho_\secpar)$ is an efficient machine, since both $H^{\mcal{M}_\secpar}_{\msf{pre}}(\secpar, m, \rho_\secpar)$ and $\SimExt^{\A(\msf{st}_{\mcal{M}})}(1^\secpar,1^{\delta^{-1}},\tilde{\tau})$ are efficient. Moreover, it does not rewind \Cref{item:one-sided:pq:step:Naor-rho,item:one-sided:pq:step:committing} of the man-in-the-middle execution. Therefore, \Cref{item:lem:one-sided:pq:proof:core:1} of \Cref{lem:one-sided:proof:core} follows immediately from the computationally-hiding property of the left Naor's commitment (i.e., \Cref{item:one-sided:pq:step:Naor-rho,item:one-sided:pq:step:committing} in the left session).

\para{Proving \Cref{item:lem:one-sided:pq:proof:core:2} of \Cref{lem:one-sided:pq:proof:core}.}  First, observe that the distribution of the prefix is identical in $G^{\mcal{M}_\secpar}(\secpar, m, \rho_\secpar)$ and $H^{\mcal{M}_\secpar}(\secpar, m, \rho_\secpar)$.
For each fixed prefix, \Cref{lem:small-tag:proof:se:pq} implies that the trace distance between the outputs of $G^{\mcal{M}_\secpar}(\secpar, m, \rho_\secpar)$ and $H^{\mcal{M}_\secpar}(\secpar, m, \rho_\secpar)$ are at most $\delta(\secpar)$ where we remark that we run $\mcal{SE}$ with the second input $1^{\delta^{-1}}$ in $G^{\mcal{M}_\secpar}(\secpar, m, \rho_\secpar)$. 
This immediately implies \Cref{item:lem:one-sided:pq:proof:core:2} of \Cref{lem:one-sided:pq:proof:core}. 

\subsection{Proof of \Cref{lem:small-tag:proof:se:pq}}
\label{lem:small-tag:proof:se:proof:pq}
First, we show a technical lemma that gives an extractor $\mcal{K}$ without the simulation property, which is the counterpart of  \Cref{lem:small-tag:proof:se:proof:K:pq}. 

\begin{lemma}\label{lem:small-tag:proof:se:proof:K:pq}
Let $H^{\mcal{M}_\secpar}_{\msf{pre}}(\secpar, m, \rho_\secpar)$, $\mcal{A}$, $\mcal{B}$ be as defined in \Cref{hybrid:H:reinterpretation:pq}. There exists a QPT machine $\mcal{K}$ such that for any $(\msf{st}_{\mcal{M}},  \msf{st}_C, \msf{st}_R, \tilde{\tau})$ in the support of $H^{\mcal{M}_\secpar}_{\msf{pre}}(\secpar, m, \rho_\secpar)$ and any noticeable $\epsilon(\secpar)$, the following holds:
\begin{enumerate}
\item \label[Property]{property:small-tag:proof:se:proof:K:syntax:pq}
{\bf (Syntax.)} $\mcal{K}$ takes as input $(1^\secpar, \msf{st}_C, \msf{st}_R, \tilde{\tau})$ and makes oracle access to $\Adv(\msf{st}_{\mcal{M}})$. It output a value $\msf{Val}_{\mcal{K}} \in \bits^{\ell(\secpar)} \cup \Set{\bot}$ such that $\msf{Val}_{\mcal{K}} = \msf{val}(\tilde{\tau})$ whenever $\msf{Val}_{\mcal{K}} \ne \bot$.
%(Also \Cref{rmk:small-tag:proof:se:proof:K:output:pq} for an intuitive explanation.)

\item \label[Property]{property:small-tag:proof:se:proof:K:pq}
If $\Pr[b = \top : (\OUT_\mcal{A}, b)\gets \langle \mcal{A}(\msf{st}_{\mcal{M}}), \mcal{B}(\msf{st}_C, \msf{st}_R) \rangle(1^\secpar, \tilde{\tau})] \ge \epsilon(\secpar)$, then it holds that
$$\Pr[\Val_{\mcal{K}} = \msf{val}(\tilde{\tau}) : \Val_{\mcal{K}} \gets \mcal{K}^{\A(\msf{st}_{\mcal{M}})}(1^\secpar,1^{\epsilon^{-1}}, \msf{st}_C, \msf{st}_R, \tilde{\tau})] \ge \frac{\epsilon'(\secpar)}{\tilde{t}},$$
where  $\epsilon'(\secpar) = \frac{\epsilon(\secpar)}{10t^2}$.
\end{enumerate}
\end{lemma}
\begin{remark}
Unlike in the classical counterpart (\Cref{lem:small-tag:proof:se:proof:K:pq}), $\mcal{K}$ in \Cref{lem:small-tag:proof:se:proof:K:pq} takes $1^{\epsilon^{-1}}$ as an additional input. This is needed because we only require witness-extended $\epsilon$-close emulation property (as per \Cref{def:PQWIAoK}) for $\WIAoK$, which causes an (arbitrarily small) noticeable simulation error. 
Note that this is enough for applying the extract-and-simulate lemma (\Cref{lem:extract_and_simulate}). 
As a positive effect of the above difference, $\mcal{K}$ in \Cref{lem:small-tag:proof:se:proof:K:pq} runs in \emph{strict} QPT whereas it runs in \emph{expected} PPT in  \Cref{lem:small-tag:proof:se:proof:K:pq}. 
%$\mcal{K}$ in \Cref{lem:small-tag:proof:se:proof:K:pq} runs in \emph{strict} QPT whereas it runs in \emph{expected} PPT in \Cref{lem:small-tag:proof:se:proof:K:pq}. This is because we rely on an extractor with $\epsilon$-close simulation (as per \Cref{def:PQWIAoK}) that runs in strict QPT.
%This could be done in the classical setting as well if we rely on the classical counter part of strict PPT extractor with $\epsilon$-close simulation.
\end{remark}

We prove \Cref{lem:small-tag:proof:se:proof:K:pq} in \Cref{sec:lem:small-tag:proof:se:proof:K:proof:pq}.
\takashi{I believe we can defer the proof of \Cref{lem:small-tag:proof:se:proof:K:pq} to Appendix in the final version. That is really the same as the classical case.} \xiao{Sure! You can leave all the figure-making task to me.}
In the rest of this subsection, we finish the proof of \Cref{lem:small-tag:proof:se:pq} assuming \Cref{lem:small-tag:proof:se:proof:K:pq} is true.
\begin{proof}[Proof of \Cref{lem:small-tag:proof:se:pq}]
We apply \Cref{lem:extract_and_simulate} where we think of $\langle \mcal{A}(\msf{st}_{\mcal{M}}), \mcal{B}(\msf{st}_C, \msf{st}_R) \rangle$ of \Cref{lem:small-tag:proof:se:proof:K:pq} as $\A$ in \Cref{lem:extract_and_simulate}. Then, the two properties of \Cref{lem:small-tag:proof:se:proof:K:pq} directly imply the two requirements of \Cref{lem:extract_and_simulate} where we think of $\msf{val}(\tilde{\tau})$ as $s^*$ in \Cref{lem:extract_and_simulate} 
noting that $\frac{\epsilon'(\secpar)}{\tilde{t}}$ is noticeable when $\epsilon(\secpar)$ is noticeable. Thus, \Cref{lem:extract_and_simulate} gives $\mcal{SE}$ that satisfies the requirements of \Cref{lem:small-tag:proof:se:pq}.
\end{proof}

\subsection{Extractor $\mcal{K}$ (Proof of \Cref{lem:small-tag:proof:se:proof:K:pq})}
\label{sec:lem:small-tag:proof:se:proof:K:proof:pq}

In this section, we prove \Cref{lem:small-tag:proof:se:proof:K:pq}. 
The proof is very similar to the proof of \Cref{lem:small-tag:proof:se:proof:K} in \Cref{sec:lem:small-tag:proof:se:proof:K:proof:pq} and the following proof is taken verbatim from there except for some adaptations. 
The only difference is that we need to carefully set a sufficiently small simulation error parameter for the extractor of $\WIAoK$. (Recall that we relied on an extractor for $\WIAoK$ with a negligible error in the classical counterpart.)
The main differences from the classical counterpart are highlighted by {\color{red} red color}.


We will construct the extractor $\mcal{K}$ prescribed in \Cref{lem:small-tag:proof:se:proof:K:pq}, and show that it satisfies the required properties. 
We will build the extractor $\mcal{K}$
gradually, starting by defining several intermediate machines.
The description of $\mcal{K}$ will appear toward the end of this subsection (on \Cpageref{extractorK:description:pq}). We found this arrangement most reader-friendly. We illustrate all the intermediate machines in \Cref{figure:one-sided:pq:games}.
\takashi{@Xiao can you make a new figure where WIAoK is replaced with WIAoK and $H^{\mcal{M}}(\secpar,m,z)$ is replaced with $H^{\mcal{M}_\secpar}(\secpar,m,\rho_\secpar)$? I believe no other change is needed.}
{\color{red}
\begin{remark}\label{rem:hardwire_epsilon}
In the following descriptions, 
we fix the noticeable function $\epsilon(\secpar)$ in \Cref{lem:small-tag:proof:se:proof:K:pq} and describe these machines as if $\epsilon$ is hardwired into them. However, it is easy to see that we can construct similar machines that work similarly when $1^{\epsilon^{-1}}$ is given as an additional input instead of being hardwired. 
\takashi{Here is a subtlety about the dependence on the parameter $\epsilon$. Does the above explanation make sense?}
\end{remark}
}




\para{Machine $\mcal{G}_{i}$ ($i \in [\tilde{t}]$):\label{machine:Gi:pq}} (Illustrated in \Cref{figure:one-sided:pq:Gi}.) 
Recall that we re-interpreted the man-in-the-middle execution $H^{\mcal{M}_\secpar}(\secpar,m,\rho_\secpar)$ defined on \Cpageref{gameH:description:pq} (and depicted in \Cref{figure:one-sided:pq:H}) as \Cref{hybrid:H:reinterpretation:pq}. We now define $\mcal{G}_1(\msf{pref})$ as the machine corresponding to \Cref{stage:hybrid:H:remainder} of \Cref{hybrid:H:reinterpretation:pq}.  That is, on input the prefix $\msf{pref}$ (defined in \Cref{hybrid:H:reinterpretation:1:pq} of \Cref{hybrid:H:reinterpretation:pq}), $\mcal{G}_1(\msf{pref})$ behaves identically as the $\langle\mcal{A}(\msf{st}_{\mcal{M}}), \mcal{B}(\msf{st}_C, \msf{st}_R) \rangle(1^\secpar, \tilde{\tau})$ defined in \Cref{expression:hybrid:H:remainder:pq}. In particular, $\mcal{G}_1(\msf{pref})$ uses the witness $(1, \tilde{x}_1)$ to go through the right {\bf WIAoK-1}. (The subscript ``1'' is meant to indicate the fact that $(1,\tilde{x}_1)$ was used).

Then, for any $i \in [\tilde{t}]\setminus \Set{1}$, we define $\mcal{G}_{i}(\msf{pref})$ as the machine that behaves identically to $\mcal{G}_1(\msf{pref})$, except that $\mcal{G}_i(\msf{pref})$ uses the witness $\tilde{x}_{i}$ in the right {\bf WIAoK-1}.

For a prefix $\msf{pref} = (\msf{st}_{\mcal{M}}, \msf{st}_C, \msf{st}_R, \tilde{\tau})$, let us define a notation that describes the probability that $\msf{pref}$ leads to an accepting execution:
\begin{definition}\label{def:p-tau:2:pq}
For any $\msf{pref} = (\msf{st}_{\mcal{M}}, \msf{st}_C, \msf{st}_R, \tilde{\tau})$ in the support of $H^{\mcal{M}}_{\msf{pre}}(\secpar,m,z)$, we define
\begin{equation}\label{eq:def:p-tau:pq}
p_{\msf{pref}} \coloneqq \Pr[b = \top : (\OUT, b) \gets \mcal{G}_1(\msf{pref})].
\end{equation}
\end{definition}
\begin{remark}\label{rmk:redefine:p-pref:pq}
It is worth noting that the above $p_{\msf{pref}}$ is exactly the following probability that appeared in \Cref{property:small-tag:proof:se:proof:K:pq} of \Cref{lem:small-tag:proof:se:proof:K:pq}: $p_{\msf{pref}} = \Pr[b = \top : (\OUT_\mcal{A}, b)\gets \langle \mcal{A}(\msf{st}_{\mcal{M}}), \mcal{B}(\msf{st}_C, \msf{st}_R) \rangle(1^\secpar, \tilde{\tau})]$.
\end{remark}

We first claim that the accepting probabilities for $\mcal{G}_i(\msf{pref})$'s with different $i \in [\tilde{t}]$  are almost the same.
\begin{figure}[!tb]
     \begin{subfigure}[t]{0.47\textwidth}
         \centering
         \fbox{
         \includegraphics[width=\textwidth,page=1]{figures/figures.pdf}
         }
         \caption{}
         \label{figure:one-sided:pq:H}
     \end{subfigure}
     \hspace{6.5pt}
     \begin{subfigure}[t]{0.47\textwidth}
         \centering
         \fbox{
         \includegraphics[width=\textwidth,page=2]{figures/figures.pdf}
         }
         \caption{}
         \label{figure:one-sided:pq:Gi}
     \end{subfigure}
     \vskip\baselineskip
      \begin{subfigure}[t]{0.47\textwidth}
         \centering
         \fbox{
         \includegraphics[width=\textwidth,page=3]{figures/figures.pdf}
         }
         \caption{}
         \label{figure:one-sided:pq:G'i}
     \end{subfigure}
     \hspace{6.5pt}
     \begin{subfigure}[t]{0.47\textwidth}
         \centering
         \fbox{
         \includegraphics[width=\textwidth,page=4]{figures/figures.pdf}
         }
         \caption{}
         \label{figure:one-sided:pq:G''i}
     \end{subfigure}
     \vskip\baselineskip
     \begin{subfigure}[t]{0.47\textwidth}
         \centering
         \fbox{
         \includegraphics[width=\textwidth,page=5]{figures/figures.pdf}
         }
         \caption{}
         \label{figure:one-sided:pq:Ki}
     \end{subfigure}
     \hspace{6.5pt}
     \begin{subfigure}[t]{0.47\textwidth}
         \centering
         \fbox{
         \includegraphics[width=\textwidth,page=6]{figures/figures.pdf}
         }
         \caption{}
         \label{figure:one-sided:pq:K}
     \end{subfigure}
     \caption{Different Hybrids/Machines \scriptsize{(Changes between adjacent machines are highlighted by red color)}}
     \label{figure:one-sided:pq:games}
\end{figure}

\begin{MyClaim}\label{claim:bound:Gi:pq}  
$\forall i \in [\tilde{t}], ~\Pr[b = \top : (\OUT, b) \gets \mcal{G}_i(\msf{pref})] \ge p_{\msf{pref}} - \negl(\secpar)$.
\end{MyClaim}
\begin{proof}
Note that the machine $\mcal{G}_i(\msf{pref})$ does not rewind the right {\bf WIAoK-1}, and for any $i \in [\tilde{t}] \setminus \Set{1}$, $\mcal{G}_i(\msf{pref})$ differs from $\mcal{G}_1(\msf{pref})$ only by the witness used in the right {\bf WIAoK-1}. Therefore, it follows from the WI property of the right {\bf WIAoK-1} that for any $i \in [\tilde{t}]$,
$$\big| \Pr[b_i = \top : (\OUT_i, b_i) \gets \mcal{G}_i(\msf{pref})] - \Pr[b_1 = \top : (\OUT_1, b_1) \gets \mcal{G}_1(\msf{pref})]\big| \le \negl(\secpar).$$
Then, by the definition of $p_{\msf{pref}}$ (as per \Cref{eq:def:p-tau:pq}), \Cref{claim:bound:Gi:pq} follows.
\end{proof}

\para{Machine $\mcal{G}'_i$ ($i\in [\tilde{t}]$):} (Illustrated in \Cref{figure:one-sided:pq:G'i}.) On input $\msf{pref}$, $\mcal{G}'_i(\msf{pref})$ behaves identically to $\mcal{G}_i(\msf{pref})$, except the following change. Instead of executing the left {\bf WIAoK-1} (i.e., \Cref{item:one-sided:pq:step:WIAoK:1} in the left) honestly, $\mcal{G}'_i$ invokes the emulation-extractor $\SimExt$ {\color{red} with the simulation error parameter $\epsilon_\wiaok(\secpar)\defeq \frac{t+1}{t^2+5t+2}\cdot \epsilon'(\secpar)=\frac{t+1}{10t^2(t^2+5t+2)}\cdot \epsilon(\secpar)$} to emulate the left {\bf WIAoK-1} while extracting some $w'$, which is the third output of $\mcal{SE}$ (see \Cref{item:PQWEE} of \Cref{def:PQWIAoK}).\footnote{Do not confuse it with $\mcal{SE}$ in \Cref{lem:small-tag:proof:se:pq}. $\mcal{SE}$ always means that in \Cref{item:PQWEE} of \Cref{def:PQWIAoK} throughout this and the next subsection.} Depending on the value of $w'$, there are two possibilities:
\begin{enumerate}
\item
{\bf Case $w' \in \Relation_{\Lang^t_f}(Y)$:} This is the case that $w'$ is a valid witness for the statement proven by the left {\bf WIAoK-1}. That is, $w'$ equals to some $(j,x_j) \in \Relation_{\Lang^t_f}(Y)$ (see \Cref{eq:one-sided:pq:Lang:OWF}). In this case, $\mcal{G}'_i(\msf{pref})$ continues to finish the execution identically as $\mcal{G}_i(\msf{pref})$.
\item
{\bf Case $w' \notin \Relation_{\Lang^t_f}(Y)$:} In this case, $\mcal{G}'_i(\msf{pref})$ aborts immediately, outputting $(\OUT, b) \coloneqq (\bot, \bot)$.
\end{enumerate}
It is worth noting that although $\SimExt$ may extract a valid $(j, x_j)$ pair, $\mcal{G}'_i(\msf{pref})$ does {\em not} use it yet.  

\begin{MyClaim}\label{claim:bound:G'i:pq}
$\forall i \in [\tilde{t}], ~\Pr[b = \top : (\OUT, b) \gets \mcal{G}'_i(\msf{pref})] \ge p_{\msf{pref}}{\color{red}-\epsilon_\wiaok(\secpar)}  - \negl(\secpar)$.
\end{MyClaim}
\begin{proof}
This claim follows immediately from \Cref{claim:bound:Gi:pq} and the witness-extended $\epsilon_\wiaok$-close emulation property (as per \Cref{item:PQWEE} of \Cref{def:PQWIAoK}) of the left {\bf WIAoK-1}.
\end{proof}


\para{Machine $\mcal{G}''_i$ ($i\in [\tilde{t}]$):} (Illustrated in \Cref{figure:one-sided:pq:G''i}.) On input $\msf{pref}$, $\mcal{G}''_i(\msf{pref})$ behaves identically to $\mcal{G}'_i(\msf{pref})$, except that $\mcal{G}''_i(\msf{pref})$ uses the $w'=(j, x_j)$ (extracted in $\mcal{G}'_i(\msf{pref})$, if it is a valid witness) to finish the left {\bf WIAoK-2} (i.e., \Cref{item:one-sided:pq:step:WIAoK:2} in the left execution).
\begin{MyClaim}\label{claim:bound:G''i:pq}  
$\forall i \in [\tilde{t}], ~\Pr[b = \top : (\OUT, b) \gets \mcal{G}''_i(\msf{pref})] \ge p_{\msf{pref}}{\color{red}-\epsilon_\wiaok(\secpar)} - \negl(\secpar)$.
\end{MyClaim}
\begin{proof}
This claim follows immediately from \Cref{claim:bound:G'i:pq} and the WI property of the left {\bf WIAoK-2}.
\end{proof}


\para{Machine $\mcal{K}_i$ ($i\in [\tilde{t}]$):} (Illustrated in \Cref{figure:one-sided:pq:Ki}.) On input a prefix $\msf{pref}$, $\mcal{K}_i(\msf{pref})$ behaves identically to $\mcal{G}''_i(\msf{pref})$, except for the following difference. Machine $\mcal{K}_i(\msf{pref})$ uses the witness-extended emulator $\SimExt$ {\color{red} with the simulation error parameter $\epsilon_\wiaok(\secpar)$} to finish the right {\bf WIAoK-2}, instead of playing the role of the honest receiver. 

\subpara{$\mcal{K}_i$'s Output:\label{subpara:K-i:output:pq}} Let $w'$ denote the third output of $\SimExt$ (see \Cref{item:PQWEE} of \Cref{def:PQWIAoK}), which is supposed to be the witness used by $\mcal{M}$ in the right {\bf WIAoK-2} (for the statement $(\tilde{\msf{com}}, \tilde{Y}$) w.r.t.\ the language $\Lang_{\tilde{\gamma}}\vee \Lang^{\tilde{t}}_{\tilde{f}}$). Depending on the value of $w'$, we define a value $\msf{Val} \in \bits^{\ell(\secpar)} \cup \Set{\bot_{\tilde{Y}}, \bot_{\msf{invalid}}}$ as follows:
\begin{enumerate}
\item \label[Case]{K-i:output:case:1:pq}
If $w'$ is a valid witness for $(\tilde{\msf{com}}, \tilde{Y}) \in \Lang_{\tilde{\gamma}}\vee \Lang^{\tilde{t}}_{\tilde{f}}$. Then, there are tow sub-cases:
\begin{enumerate}
\item \label[Case]{K-i:output:case:1a:pq}
$w'$ is a valid witness for $\tilde{\msf{com}} \in \Lang_{\tilde{\gamma}}$. In this case, $w'$ consists of the value $\msf{val}(\tilde{\tau})$, i.e., the value committed in $\tilde{\tau}=(\tilde{\gamma}, \tilde{\msf{com}})$, and the randomness $\tilde{r}$. We set $\msf{Val} \coloneqq \msf{val}(\tilde{\tau})$. Importantly, notice that we do {\em not} include the randomness $\tilde{r}$ in $\msf{Val}$. %(as explained in \Cref{rmk:small-tag:proof:se:proof:K:output}.).
\item \label[Case]{K-i:output:case:1b:pq}
$w'$ is a valid witness for $\tilde{Y} \in \Lang^{\tilde{t}}_{\tilde{f}}$: In this case, we set $\msf{Val} \coloneqq \bot_{\tilde{Y}}$.
\end{enumerate}

\item \label[Case]{K-i:output:case:2:pq}
Otherwise, set $\msf{Val} \coloneqq \bot_{\msf{invalid}}$.
\end{enumerate}


The output of $\mcal{K}_i$ is defined to be $\msf{Val}$. Note that this is in contrast to all previous machines, for which the output is defined to be the main-in-the-middle's output and the honest receiver's decision bit. We emphasize that such a $\msf{Val}$ satisfies the syntax requirement in \Cref{property:small-tag:proof:se:proof:K:syntax} of \Cref{lem:small-tag:proof:se:proof:K:pq}. In particular, {\em $\msf{Val} = \msf{val}(\tilde{\tau})$ whenever $\msf{Val} \ne \bot$}.\footnote{Note that here we defined two types of abortion: $\bot_{\tilde{Y}}$ and $\bot_{\msf{invalid}}$, while \Cref{property:small-tag:proof:se:proof:K:syntax} of \Cref{lem:small-tag:proof:se:proof:K:pq} only allows a single abortion symbol $\bot$. We remark that this is only a cosmetic difference---It can be made consistent using the following rules: $\bot = \bot_{\tilde{Y}}$ {\em and} $\bot = \bot_{\msf{invalid}}$ (i.e., $\msf{Val} \ne \bot  \Leftrightarrow (\msf{Val} \ne \bot_{\tilde{Y}} \wedge \msf{Val} \ne \bot_{\msf{invalid}})$).}

\begin{MyClaim}\label{claim:bound:Ki:pq}
$\forall i \in [\tilde{t}], ~\Pr[\Val \ne \bot_{\msf{invalid}} :\Val \gets \mcal{K}_i(\msf{pref})] \ge p_{\msf{pref}} {\color{red}-2\epsilon_\wiaok(\secpar)}- \negl(\secpar)$.
\end{MyClaim}
\begin{proof}
This claim follows immediately from \Cref{claim:bound:G''i:pq} and the witness-extended $\epsilon_\wiaok$-close emulation property (as per \Cref{item:PQWEE} of \Cref{def:PQWIAoK}) of the right {\bf WIAoK-2}.
\end{proof}

Finally, we are ready to define the extractor $\mcal{K}$. Intuitively, $\mcal{K}$ can be conceived as an average-case version of $\Set{\mcal{K}_i}_{i\in[\tilde{t}]}$:

\para{Extractor $\mcal{K}$:\label{extractorK:description:pq}} (Illustrated in \Cref{figure:one-sided:pq:K}.)  On input $\msf{pref}$, $\mcal{K}(\msf{pref})$ samples uniformly at random an index $i \pick [\tilde{t}]$, executes $\mcal{K}_i(\msf{pref})$, and outputs whatever $\mcal{K}_i(\msf{pref})$ outputs.


\begin{remark}[On the Notation of $\mcal{K}$]\label{rmk:notation-K:pq}
It is worth noting that in the above, we write machine $\mcal{K}$ as $\mcal{K}(\msf{pref})$, while it was written as in \Cref{lem:small-tag:proof:se:proof:K:pq} as $\mcal{K}^{\A(\msf{st}_{\mcal{M}})}(1^\secpar,1^{\epsilon^{-1}} \msf{st}_C, \msf{st}_R, \tilde{\tau})$. This is only a cosmetic difference---
First, we remark that we consider $\epsilon$ to be hardwired into $\mcal{K}$ for simplicity as remarked in \Cref{rem:hardwire_epsilon}. 
Then, $\mcal{K}(\msf{pref})$ can be explained in the following way: first, parse $\msf{pref}$ as $(\msf{st}_{\mcal{M}},\msf{st}_C, \msf{st}_R, \tilde{\tau})$; then, run $\mcal{K}^{\A(\msf{st}_{\mcal{M}})}(1^\secpar, \msf{st}_C, \msf{st}_R, \tilde{\tau})$. 
\end{remark}


Next, we show that the extractor $\mcal{K}$ satisfies the requirements in \Cref{lem:small-tag:proof:se:proof:K:pq}.

\para{Running Time of $\mcal{K}$.} Observe that for each $i \in [\tilde{t}]$, $\mcal{K}_i(\msf{pref})$ is the same as the real man-in-the-middle execution conditioned on the prefix $\msf{pref}$, except that $(i,\tilde{x}_i)$ is used in the right {\bf WIAoK-1} and the witness-extended emulator $\SimExt$ is used in the right {\bf WIAoK-2} and the left {\bf WIAoK-1}. Since $\SimExt$ runs in QPT, so does $\mcal{K}_i(\msf{pref})$. Therefore, $\mcal{K}(\msf{pref})$ also runs in QPT.

\para{Proving \Cref{property:small-tag:proof:se:proof:K:syntax:pq} of \Cref{lem:small-tag:proof:se:proof:K:pq}.} It is straightforward to see that the $\mcal{K}$ defined above satisfies the syntax requirement in \Cref{lem:small-tag:proof:se:proof:K:pq} (see also \Cref{rmk:notation-K:pq}). In particular, we have $\msf{Val}_{\mcal{K}} = \msf{val}(\tilde{\tau})$ whenever $\msf{Val}_{\mcal{K}} \ne \bot$, because this is true for each $\mcal{K}_i$ by definition (see the paragraph for ``\underline{$\mcal{K}_i$'s Output}'' on \Cpageref{subpara:K-i:output:pq}).


\para{Proving \Cref{property:small-tag:proof:se:proof:K:pq} of \Cref{lem:small-tag:proof:se:proof:K:pq}.} First, recall that \Cref{property:small-tag:proof:se:proof:K:pq} requires that 
for any $\msf{pref}$ in the support of $H^{\mcal{M}}_{\msf{pre}}(\secpar, m, z)$ , if $p_{\msf{pref}} \ge \epsilon(\secpar)$ (see \Cref{rmk:redefine:p-pref}), then it holds that
\begin{equation}\label[Inequality]{eq:bound:averageK:pq}
\Pr[\Val_{\mcal{K}} = \msf{val}(\tilde{\tau}) : \Val_{\mcal{K}} \gets \mcal{K}(\msf{pref})] \ge \frac{\epsilon'(\secpar)}{\tilde{t}}.
\end{equation} 
Also recall that $\mcal{K}(\msf{pref})$ is defined to execute the machine $\mcal{K}_i(\msf{pref})$  with  $i$ uniformly sampled from $[\tilde{t}]$. Therefore, \Cref{eq:bound:averageK:pq} can be reduced to the following \Cref{lem:bound:Ki:pq}. We will prove \Cref{lem:bound:Ki:pq} in \Cref{sec:lem:bound:Ki:proof}, which will eventually finish the current proof of \Cref{lem:small-tag:proof:se:proof:K:pq}.
\begin{lemma}\label{lem:bound:Ki:pq}
Let $\epsilon(\secpar) = \frac{1}{\poly(\secpar)}$ and $\epsilon'(\secpar) = \frac{\epsilon(\secpar)}{t^2}$.
For any $\msf{pref} = (\msf{st}_{\mcal{M}},\msf{st}_C, \msf{st}_R, \tilde{\tau})$, if $p_\msf{pref} \ge \epsilon(\secpar)$, then there exists an $i \in [\tilde{t}]$ such that 
$$\Pr[\Val = \msf{val}(\tilde{\tau}) :\Val \gets \mcal{K}_i(\msf{pref})] \ge \epsilon'(\secpar).$$
\end{lemma}

\subsection{Proof of \Cref{lem:bound:Ki:pq}}
\label{sec:lem:bound:Ki:proof:pq}
The proof of \Cref{lem:bound:Ki:pq} is almost identical to the proof of \Cref{lem:bound:Ki:pq} in \Cref{sec:lem:bound:Ki:proof:pq}. 
The main differences from the classical counterpart are highlighted by {\color{red} red color}.

\para{Notation.} We highly recommend reviewing the ``\underline{$\mcal{K}_i$'s Output}'' part on \Cpageref{subpara:K-i:output:pq} (in particular, the meanings of $\msf{Val}$, $\bot_{\tilde{Y}}$, and $\bot_{\msf{invalid}}$) before starting reading this subsection.  Recall that $\mcal{K}_i$'s output $\msf{Val}$ is determined by the $w'$ output by the right {\bf WIAoK-2} simulation-extractor $\mcal{SE}$. In this subsection, we will need to refer to this $w'$, although it is not included as a part of $\mcal{K}_i$'s output. Particularly, we will make use of the following notation: whenever we write an expression of the form 
 $$\Pr[\text{Some Event $E_{w'}$ about $w'$}: \msf{Val} \gets \mcal{K}_i(\msf{pref})],$$
it should be understood as the provability of $E_{w'}$, where $w'$ refers to the $w'$ generated during the random procedure $\msf{Val} \gets\mcal{K}_i(\msf{pref})$, over which the probability is taken. 

Using these notations, we can partition the event $\msf{Val} = \bot_{\tilde{Y}}$ as the following {\em mutually exclusive} events: $w' = (1, \tilde{x}_1)$, or, $\ldots$, or $w' =(\tilde{t}, \tilde{x}_{\tilde{t}})$, where $\tilde{y}_i = \tilde{f}(\tilde{x}_i)$ for each $i \in [\tilde{t}]$.   Formally, we express this relation by 
\begin{equation}\label{eq:bot-tilde-Y:partition:pq}
\Pr[\msf{Val} = \bot_{\tilde{Y}}: \msf{Val} \gets \mcal{K}_i(\msf{pref})] = \sum_{i = 1}^{\tilde{t}} \Pr[w' = (i,\tilde{x}_i): \msf{Val} \gets \mcal{K}_i(\msf{pref})]
\end{equation}

With the above notations, we start proving \Cref{lem:bound:Ki:pq} in the following.

\para{The Actual Proof for \Cref{lem:bound:Ki:pq}.} We assume for contradiction that for some $\msf{pref}$ satisfying $p_{\msf{pref}} \ge \epsilon(\secpar)$, it holds that 
\begin{equation}\label[Inequality]{eq:proof:averageK:contra-assump:pq}
\forall i \in [\tilde{t}], ~\Pr[\Val = \msf{val}(\tilde{\tau}) :\Val \gets \mcal{K}_i(\msf{pref})] < \epsilon'(\secpar).
\end{equation}
\begin{MyClaim}\label{claim:bound:Ki-xi:pq}
Under the assumption in \Cref{eq:proof:averageK:contra-assump:pq}, it holds that 
$$\forall i \in [\tilde{t}], ~\Pr[w' = (i, \tilde{x}_i) :\Val \gets \mcal{K}_i(\msf{pref})] \ge p_{\msf{pref}}  {\color{red}-2\epsilon_\wiaok(\secpar)} - \epsilon'(\secpar) - \negl(\secpar).$$
\end{MyClaim}
\begin{proof}
% First, recall that the event $\Val \ne \bot$ (i.e., $\Val$ is a valid witness) can be partitioned into the following {\em disjoint} events: $\Val = \msf{val}(\tilde{\tau})$, $\Val = \tilde{x}_1$, \ldots, $\Val = \tilde{x}_{\tilde{t}}$. Therefore,

 First, notice that
\begin{align*}
\forall i \in [\tilde{t}], ~\Pr[\Val \ne \bot_{\msf{invlid}}] 
& = 
\Pr[\Val = \msf{val}(\tilde{\tau})] +  \Pr[\Val = \bot_{\tilde{Y}}] \\
\text{(by \Cref{eq:bot-tilde-Y:partition:pq})} ~& = 
\Pr[\Val = \msf{val}(\tilde{\tau})] + \Pr[w' = (i, \tilde{x}_i)] + \sum_{j \in [\tilde{t}]\setminus \Set{i}} \Pr[w' = (j, \tilde{x}_j)], \numberthis \label{eq:bound:Ki-xi:1:pq}
\end{align*}
where all the probabilities are taken over the random procedure $\Val \gets \mcal{K}_i(\msf{pref})$.

Then, the following holds
(all the probabilities below are taken w.r.t.\ $\Val \gets \mcal{K}_i(\msf{pref})$):
\begingroup\fontsize{9.5pt}{0pt}\selectfont
\begin{align}
\forall i \in [\tilde{t}], ~\Pr[w' = (i, \tilde{x}_i)] 
& = 
\Pr[\Val \ne \bot_{\msf{invalid}}] - \Pr[\Val = \msf{val}(\tilde{\tau})] -  \bigg(\sum_{j \in [\tilde{t}]\setminus \Set{i}} \Pr[w' = (j, \tilde{x}_j)] \bigg)  \label{eq:bound:Ki-xi:derive:1:pq} \\
& \ge p_{\msf{pref}} {\color{red}-2\epsilon_\wiaok(\secpar)}- \negl(\secpar) - \Pr[\Val = \msf{val}(\tilde{\tau})] -  \bigg(\sum_{j \in [\tilde{t}]\setminus \Set{i}} \Pr[w' = (j,\tilde{x}_j)] \bigg)  \label[Inequality]{eq:bound:Ki-xi:derive:2:pq}\\
& \ge p_{\msf{pref}} {\color{red} -2\epsilon_\wiaok(\secpar)} - \negl(\secpar) - \epsilon'(\secpar) -  \bigg(\sum_{j \in [\tilde{t}]\setminus \Set{i}} \Pr[w' = (j,\tilde{x}_j)] \bigg), \label[Inequality]{eq:bound:Ki-xi:derive:3:pq}
\end{align}
\endgroup
where \Cref{eq:bound:Ki-xi:derive:1:pq} follows from \Cref{eq:bound:Ki-xi:1:pq}, \Cref{eq:bound:Ki-xi:derive:2:pq} follows from \Cref{claim:bound:Ki:pq}, and \Cref{eq:bound:Ki-xi:derive:3:pq} follows from \Cref{eq:proof:averageK:contra-assump:pq}.

Now, to prove \Cref{claim:bound:Ki-xi:pq}, it suffices to show that 


\begin{equation}
\forall i \in [\tilde{t}],~\forall j \in [\tilde{t}]\setminus \Set{i}, ~\Pr[w' = (j,\tilde{x}_j) : \Val \gets \mcal{K}_i(\msf{pref})] = \negl(\secpar).
\end{equation}
This can be reduced via standard techniques to the one-wayness of the OWF $\tilde{f}$ in \Cref{item:one-sided:pq:step:OWFs} of the right execution. In more details, we assume for contradiction that there exist $i^*, j^* \in [\tilde{t}]$ such that $i^* \ne j^*$ and that the probability $\Pr[w' = (j^*, \tilde{x}_{j^*}) : \Val \gets \mcal{K}_{i^*}(\msf{pref})]$ is non-negligible, where, by definition, $\tilde{x}_{j^*}$ is the preimage of $\tilde{y}_{j^*}$ under the right OWF $\tilde{f}$. Then, we can build a QPT adversary $\Adv_\textsc{owf}$ breaking one-wayness in the following way: $\Adv_\textsc{owf}$ obtains the challenge $y^*$ from the external one-wayness challenger; it then runs the machine $\mcal{K}_{i^*}(\msf{pref})$ internally, for which $\Adv_\textsc{owf}$ uses $y^*$ in place of $\tilde{y}_{j^*}$ when executing \Cref{item:one-sided:pq:step:OWFs} in the right. Note that the internal execution of $\mcal{K}_{i^*}(\msf{pref})$ is identically to the real execution of $\mcal{K}_{i^*}$, thus the extracted $w' =(j^*, \tilde{x}_{j^*})$ must satisfy $\tilde{f}(\tilde{x}_{j^*}) = \tilde{y}_j^*~(=y^*)$ with non-negligible probability, breaking one-wayness. 

This finishes the proof of \Cref{claim:bound:Ki-xi:pq}.
\end{proof}

\takashi{@Xiao Can I ask you to replace WIPoK with WIAoK in \Cref{figure:one-sided:K'i-K''i:pq}
?} \xiao{Yes, I'll do that. Actually, I'll considering replacing WIPoK by WIAoK throughout the whole paper.}

\para{Machine $\mcal{K}'_i$ ($i \in [\tilde{t}]$):\label{machineK':description:pq}} (Illustrated in \Cref{figure:one-sided:K'i:pq}.) On input a prefix $\msf{pref}$, $\mcal{K}'_i(\msf{pref})$ proceeds as follows:
\begin{enumerate}
\item
$\mcal{K}'_i(\msf{pref})$ first finishes \Cref{item:one-sided:pq:step:OWFs} of the man-in-the-middle execution in the same way as $\mcal{K}_i(\msf{pref})$. In particular, it will see in the left execution the values $Y = (y_1, \ldots, y_t)$ sent from $\mcal{M}$; 
\item
$\mcal{K}'_i(\msf{pref})$ recovers $(x_1, \ldots, x_t)$ by brute-force: Namely, for each $i \in [t]$, it inverts the OWF $f$ to find $x_i$ s.t.\ $f(x_i) = y_i$. It is possible that there exist some ``bad'' $y_i$'s that are not in the range of $f$. For such bad $i$'s, it sets $x_i = \bot$. If all the $x_i$'s are bad, $\mcal{K}'_i(\msf{pref})$ halts and outputs $\msf{Fail}$;
\item \label[Step]{item:machineK':3:pq}
If this step is reached, we know that $(x_1, \ldots, x_t)$ cannot be all $\bot$. $\mcal{K}'_i(\msf{pref})$ then picks an $(s, x_s)$ uniformly at random from the good (i.e.\ non-$\bot$) $x_i$'s.
\item
$\mcal{K}'_i(\msf{pref})$ continues to finish the execution in the same way as $\mcal{K}_i(\msf{pref})$, except that it uses $(s, x_s)$ as the witness when executing the left {\bf WIAoK-2}. 
\end{enumerate}
It is worth noting that the $(j, x_j)$ extracted by the witness-extended emulator for the left {\bf WIAoK-1} (inherited from $\mcal{K}_i(\msf{pref})$) is not used any more by $\mcal{K}'_i(\msf{pref})$. 

It is easy to see that if the $(s, x_s)$ picked by $\mcal{K}'_i(\msf{pref})$ is equal to the $(j, x_j)$ extracted in $\mcal{K}_i(\msf{pref})$ from its left {\bf WIAoK-1}, then $\mcal{K}'_i(\msf{pref})$ and $\mcal{K}_i(\msf{pref})$ are identical (see \Cref{rmk:injectivity-of-OWF:pq}). Since $\mcal{K}'_i(\msf{pref})$ samples $(s,x_s)$ uniformly from all the good $(i, x_i)$'s, then $(s, x_s) = (j,x_j)$ with probability at least $1/t$.  Therefore, the following must hold: 
\begin{equation}\label[Inequality]{eq:bound:K'i:pq}
\forall i \in [\tilde{t}], ~\Pr[w' = (i, \tilde{x}_i) : \Val \gets \mcal{K}'_i(\msf{pref})] \ge \frac{1}{t}\cdot \Pr[w' = (i, \tilde{x}_i) : \Val \gets \mcal{K}_i(\msf{pref})].
\end{equation}
\begin{remark}[On Injectivity of the OWF]\label{rmk:injectivity-of-OWF:pq}
We emphasize that throughout the proof of non-malleability, this is {\em the only} place where we rely on the injectivity of the OWF. In particular, we rely on the injectivity of the OWF $f$ in the left session to ensure that there is a unique preimage for each $\Set{{y}_i}_{i \in [t]}$. Thus, if both the $x_s$ with $s = j$ (sampled by $\mcal{K}'_i(\msf{pref})$) and the extracted $x_j$ (in $\mcal{K}_i(\msf{pref})$) are a valid preimage for the same $y_j$, then $x_s$ must equal $x_j$.
The requirement of injectivity can be removed similarly to the classical case, which is explained in \Cref{sec:removing-injectivity}. 
%We will show how to remove the requirement of injectivity in \Cref{sec:removing-injectivity}.
\end{remark}
\begin{figure}[!tb]
     \begin{subfigure}[t]{0.47\textwidth}
         \centering
         \fbox{
         \includegraphics[width=\textwidth,page=7]{figures/figures.pdf}
         }
         \caption{}
         \label{figure:one-sided:K'i:pq}
     \end{subfigure}
     \hspace{6.5pt}
     \begin{subfigure}[t]{0.47\textwidth}
         \centering
         \fbox{
         \includegraphics[width=\textwidth,page=8]{figures/figures.pdf}
         }
         \caption{}
         \label{figure:one-sided:K''i:pq}
     \end{subfigure}
     \caption{Machines $\mcal{K}'_i(\msf{pref})$ and $\mcal{K}''_i(\msf{pref})$ \scriptsize{(Changes between adjacent machines are highlighted by red color)}}
     \label{figure:one-sided:K'i-K''i:pq}
\end{figure}

\para{Machine $\mcal{K}''_i$ ($i\in [\tilde{t}]$):} (Illustrated in \Cref{figure:one-sided:K''i:pq}.) On input a prefix $\msf{pref}$,  $\mcal{K}''_i(\msf{pref})$ behaves identically to $\mcal{K}'_i(\msf{pref})$ except that it plays as the honest committer in the left {\bf WIAoK-1}, instead of running the witness-extended emulator. Recall that starting from $\mcal{K}'_i$, the witness $(j, x_j)$ extracted by the witness-extended emulator from the left {\bf WIAoK-1} is not used any more. Thus, machine $\mcal{K}''_i$ does not need to perform this witness-extended emulation.

By the witness-extended $\epsilon_\wiaok$-close emulation property (as per \Cref{item:PQWEE} of \Cref{def:PQWIAoK}) of the left {\bf WIAoK-1}, it is easy to see that 
\begin{equation}\label[Inequality]{eq:relation:K'-K'':pq}
\forall i \in [\tilde{t}], ~\Pr[w' = (i,\tilde{x}_i):\Val \gets \mcal{K}''_i(\msf{pref})] \ge \Pr[w' = (i,\tilde{x}_i):\Val \gets \mcal{K}'_i(\msf{pref})] {\color{red}-\epsilon_\wiaok(\secpar)} -\negl(\secpar).
\end{equation}
Also, by the WI property of the right {\bf WIAoK-1}, the following must hold
\begin{equation}\label[Inequality]{eq:relation:K:WI:pq}
\forall i \in [\tilde{t}], ~\big|\Pr[w' = (i,\tilde{x}_i):\Val \gets \mcal{K}''_i(\msf{pref})] - \Pr[w' = (i,\tilde{x}_i):\Val \gets \mcal{K}''_1(\msf{pref})]\big|  \le \negl(\secpar).
\end{equation}
Then, we have the following claim:
\begin{MyClaim}\label{claim:bound:K''1:pq}
% For any $\mcal{\tau}$, if $p_{\tilde{\tau}} \ge \epsilon(\secpar)$, then it holds that
$\forall i \in [\tilde{t}], ~\Pr[w' = (i,\tilde{x}_i):\Val \gets \mcal{K}''_1({\msf{pref}})] \ge \frac{1}{t} \cdot \big(p_{\msf{pref}} {\color{red}-(t+2)\epsilon_\wiaok(\secpar)} -\epsilon'(\secpar)\big) - \negl(\secpar)$.
\end{MyClaim}
\begin{proof} 
This claim follows from \Cref{claim:bound:Ki-xi:pq} and \Cref{eq:bound:K'i:pq,eq:relation:K'-K'':pq,eq:relation:K:WI:pq}. Formally,
\begin{align}
\forall i \in [\tilde{t}], ~\Pr[w' = (i,\tilde{x}_i):\Val \gets \mcal{K}''_1({\msf{pref}})] 
 & \ge \Pr[w' = (i,\tilde{x}_i):\Val \gets \mcal{K}''_i({\msf{pref}})]{\color{red}-\epsilon_\wiaok(\secpar)}  - \negl(\secpar)
\label[Inequality]{claim:bound:K''1:proof:1:pq}\\
 & \ge 
\Pr[w' = (i,\tilde{x}_i):\Val \gets \mcal{K}'_i({\msf{pref}})]  {\color{red}-\epsilon_\wiaok(\secpar)}- \negl(\secpar) 
\label[Inequality]{claim:bound:K''1:proof:2:pq}\\
 & \ge 
\frac{1}{t}\cdot\Pr[w' = (i,\tilde{x}_i):\Val \gets \mcal{K}_i({\msf{pref}})] {\color{red}-\epsilon_\wiaok(\secpar)} - \negl(\secpar) 
\label[Inequality]{claim:bound:K''1:proof:3:pq}\\
& \ge 
\frac{1}{t} \cdot \big(p_{\msf{pref}} {\color{red}-2\epsilon_\wiaok(\secpar)} -\epsilon'(\secpar)\big) {\color{red}-\epsilon_\wiaok(\secpar)}- \negl(\secpar), \label[Inequality]{claim:bound:K''1:proof:4:pq}
\end{align}
where \Cref{claim:bound:K''1:proof:1:pq} follows from \Cref{eq:relation:K:WI:pq}, \Cref{claim:bound:K''1:proof:2:pq} follows from \Cref{eq:relation:K'-K'':pq}, \Cref{claim:bound:K''1:proof:3:pq} follows from \Cref{eq:bound:K'i:pq}, and \Cref{claim:bound:K''1:proof:4:pq} follows from \Cref{claim:bound:Ki-xi:pq}.

\end{proof}

Now, we show the last claim which, together with \Cref{claim:bound:K''1:pq}, will lead to the desired contradiction.
\begin{MyClaim}\label{claim:K'':non-abort:pq}
$\Pr[\Val \ne \bot_{\msf{invalid}}:\Val \gets \mcal{K}''_1({\msf{pref}})] \le p_{\msf{pref}}{\color{red} +2\epsilon_\wiaok(\secpar)} + \negl(\secpar)$.
\end{MyClaim}
\para{Deriving the Contradiction.} Before proving \Cref{claim:K'':non-abort:pq}, we first show why \Cref{claim:bound:K''1:pq,claim:K'':non-abort:pq} are contradictory. In the following, all the probabilities are taken over $\Val \gets \mcal{K}''_1({\msf{pref}})$:
\begin{align*}
\Pr[\Val \ne \bot_{\msf{invalid}}] 
& = \Pr[\Val = \msf{val}(\tilde{\tau})]  + \Pr[\Val = \bot_{\tilde{Y}}] \\
& = \Pr[\Val = \msf{val}(\tilde{\tau})] + \sum_{i =1 }^{\tilde{t}} \Pr[w' = (i,\tilde{x}_i)] \numberthis \label{eq:bound:Ki:final-contradiction:0:pq}\\
& \ge  \sum_{i =1 }^{\tilde{t}} \Pr[w' = (i,\tilde{x}_i)] \\
&\ge \tilde{t} \cdot \frac{1}{t} \cdot \big(p_{\msf{pref}}{\color{red}-(t+2)\epsilon_\wiaok(\secpar)} - \epsilon'(\secpar)\big) - \negl(\secpar) \numberthis \label[Inequality]{eq:bound:Ki:final-contradiction:1:pq}\\
& \ge (1+\frac{1}{t}) \cdot (p_{\msf{pref}}{\color{red}-(t+2)\epsilon_\wiaok(\secpar)} - \epsilon'(\secpar)) - \negl(\secpar) \numberthis \label[Inequality]{eq:bound:Ki:final-contradiction:2:pq}\\
& = (1+\frac{1}{t}) \cdot \bigg(p_{\msf{pref}}{\color{red}-\frac{t^2+5t+2}{t+1}\cdot\epsilon_\wiaok(\secpar)} - \epsilon'(\secpar)\bigg){\color{red}+ 2\epsilon_\wiaok(\secpar)} - \negl(\secpar) \\
& = (1+\frac{1}{t}) \cdot \bigg(p_{\msf{pref}}{\color{red}- 2\epsilon'(\secpar)}\bigg){\color{red}+ 2\epsilon_\wiaok(\secpar)} - \negl(\secpar) \numberthis \label{eq:bound:Ki:final-contradiction:2.5:pq}\\
& = p_{\msf{pref}}{\color{red}+ 2\epsilon_\wiaok(\secpar)} + \bigg(\frac{p_{\msf{pref}}}{t} {\color{red}- 2\epsilon'(\secpar) - \frac{2\epsilon'(\secpar)}{t}}\bigg) - \negl(\secpar)\\
& \ge p_{\msf{pref}}{\color{red}+ 2\epsilon_\wiaok(\secpar) + \frac{5t^2 - t -1}{5t^3}\cdot \epsilon(\secpar)} - \negl(\secpar) \numberthis \label[Inequality]{eq:bound:Ki:final-contradiction:3:pq}\\
\end{align*}
where \Cref{eq:bound:Ki:final-contradiction:0:pq} follows from \Cref{eq:bot-tilde-Y:partition:pq}, \Cref{eq:bound:Ki:final-contradiction:1:pq} follows from \Cref{claim:bound:K''1:pq}, \Cref{eq:bound:Ki:final-contradiction:2:pq} follows from the assumption that $\tilde{t} \ge t+1$, 
{\color{red} \Cref{eq:bound:Ki:final-contradiction:2.5:pq} follows from our parameter setting $\epsilon_\wiaok(\secpar)=\frac{t+1}{t^2+5t+2}\cdot \epsilon'(\secpar)$,} and
\Cref{eq:bound:Ki:final-contradiction:3:pq} follows from the assumption that $p_{\msf{pref}} \ge \epsilon(\secpar)$ and our parameter setting $\epsilon'(\secpar) = \frac{\epsilon(\secpar)}{10t^2}$.

Recall that $t$ is the tag taking values from $[2n]$ with $n$ being a polynomial of $\secpar$. Also recall that $\epsilon(\secpar)$ is an inverse polynomial on $\secpar$. Therefore, \Cref{eq:bound:Ki:final-contradiction:3:pq} can be written as:
$$\Pr[\Val \ne \bot_{\msf{invalid}}:\Val \gets \mcal{K}''_1({\msf{pref}})] \ge p_{\msf{pref}} {\color{red}+ 2\epsilon_\wiaok(\secpar)}+ \frac{1}{\poly(\secpar)} - \negl(\secpar),$$
which contradicts \Cref{claim:K'':non-abort:pq}.

This eventually finishes the proof of \Cref{lem:bound:Ki:pq} (modulo the proof of \Cref{claim:K'':non-abort:pq} which we will show next).



\begin{proof}[Proof of {\Cref{claim:K'':non-abort:pq}}]
We first define two extra machines $\mcal{K}^{**}_1$ and $\mcal{K}^*_1$.

\takashi{@Xiao Can I ask you to replace WIPoK with WIAoK in \Cref{figure:one-sided:K**1-K*1:pq}
?}

\para{Machine $\mcal{K}^{**}_1$:} (Illustrated in \Cref{figure:one-sided:K**i:pq}.) On input a prefix $\msf{pref}$, $\mcal{K}^{**}_1(\msf{pref})$ behaves identically as $\mcal{K}''_1(\msf{pref})$ except that $\mcal{K}^{**}_1(\msf{pref})$ finishes the right {\bf WIAoK-2} using the honest receiver's algorithm, instead of using the witness-extended emulator. 

\subpara{$\mcal{K}^{**}_1$'s Output.} We define the output of $\mcal{K}^{**}_1(\msf{pref})$ to be the honest receiver's decision $b \in \Set{\top, \bot}$. This is in contrast to previous hybrids (i.e., $\mcal{K}'_i(\msf{pref})$, $\mcal{K}''_i(\msf{pref})$, and $\mcal{K}_i(\msf{pref})$, whose output is defined to be the value $\msf{Val}$ that depends on the value $w'$ extracted by the $\mcal{SE}$ for the right {\bf WIAoK-2}.

 By the witness-extended $\epsilon_\wiaok$-close emulation property (as per \Cref{item:PQWEE} of \Cref{def:PQWIAoK}), it holds that
\begin{equation}\label[Inequality]{eq:K''1-K**1:pq}
\big|\Pr[\Val \ne \bot_{\msf{invalid}} :\Val\gets \mcal{K}''_1(\msf{pref})] - \Pr[b = \top : b\gets \mcal{K}^{**}_1(\msf{pref})] \big| \le {\color{red} \epsilon_\wiaok(\secpar)} + \negl(\secpar).
\end{equation}

\para{Machine $\mcal{K}^{*}_1$:} (Illustrated in \Cref{figure:one-sided:K*i:pq}.) On input a prefix $\msf{pref}$, $\mcal{K}^{*}_1({\msf{pref}})$ behaves identically as $\mcal{K}^{**}_1({\msf{pref}})$ except for the witness used in the left {\bf WIAoK-2}: $\mcal{K}^{*}_1({\msf{pref}})$ use the $(m, r)$ used to generated $\com = \Com_\gamma(m;r)$ as the witness to finish the left {\bf WIAoK-2}. (Note that this witness pair $(m,r)$ must be contained in ${\msf{pref}}$---because ${\msf{pref}}$ is corresponding to the first two steps of the man-in-the-middle execution, and the left execution is done by the honest committer.) It is worth noting that machine $\mcal{K}^*_1$ is actually identical to the machine $\mcal{G}_1$ we defined on \Cpageref{machine:Gi:pq}. Therefore, it holds that
\begin{equation}\label{eq:K*1-G1:pq}
\Pr[b^* = \top: b^* \gets \mcal{K}^{*}_1(\msf{pref})] = \Pr[ b_{\mcal{G}_1}=\top:(\OUT_{\mcal{G}_1}, b_{\mcal{G}_1})\gets \mcal{G}_1(\msf{pref})] = p_{\msf{pref}}, 
\end{equation}
where the last equivalence follows by definition (see \Cref{def:p-tau:2:pq}).

\begin{figure}[!tb]
     \begin{subfigure}[t]{0.47\textwidth}
         \centering
         \fbox{
         \includegraphics[width=\textwidth,page=9]{figures/figures.pdf}
         }
         \caption{}
         \label{figure:one-sided:K**i:pq}
     \end{subfigure}
     \hspace{6.5pt}
     \begin{subfigure}[t]{0.47\textwidth}
         \centering
         \fbox{
         \includegraphics[width=\textwidth,page=10]{figures/figures.pdf}
         }
         \caption{}
         \label{figure:one-sided:K*i:pq}
     \end{subfigure}
     \caption{Machines $\mcal{K}^{**}_1(\msf{pref})$ and $\mcal{K}^*_1(\msf{pref})$ \scriptsize{(Changes between adjacent machines are highlighted by red color)}}
     \label{figure:one-sided:K**1-K*1:pq}
\end{figure}

Next, let us recall the witness used by $\mcal{K}^{**}_1$ for the left {\bf WIAoK-2}. By definition, machine $\mcal{K}^{**}_1(\msf{pref})$ performs brute-force to extract $(x_1, \ldots, x_t)$,\footnote{This brute-forcing was there starting from $\mcal{K}'_1$ (defined on \Cpageref{machineK':description:pq}), and was inherited by $\mcal{K}''_1$, $\mcal{K}^{**}_1$, and eventually by $\mcal{K}^{*}_1$.} and samples a random {\em good}\footnote{Recall from \Cref{item:machineK':3:pq}
 of $\mcal{K}'_i(\msf{pref})$ (\Cpageref{machineK':description:pq}) that ``good'' means that $x^*_j$ is a valid pre-image of $y_j$.} $x^*_j$ as the witness to go through the left {\bf WIAoK-2}. 
 %In summary, the only difference between $\mcal{K}^{*}_1$ and $\mcal{K}^{**}_1$ is the witness used in the left {\bf WIAoK-2}.\takashi{If I understand correctly, another difference occurs when none of $y_j$ has a preimage but the adversary somehow passes the verification in the left {\bf WIAoK-1}.(If I understand correctly, these extractors run the verifier of the the left {\bf WIAoK-1} honestly instead of running the extractor.) So, should we also rely on the soundness of {\bf WIAoK-1} here?}
% Also, note that neither $\mcal{K}^{*}_1$ nor $\mcal{K}^{**}_1$ rewinds the {\bf WIAoK-2} because we already get rid of the witness-extended emulation starting from $\mcal{K}^{**}_1$. 
Thus, there are the following two differences between $\mcal{K}^{*}_1$ and $\mcal{K}^{**}_1$:
 \begin{enumerate}
\item If the left {\bf WIAoK-1} accepts and there is at least one $j$ such that $y_j$ has a preimage, they use different witnesses in the left {\bf WIAoK-2};
\item If the left {\bf WIAoK-1} accepts and there is \emph{no} $j$ such that $y_j$ has a preimage, $\mcal{K}^{**}_1$ aborts whereas $\mcal{K}^{*}_1$ does not.  
 \end{enumerate}
It is easy to see that the second case occurs with probability {\color{red} at most $\epsilon_\wiaok(\secpar)$} by the witness-extended $\epsilon_\wiaok$-close emulation property of the left {\bf WIAoK-1}.  
For the first case, we note that neither $\mcal{K}^{*}_1$ nor $\mcal{K}^{**}_1$ rewinds the {\bf WIAoK-2} because we already get rid of the witness-extended emulation starting from $\mcal{K}^{**}_1$. 
Therefore, 
by the (non-uniform) WI property of the left {\bf WIAoK-2}, it holds that
\begin{equation}\label[Inequality]{eq:K**1-K*1:pq}
\big|\Pr[b = \top : b \gets \mcal{K}^{**}_1({\msf{pref}})] - \Pr[b^* = \top : b^* \gets \mcal{K}^{*}_1({\msf{pref}})] \big| \le {\color{red} \epsilon_\wiaok(\secpar)}+ \negl(\secpar).
\end{equation}
Therefore, the following holds:

\begin{align}
\Pr[\Val \ne \bot_{\msf{invalid}} :\Val\gets \mcal{K}''_1({\msf{pref}})] & \le \Pr[b = \top : b\gets \mcal{K}^{**}_1(\msf{pref})]\le {\color{red} +\epsilon_\wiaok(\secpar)} +  \negl(\secpar) \label[Inequality]{eq:K'':non-abort:final:1:pq} \\
& \le \Pr[b^* = \top : b^* \gets \mcal{K}^{*}_1({\msf{pref}})] \le {\color{red} +2\epsilon_\wiaok(\secpar)}+ \negl(\secpar) \label[Inequality]{eq:K'':non-abort:final:2:pq} \\
& = p_{\msf{pref}} {\color{red} +2\epsilon_\wiaok(\secpar)}+ \negl(\secpar), \label{eq:K'':non-abort:final:3:pq}
\end{align}
where \Cref{eq:K'':non-abort:final:1:pq} follows from \Cref{eq:K''1-K**1:pq}, \Cref{eq:K'':non-abort:final:2:pq} follows from \Cref{eq:K**1-K*1:pq}, and \Cref{eq:K'':non-abort:final:3:pq} follows from \Cref{eq:K*1-G1:pq}. 

This finishes the proof of \Cref{claim:K'':non-abort:pq}.
\end{proof}



\if0
\UpdateLine

\xiao{@Takashi: Everything below this red line is not up to date. They are old stuff before I finished the new version of \Cref{sec:small-tag-one-sided-sync-classical}. So, you may find they are not consistent in terms of notation and logic flow from their classical counterpart i.e.,  \Cref{sec:small-tag-one-sided-sync-classical}. Since you anyway will redo this part, feel free to delete these old stuff.}

We now prove \Cref{lem:one-sided:pq:proof:core:} by constructing the machine $G$ prescribed in \Cref{lem:one-sided:pq:proof:core:} and proving that it satisfies the required properties. At a high-level, $G$ works similarly as the $G^{\mcal{M}}$ presented in \Cref{hybrid:G}. \xiao{Talk about their difference. In particular, stress that we will use the extraction-simulator from \Cref{lem:extract_and_simulate}.}

% We present the formal description of $G$ in \Cref{hybrid:G:pq}.
% \begin{AlgorithmBox}[label={hybrid:G:pq}]{Hybrid \textnormal{$G^{\mcal{M}_\secpar}(m,\rho_\secpar)$}}
% This hybrid proceeds as follows:
% \begin{enumerate}
% \item
% It finishes the first two steps of \Cref{prot:one-sided:classical} identically as $H^{\mcal{M}_\secpar}(m, \rho_\secpar)$. Formally, $G^{\mcal{M}_\secpar}(m,\rho_\secpar)$ emulates \Cref{item:one-sided:pq:step:Naor-rho,item:one-sided:pq:step:committing} of the man-in-the-middle game of \Cref{prot:one-sided:classical}, where it plays as the honest committer in the left committing to $m$ and the honest receiver in the right session, with $\mcal{M}_\secpar(\rho_\secpar)$ being the man-in-the-middle adversary.

% \subpara{Notation:} Let $\rho'_\secpar$ denote the quantum state of $\mcal{M}_\secpar$ at the end of \Cref{item:one-sided:pq:step:committing}. Let $\tau$ denote the tuple $(\tilde{\gamma}, \tilde{\msf{com}})$. Recall that $\tilde{\gamma}$ and  $\tilde{\msf{com}}$ are the \Cref{item:one-sided:pq:step:Naor-rho,item:one-sided:pq:step:committing} messages in the right session; they constitutes an execution of Naor's commitment.

% \item
% \red{need to mention the existance of the simulation-extractor $\mcal{SE}$ prescribed in \Cref{lem:extract_and_simulate}.}
% This hybrid then invoke the simulation-extractor $\mcal{SE}$ guaranteed by \red{Cref to the proper lemma}, which takes as input $(1^\secpar, \red{1^{\epsilon}}, \tau)$ and uses $\mcal{M_\secpar}(\rho'_\secpar)$ as the oracle. 

% \subpara{Notation:} we denote this step by $\big(\OUT_{\mcal{SE}}, \msf{Val}_{\mcal{SE}}\big) \gets \mcal{SE}^{\mcal{M}_\secpar(\rho'_\secpar)}(1^\secpar, \red{1^{\epsilon}}, \tau)$.

% \item
% $G^{\mcal{M}_\secpar}(m,\rho_\secpar)$ simply sets $\OUT_{G}\coloneqq \OUT_{\mcal{SE}}$ and $ \msf{Val}_{G}\coloneqq \msf{Val}_{\mcal{SE}}$, and outputs $(\OUT_{G}, \msf{Val}_{G})$.
% \end{enumerate}
% \end{AlgorithmBox}



In \Cref{hybrid:H:pq:reinterpretation}, we provide a new but equivalent interpretation of the game $H^{\mcal{M}_\secpar}(m,\rho_\secpar)$.
\begin{AlgorithmBox}[label={hybrid:H:pq:reinterpretation}]{Re-interpretation of Game \textnormal{$H^{\mcal{M}_\secpar}(m,\rho_\secpar)$}}
Game $H^{\mcal{M}_\secpar}(m,\rho_\secpar)$ can be split into the following stages:
\begin{enumerate}
\item \label[Stage]{hybrid:H:pq:reinterpretation:1}
{\bf Prefix Generation:}
First, execute \Cref{item:one-sided:pq:step:Naor-rho,item:one-sided:pq:step:committing} of the man-in-the-middle game of \Cref{prot:one-sided:classical}---it plays as the honest committer in the left committing to $m$ and the honest receiver in the right session, with $\mcal{M}_\secpar(\rho_\secpar)$ being the man-in-the-middle adversary.

\subpara{Notation:} Let $\rho'_\secpar$ denote the quantum state of $\mcal{M}_\secpar$ at the end of \Cref{item:one-sided:pq:step:committing}; let $\msf{st}_C$  (resp.\ $\msf{st}_R$) denote the state of the honest committer (resp.\ receiver) at the end of \Cref{item:one-sided:pq:step:committing}; let $\tau$ denote the tuple $(\tilde{\gamma}, \tilde{\msf{com}})$\footnote{Recall that $\tilde{\gamma}$ and  $\tilde{\msf{com}}$ are the \Cref{item:one-sided:pq:step:Naor-rho,item:one-sided:pq:step:committing} messages in the right session; they constitutes an execution of Naor's commitment.}. In terms of notation, we denote the execution of this stage by 
\begin{equation}\label[Expression]{expression:hybrid:H:pq:prefix}
(\rho'_\secpar,  \msf{st}_C, \msf{st}_R, \tau)\getsH^{\mcal{M}_\secpar}_{\msf{pre}}(m,\rho_\secpar).
\end{equation}

\item \label[Stage]{stage:hybrid:H:pq:remainder}
{\bf The Remainder:}
Next, it simply resumes from where the {\bf Prefix Generation} stage stops, to finish the remaining steps of the man-in-the-middle execution $H^{\mcal{M}_\secpar}(m,\rho_\secpar)$.

\subpara{Notation.} We introduce the following notation to captures this step. Define a QPT machine $\Adv$ that takes as input $(\rho'_\secpar, \tau)$; machine $\mcal{A}$ is supposed to run the residual strategy of $\mcal{M}_\secpar$ starting from $\rho'_\secpar$. Also, define a PPT machine $\mcal{B}$ that takes as input $(\msf{st}_C, \msf{st}_R, \tau)$; machine $\mcal{B}$ is supposed to run the residual strategies of the honest committer $C$ and receiver $R$, starting from 
$\msf{st}_C$ and $\msf{st}_R$ respectively\footnote{Note that it is not necessary to give $\tau$ as common input to these parties; indeed, it can be included in their respective internal states. We choose to make $\tau$ explicit only to match the syntax of \Cref{lem:extract_and_simulate}.}. With the above notations, we can denote the execution of the remainder steps of $H^{\mcal{M}_\secpar}(m,\rho_\secpar)$ by
\begin{equation}\label[Expression]{expression:hybrid:H:pq:remainder}
(\OUT_\mcal{A}, b)\gets \langle \mcal{A}(\rho'_\secpar), \mcal{B}(\msf{st}_C, \msf{st}_R) \rangle(1^\secpar, \tau),
\end{equation}
where $\OUT_\mcal{A}$ is the output of $\mcal{A}$, and $b \in \Set{\bot, \top}$ is the output of the honest receiver $R$ (in the right), indicating if the man-in-the-middle's commitment (i.e., the right session) is accepted ($b = \top$) or not ($b = \bot$).
\item
{\bf Output:} It sets $\OUT_{H} \coloneqq \OUT_\mcal{A}$ and sets $\msf{trans}$ to the transcript of the right session. In particular, $\msf{trans}$ includes the $b$ defined in \Cref{expression:hybrid:H:pq:remainder}, indicating if the honest receiver accepts or not. It outputs $(\OUT_{H}, \msf{trans})$.  
\end{enumerate}
\end{AlgorithmBox}

\xiao{Say that this is the major lemma for this proof. It is the quantum counterpart of lemma XXX in the classical case...}
\begin{lemma}\label{lem:small-tag:pq:proof:sim-less}
There exists a QPT algorithm $\ext_{\simless}$ such that for machines $\mcal{A}$ and $\mcal{B}$ defined in \Cref{stage:hybrid:H:pq:remainder} of \Cref{hybrid:H:pq:reinterpretation}, for any tuple $(\rho'_\secpar, \msf{st}_C, \msf{st}_R, \tau)$ in the support of $H^{\mcal{M}_\secpar}_{\msf{pre}}(m,\rho_\secpar)$ (defined in \Cref{expression:hybrid:H:pq:prefix}), the following requirements are satisfies:
\begin{enumerate}
\item {\bf (Syntax.)}
$\ext_{\simless}$ takes as input the security parameter $1^\secpar$ and the commitment $\tau$, accesses $\Adv(\rho'_\secpar)$ as an oracle, and outputs a string $\msf{Val}$. We denote this procedure by $\msf{Val} \gets \ext_{\simless}^{\Adv(\rho'_\secpar)}(1^\secpar, \tau)$.
\item 
if $\Pr[b = \top: (\OUT_\Adv, b) \leftarrow \langle\A(\rho'_\secpar),\mcal{B}(\msf{st}_C, \msf{st}_R) \rangle(1^\secpar,\tau)]\geq  \delta(\secpar)$, then it holds that
$$
\Pr[\msf{Val}=\val(\tau): \msf{Val} \gets \ext_{\simless}^{\Adv(\rho'_\secpar)}(1^\secpar, \tau)]\geq  \delta'(\secpar).
$$
\xiao{set $\delta'(\secpar)$ properly.}
\end{enumerate}
\end{lemma}
\xiao{Say that \Cref{lem:small-tag:pq:proof:sim-less} is the main technical lemma for the current proof of \Cref{item:lem:one-sided:pq:proof:core::2}. We present its proof in \Cref{sec:lem:small-tag:pq:proof:sim-less:proof}. In the following, we finish the proof of \Cref{item:lem:one-sided:pq:proof:core::2} assuming that \Cref{lem:small-tag:pq:proof:sim-less} is true.}

Combining \Cref{lem:extract_and_simulate,lem:small-tag:pq:proof:sim-less}, we obtain immediately the following  \Cref{cor:small-tag:pq:proof:sim}.

\begin{corollary}\label{cor:small-tag:pq:proof:sim} 
Let $(\Adv, \mcal{B}, \rho'_\secpar, \msf{st}_C, \msf{st}_R, \tau)$ be the same as in \Cref{hybrid:H:pq:reinterpretation}. Then, there exists an efficiently constructible QPT (oracle) algorithm $\SimExt$ such that for any noticeable $\epsilon(\secpar)$, it holds that 
$$
\big\{\SimExt^{\A(\rho'_\secpar)}(1^\secpar,1^{\epsilon^{-1}},\tau)\big\}_{\secpar \in \Naturals}
\statind_{\epsilon} 
\big\{\big(\OUT_{\mcal{A}},\val_b(\tau)\big): (\OUT_\Adv, b) \leftarrow \langle\A(\rho'_\secpar),\mcal{B}(\msf{st}_C, \msf{st}_R) \rangle(1^\secpar,\tau) \big\}_{\secpar \in \Naturals},
$$
where 
$
\val_b(\tau)\defeq 
\begin{cases}
\val(\tau) & \text{if}~ b=\top \\
\bot & \text{otherwise}
\end{cases}
$.
\end{corollary}

Now, we are ready to present the description of $G$.
\begin{AlgorithmBox}[label={hybrid:G:pq}]{Hybrid \textnormal{$G^{\mcal{M}_\secpar}(m,\rho_\secpar)$}}
This hybrid proceeds as follows:
\begin{enumerate}
\item
{\bf Prefix Generation:}
This stage is identical to \Cref{hybrid:H:pq:reinterpretation:1} of $H^{\mcal{M}_\secpar}(m,\rho_\secpar)$. Formally, it executes 
$$(\rho'_\secpar,  \msf{st}_C, \msf{st}_R, \tau)\getsH^{\mcal{M}_\secpar}_{\msf{pre}}(m,\rho_\secpar),$$
where $H^{\mcal{M}_\secpar}_{\msf{pre}}(m,\rho_\secpar)$ is defined in \Cref{hybrid:H:pq:reinterpretation:1} of \Cref{hybrid:H:pq:reinterpretation}.
\item
{\bf The Remainder:}
Define $\mcal{A}$ in the same way as in \Cref{stage:hybrid:H:pq:remainder} of $H^{\mcal{M}_\secpar}(m,\rho_\secpar)$. With this $\mcal{A}$  and the $(\rho'_\secpar,  \msf{st}_C, \msf{st}_R, \tau)$ from the previous stage, $G^{\mcal{M}_\secpar}(m,\rho_\secpar)$ invokes the $\mcal{SE}$ prescribed in \Cref{cor:small-tag:pq:proof:sim}. Formally, it does the following:
$$(\OUT_{\mcal{SE}}, \msf{Val}_{\mcal{SE}}) \gets \SimExt^{\A(\rho'_\secpar)}(1^\secpar,1^{\delta^{-1}},\tau),$$
where the $\delta$ is the statistical distance that we want to show for \Cref{item:lem:one-sided:pq:proof:core::2} of \Cref{lem:one-sided:pq:proof:core:}.

\item
{\bf Output:}
% $G^{\mcal{M}_\secpar}(m,\rho_\secpar)$ sets $\OUT_{G}\coloneqq \OUT_{\mcal{SE}}$ and $ \msf{Val}_{G}\coloneqq \msf{Val}_{\mcal{SE}}$, and 
It outputs $(\OUT_{\mcal{SE}}, \msf{Val}_{\mcal{SE}})$.
\end{enumerate}
\end{AlgorithmBox}

\para{Proving \Cref{item:lem:one-sided:pq:proof:core::1} of \Cref{lem:one-sided:pq:proof:core:}.} This part is similar to its classical counterpart, i.e., the ``{\bf Proving \Cref{item:lem:one-sided:proof:core:1} in \Cref{lem:one-sided:proof:core}}'' on \Cpageref{para:lem:one-sided:proof:core:1}. Observe that hybrid $G^{\mcal{M}_\secpar}(m,\rho_\secpar)$ is an efficient machine. \xiao{(this makes use of \Cref{item:extractorK:efficiency} in \Cref{lem:extractorK}) need to modify}. Moreover, it does not rewind \Cref{item:one-sided:pq:step:Naor-rho,item:one-sided:pq:step:committing} of the man-in-the-middle execution. Therefore, \Cref{item:lem:one-sided:pq:proof:core::1} of \Cref{lem:one-sided:pq:proof:core:} follows immediately from the computationally-hiding property of the left Naor's commitment (i.e., \Cref{item:one-sided:pq:step:Naor-rho,item:one-sided:pq:step:committing} in the left execution).

Then, to finish the proof of \Cref{lem:one-sided:pq:proof:core:}, we only need to prove \Cref{item:lem:one-sided:pq:proof:core::2}.


\para{Proving \Cref{item:lem:one-sided:pq:proof:core::2} of \Cref{lem:one-sided:pq:proof:core:}.} This part is similar to its classical counterpart, i.e., the ``{\bf Proving \Cref{item:lem:one-sided:proof:core:2} in \Cref{lem:one-sided:proof:core}}'' on \Cpageref{para:lem:one-sided:proof:core:2}. First, observe that $G^{\mcal{M}_\secpar}(m,\rho_\secpar)$ and $H^{\mcal{M}_\secpar}(m, \rho_\secpar)$ (as per \Cref{hybrid:H:pq:reinterpretation}) are identical up to the end of \Cref{item:one-sided:pq:step:committing} of the man-in-the-middle game of \Cref{prot:one-sided:classical}. \xiao{Say that this follows immediately from \Cref{cor:small-tag:pq:proof:sim}.}



\subsection{Proof of \Cref{lem:small-tag:pq:proof:sim-less}}
\label{sec:lem:small-tag:pq:proof:sim-less:proof}

\xiao{To do...}

\UpdateLine
\fi


==> sections/old-stuff.tex <==

\subsection{Extractor $\mcal{K}$ (Proof of \Cref{lem:extractorK})}
\label{sec:lem:extractorK:proof}

\para{Machine $\mcal{G}_{i}$ ($i \in [\tilde{t}]$):}\label{machine:Gi}
\xiao{We can interpret $H^{\mcal{M}}(\secpar,m,z)$ as first generating prefix $\tau$, then running $\mcal{G}_1(\tau)$. At the end, $\mcal{G}_1(\tau)$ outputs the view of $\mcal{M}$. The subscript $i$ indicates that the witness $\tilde{x}_1$ is used in the right {\bf WIPoK-1}. Then, for any $\tau$, $\mcal{G}_{i}(\tau)$ is defined as machine that is identical to $\mcal{G}_1(\tau)$ except that the witness $\tilde{x}_{i}$ is used in the right {\bf WIPoK-1}.}

\begin{xiaoenv}{}
For any $\tau$ that corresponds to the first 2 steps of the execution $H^{\mcal{M}}(\secpar,m,z)$, we define
\begin{equation}\label{eq:def:p-tau}
p_\tau \coloneqq \Pr[\View~\text{is accepting}: \View \gets \mcal{G}_1(\tau)].
\end{equation}
\end{xiaoenv}

\xiao{In the following, we need a noticeable function $\epsilon(\secpar)$. Will fix it later.}

\begin{MyClaim}\label{claim:bound:Gi}
% For any $\tau$, if $p_\tau \ge \epsilon(\secpar)$, then it holds that  
$\forall i \in [\tilde{t}], ~\Pr[\View~\text{is accepting}:\View \gets \mcal{G}_i(\tau)] \ge p_\tau - \negl(\secpar)$.
\end{MyClaim}
\begin{proof}
\xiao{This follows immediately from the WI property of the right {\bf WIPoK-1}.}
\end{proof}

\para{Machine $\mcal{G}'_i$ ($i\in [\tilde{t}]$):} On any input $\tau$, $\mcal{G}'_i(\tau)$ behaves identically to $\mcal{G}_i(\tau)$, except the following change. Instead of executing \Cref{item:one-sided:step:WIPoK:1} in the left honestly, $H_1$ invokes the emulation-extractor $\mcal{E}$ to simulate the \Cref{item:one-sided:step:WIPoK:1} transcript $\mcal{T}$ while extracting a value $(j, x_j)$. Recall that the existence of $\mcal{E}$ is guaranteed by the PoK property of $\WIPoK$ (see \Cref{def:WEE}). If  $(j, x_j) \notin \Relation_{\Lang^t_f}(Y)$ (see \Cref{eq:one-sided:Lang:OWF}), $\mcal{G}'_i(\tau)$ aborts; otherwise, $H_1$ continues to finish the execution as $\mcal{G}_i(\tau)$. It is worth noting that although $\mcal{E}$ may extract a valid $(j, x_j)$ pair, $\mcal{G}'_i(\tau)$ does not use this pair.  

\begin{MyClaim}\label{claim:bound:G'i}
% For any $\tau$, if $p_\tau \ge \epsilon(\secpar)$, then it holds that  
$\forall i \in [\tilde{t}], ~\Pr[\View~\text{is accepting}:\View \gets \mcal{G}'_i(\tau)] \ge p_\tau - \negl(\secpar)$.
\end{MyClaim}
\begin{proof}
\xiao{The claim follows immediately from \Cref{claim:bound:Gi} and the witness-extended emulation property of the left {\bf WIPoK-1}.}
\end{proof}

\para{Machine $\mcal{G}''_i$ ($i\in [\tilde{t}]$):} On any input $\tau$, $\mcal{G}''_i(\tau)$ behaves identically to $\mcal{G}'_i(\tau)$, except that $\mcal{G}''_i(\tau)$ use the $(j, x_j)$ (extracted in $\mcal{G}'_i(\tau)$) to finish the left {\bf WIPoK-2} (i.e., \Cref{item:one-sided:step:WIPoK:2} in the left execution).

\begin{MyClaim}\label{claim:bound:G''i}
% For any $\tau$, if $p_\tau \ge \epsilon(\secpar)$, then it holds that  
$\forall i \in [\tilde{t}], ~\Pr[\View~\text{is accepting}:\View \gets \mcal{G}''_i(\tau)] \ge p_\tau - \negl(\secpar)$.
\end{MyClaim}
\begin{proof}
\xiao{The claim follows immediately from \Cref{claim:bound:G'i} and the WI property of the left {\bf WIPoK-2}.}
\end{proof}

\para{Machine $\mcal{K}_i$ ($i\in [\tilde{t}]$):} On any input $\tau$, $\mcal{K}_i(\tau)$ behaves identically to $\mcal{G}''_i(\tau)$, except for the following difference. Machine $\mcal{K}_i(\tau)$ uses the witness-extended emulator $\SimExt$ to finish the right {\bf WIPoK-2}, instead of playing the role of the honest receiver. Let $\Val$ denote the witness extracted by $\SimExt$. We use $\Val = \bot$ to denote the situation where $\Val$ is not a valid witness for the statement $\big(\tilde{com}, (\tilde{y}_1, \ldots, \tilde{y}_{\tilde{t}})\big)$. (Recall that  $\big(\tilde{\com}, (\tilde{y}_1, \ldots, \tilde{y}_{\tilde{t}})\big)$ is supposed to be an instance in the language $\Lang_{\tilde{\rho}} \vee \Lang^{\tilde{t}}_{\tilde{f}}$.) %If $\Val = \bot$, $\mcal{K}_i(\tau)$ aborts and outputs a special symbol $\msf{Fail}_{\mcal{K}}$. 
\begin{MyClaim}\label{claim:bound:Ki}
% For any $\tau$, if $p_\tau \ge \epsilon(\secpar)$, then it holds that
$\forall i \in [\tilde{t}], ~\Pr[\Val \ne \bot :\Val \gets \mcal{K}_i(\tau)] \ge p_\tau - \negl(\secpar)$.
\end{MyClaim}
\begin{proof}
\xiao{This claim follows immediately from \Cref{claim:bound:G''i} and the witness-extended emulation property of the right {\bf WIPoK-2}.}
\end{proof}

Next, we define a machine $\mcal{K}$ that can be considered as an average-case machine of $\Set{\mcal{K}_i}_{i\in[\tilde{t}]}$:

\para{Machine $\mcal{K}$:} one any input $\tau$, $\mcal{K}(\tau)$ samples uniformly at random an $i \pick [\tilde{t}]$, executes $\mcal{K}_i(\tau)$, and outputs whatever $\mcal{K}_i(\tau)$ outputs.
\begin{lemma}\label{lem:bound:averageK}
For any $\tau$, if $p_\tau \ge \epsilon(\secpar)$, then it holds that
$$\Pr[\Val = \tilde{m}(\tau) :\Val \gets \mcal{K}(\tau)] \ge \epsilon'(\secpar)/\tilde{t}.$$
\xiao{Need to define $\tilde{m}(\tau)$; also need to specify $\epsilon'$ (w.r.t.\ $\epsilon$)..}
\end{lemma}
\xiao{Say that we postpone the proof of \Cref{lem:bound:averageK} to \Cref{sec:proof:lem:bound:averageK}}

\xiao{Assume \Cref{lem:bound:averageK} is true, finish the proof of non-malleability.}

\subsection{Proof of \Cref{lem:bound:averageK}}
\label{sec:proof:lem:bound:averageK}


To prove \Cref{lem:bound:averageK}, it suffices to show that if $\tau$ satisfying $p_\tau \ge \epsilon(\secpar)$, then there exists an $i \in [\tilde{t}]$ such that $\Pr[\Val = \tilde{m}(\tau) :\Val \gets \mcal{K}_i(\tau)] \ge \epsilon'(\secpar)$.

We assume for contradiction that (for $\tau$ satisfying $p_\tau \ge \epsilon(\secpar)$)
\begin{equation}\label[Inequality]{eq:proof:averageK:contra-assump}
\forall i \in [\tilde{t}], ~\Pr[\Val = \tilde{m}(\tau) :\Val \gets \mcal{K}_i(\tau)] < \epsilon'(\secpar).
\end{equation}

\begin{MyClaim}\label{cliam:bound:Ki-xi}
For any $\tau$, if $p_\tau \ge \epsilon(\secpar)$, then it holds that
$$\forall i \in [\tilde{t}], ~\Pr[\Val = \tilde{x}_i:\Val \gets \mcal{K}_i(\tau)] \ge p_\tau - \epsilon'(\secpar) - \negl(\secpar).$$
\end{MyClaim}
\begin{proof}
\xiao{Follows from \Cref{claim:bound:Ki} and the one-wayness of $\tilde{f}$. Need to expand this argument.}
\end{proof}

\para{Machine $\mcal{K}'_i$ ($i \in [\tilde{t}]$):} On any input $\tau$ that corresponding to the first 2 steps of the man-in-the-middle execution, 
\begin{xiaoenv}{}
Brute force to extract $(x_1, \ldots, x_t)$ from $\tau$. (Note that some $x_i$ may be ``bad''.) Pick a random $x^*_j$. It then finish the execution identically as $\mcal{K}_i$, except that it uses $x^*_j$ as the witness when executing the left {\bf WIPoK-2}.
\end{xiaoenv}
It is worth noting that the $(j, x_j)$ extracted by the witness-extended emulator for the left {\bf WIPoK-1} is not used any more by $\mcal{K}'_i(\tau)$. 

Obviously, if $\mcal{K}'_i(\tau)$ picked the $x^*_j$ that is the same as the $x_j$ extracted by $\mcal{K}_i(\tau)$ from its left {\bf WIPoK-1}, then $\mcal{K}'_i(\tau)$ and $\mcal{K}_i(\tau)$ are identical\footnote{In this step, we rely on the injectiveness of the OWF $f$ in the right. That is, there is a unique preimage for each image. Thus, if both the $x^*j$ (sampled by $\mcal{K}'_i(\tau)$) and the extracted $x_j$ (in $\mcal{K}_i(\tau)$) are a valid preimage for $y_j$, then it must be that $x^*_j = x_j$.}. Since $\mcal{K}'_i(\tau)$ samples $x^*_j$ uniformly, then $x^*_j = x_j$ with probability exactly $1/t$. Therefore, the following must holds: \xiao{double check that we don't need an averaging argument here to fix the preamble before the WIPoK starts...}
\begin{equation}\label[Inequality]{eq:bound:K'i}
\forall i \in [\tilde{t}], ~\Pr[\Val = \tilde{x}_i:\Val \gets \mcal{K}'_i(\tau)] \ge \frac{1}{t}\cdot \Pr[\Val = \tilde{x}_i:\Val \gets \mcal{K}_i(\tau)].
\end{equation}

\para{Machine $\mcal{K}''_i$ ($i\in [\tilde{t}]$):} On any input $\tau$,  $\mcal{K}''_i(\tau)$ behaves identically to $\mcal{K}'_i(\tau)$ except that it plays as the honest committer in the left {\bf WIPoK-1}, instead of running the witness-extended emulator. Recall that starting from $\mcal{K}'_i$, the witness $(j, x_j)$ extracted by the witness-extended emulator for the left {\bf WIPoK-1} is not used any more. Thus, machine $\mcal{K}''_i$ does not need to perform this witness-extended emulation.

By the witness-extended emulation property of the left {\bf WIPoK-1}, it is easy to see that 
\begin{equation}\label[Inequality]{eq:relation:K'-K''}
\forall i \in [\tilde{t}], ~\Pr[\Val = \tilde{x}_i:\Val \gets \mcal{K}''_i(\tau)] \ge \Pr[\Val = \tilde{x}_i:\Val \gets \mcal{K}'_i(\tau)] -\negl(\secpar).
\end{equation}
Moreover, by the WI property of the right {\bf WIPoK-1}, it is easy to see that
\begin{equation}\label[Inequality]{eq:relation:K:WI}
\forall i \in [\tilde{t}], ~\Pr[\Val = \tilde{x}_i:\Val \gets \mcal{K}''_i(\tau)] \ge \Pr[\Val = \tilde{x}_i:\Val \gets \mcal{K}''_1(\tau)] -\negl(\secpar).
\end{equation}

\begin{MyClaim}\label{claim:bound:K''1}
For any $\tau$, if $p_\tau \ge \epsilon(\secpar)$, then it holds that
$$\forall i \in [\tilde{t}], ~\Pr[\Val = \tilde{x}_i:\Val \gets \mcal{K}''_1(\tau)] \ge \frac{1}{t} \cdot \big(p_\tau - \epsilon'(\secpar)\big) - \negl(\secpar).$$
\end{MyClaim}
\begin{proof}
This following immediately from \Cref{cliam:bound:Ki-xi,eq:bound:K'i,eq:relation:K'-K'',eq:relation:K:WI}.
\end{proof}

Now, we show a final claim which, together with \Cref{claim:bound:K''1}, will lead to the desired contradiction.
\begin{MyClaim}\label{claim:K'':non-abort}
%For any $\tau$, if $p_\tau \ge \epsilon(\secpar)$, then it holds that
$\Pr[\Val \ne \bot:\Val \gets \mcal{K}''_1(\tau)] \le p_\tau + \negl(\secpar)$.
\end{MyClaim}
\xiao{Before proving \Cref{claim:K'':non-abort}, we first show why \Cref{claim:bound:K''1,claim:K'':non-abort} are contradicting.}

\begin{proof}[Proof of {\Cref{claim:K'':non-abort}}]
We first define two extra machines $\mcal{K}^*_1$ and $\mcal{K}^{**}_1$.

\para{Machine $\mcal{K}^{**}_1$:} On any input $\tau$, $\mcal{K}^{**}_1(\tau)$ behaves identically as $\mcal{K}''_1(\tau)$ except that $\mcal{K}^{**}_1(\tau)$ finishes the right {\bf WIPoK-2} using the honest receiver's algorithm, instead of using the witness-extended emulator. $\mcal{K}^{**}_1(\tau)$ simply outputs the view of $\mcal{M}$ during the execution. By the witness-extended emulation property, it holds that
\begin{equation}\label{eq:K''1-K**1}
\Pr[\Val \ne \bot :\Val\gets \mcal{K}''_1(\tau)] = \Pr[\View~\text{is accepting}:\View\gets \mcal{K}^{**}_1(\tau)] \pm \negl(\secpar).
\end{equation}


\para{Machine $\mcal{K}^{*}_1$:} On any input $\tau$, $\mcal{K}^{*}_1(\tau)$ behaves identically as $\mcal{K}^{**}_1(\tau)$ except for the witness used in the left {\bf WIPoK-2}: $\mcal{K}^{*}_1(\tau)$ use the $(m, r)$ used to generated $\com = \Com_\rho(m;r)$ as the witness to finish the left {\bf WIPoK-2}. (Note that this witness pair $(m,r)$ must be contained in $\tau$---because $\tau$ is corresponding to the first steps of the man-in-the-middle execution, and the left execution is done by the honest committer.) It is worth noting that machine $\mcal{K}^*_1$ is exactly the machine $\mcal{G}_1$ we defined on \Cpageref{machine:Gi}. Therefore, it follows immediately that
\begin{equation}\label{eq:K*1-G1}
\Pr[\View~\text{is accepting}:\View\gets \mcal{K}^{*}_1(\tau)] = \Pr[\View~\text{is accepting}:\View\gets \mcal{G}_1(\tau)] = p_\tau, 
\end{equation}
where the last equivalence follows by definition (see \Cref{eq:def:p-tau}).

Next, let us recall the witness used by $\mcal{K}^{**}_1$ for the left {\bf WIPoK-2}. Machine $\mcal{K}^{**}_1(\tau)$ performed brute-force to extract $(x_1, \ldots, x_t)$ from $\tau$,\footnote{This brute-forcing is there starting from $\mcal{K}'_1$, and inherited by $\mcal{K}'_1$, $\mcal{K}''_1$, $\mcal{K}^{**}_1$, and eventually by $\mcal{K}^{*}_1$.} and pick a random \xiao{valid} $x_i$ as the witness to go through the left {\bf WIPoK-2}. In summary, the only difference between $\mcal{K}^{*}_1$ and $\mcal{K}^{**}_1$ is the witness used in the left {\bf WIPoK-2}. Also, note that neither $\mcal{K}^{*}_1$ nor $\mcal{K}^{**}_1$ rewinds the {\bf WIPoK-2} because we already get rid of the witness-extended emulation starting from $\mcal{K}^{**}_1$. Therefore, 
by the WI property of the left {\bf WIPoK-2}, it holds that
\begin{equation}\label{eq:K**1-K*1}
\Pr[\View~\text{is accepting}:\View\gets \mcal{K}^{**}_1(\tau)] = \Pr[\View~\text{is accepting}:\View\gets \mcal{K}^{*}_1(\tau)] \pm \negl(\secpar).
\end{equation}
Combining \Cref{eq:K''1-K**1,eq:K*1-G1,eq:K**1-K*1}
$$\Pr[\Val \ne \bot :\Val\gets \mcal{K}''_1(\tau)] = p_\tau \pm \negl(\secpar).$$
This in particular implies the inequality in \Cref{claim:K'':non-abort}.
\end{proof}



\UpdateLine
\xiao{Old Stuff below}

\subsection{Proving Non-Malleability \red{(Old Stuff)}}
\begin{theorem}\label{thm:one-sided:non-malleability}
The commitment scheme $\langle C, R \rangle$ in \Cref{prot:one-sided:classical} is a one-sided non-malleable commitment scheme against synchronous PPT adversaries.
\end{theorem}	
To prove \Cref{thm:one-sided:non-malleability}, we show that
\begin{equation}\label[Expression]{eq:one-sided:goal}
\Set{\msf{mim}^\mcal{M}_{\langle C, R \rangle}(\secpar, m_0, z)}_{\secpar, m_0, m_1, z} \cind \Set{\msf{mim}^\mcal{M}_{\langle C, R \rangle}(\secpar, m_1, z)}_{\secpar, m_0, m_1, z},
\end{equation}
where $\secpar \in \Naturals$, $m_0, m_1 \in \bits^{\secpar}$, and $z \in \bits^*$.

\para{Focusing on Non-Trivial $\mcal{M}$.} \xiao{(This part seems unnecessary. Delete it later)} First, observe that it is easy to establish \Cref{eq:one-sided:goal} if $\mcal{M}$ makes $R$ accept in the man-in-the-middle execution $\msf{mim}^\mcal{M}_{\langle C, R \rangle}(\secpar, m_0, z)$ with negligible probability. This is because:
\begin{enumerate}
\item
by the computationally-hiding property of $\Com$, the probability that $\mcal{M}$ makes $R$ accept in the  execution $\msf{mim}^\mcal{M}_{\langle C, R \rangle}(\secpar, m_1, z)$ must also be negligible; {\bf and}
\item 
when $R$ rejects, $\tilde{m}$ is defined to be $\bot$. 
\end{enumerate} 
Therefore, we only need to focus on $\mcal{M}$ for which $R$ accepts with non-negligible probability. Formally, we assume w.l.o.g.\ that there is a polynomial $p(\secpar)$ and a PPT machine $\mcal{D}$ s.t.\ for infinitely many $\secpar\in \Naturals$, 
\begin{equation}
\left|\Pr[\mcal{D}\left(\msf{mim}^\mcal{M}_{\langle C, R \rangle}(\secpar, m_0, z)\right) = 1] - \Pr[\mcal{D}\left(\msf{mim}^\mcal{M}_{\langle C, R \rangle}(\secpar, m_1, z)\right) = 1] \right|\ge p(\secpar).
\end{equation}
We will refer to such $\mcal{M}$ as a {\em non-trivial} $\mcal{M}$.

% In the remainder of this proof, fix any such generic $\secpar$. \xiao{not sure if this is needed.}

\para{Hybrid Argument.} We will define a sequence of hybrids where the first and the last hybrids are the man-in-the-middle executions corresponding to the LHS and the RHS of \Cref{eq:one-sided:goal} respectively. We will argue that the joint distribution of $\mcal{M}$'s view {\em and} the value $\tilde{m}$ committed by the right execution are computationally indistinguishable between adjacent hybrids. Obviously, this will imply \Cref{eq:one-sided:goal}.

In the following, we define the hybrids. In each hybrid, we use $(\view, \tilde{m})$ to denote the view of $\mcal{M}$ and the value committed by the right execution. In particular, we assume it can be efficiently told from $\view$ if the right-side $R$ rejects or not. If $R$ rejects in $\view$, we define $\tilde{m} \coloneqq \bot$; otherwise, $\tilde{m}$ is defined to be the value statistically-bounded in the $\tilde{\sf{com}}$ in \Cref{item:one-sided:step:committing} of the right execution. \xiao{Is this ok? do we assume public verifiability??}

\subpara{Hybrid $H_0$:} This is the man-in-the-middle execution defined by $\msf{mim}^\mcal{M}_{\langle C, R \rangle}(\secpar, m_0, z)$. 

\subpara{Hybrid $H_1$:} This hybrid is identical to the previous one, except the following change. Instead of executing \Cref{item:one-sided:step:WIPoK:1} in the left honestly, $H_1$ invokes the emulation-extractor $\mcal{E}$ to simulate the \Cref{item:one-sided:step:WIPoK:1} transcript $\mcal{T}$ while extracting a value $(j, x_j)$. Recall that the existence of $\mcal{E}$ is guaranteed by the PoK property of $\WIPoK$ (see \Cref{def:WEE}). If  $(j, x_j) \notin \Relation_{\Lang^t_f}(Y)$ (see \Cref{eq:one-sided:Lang:OWF}), $H_1$ aborts; otherwise, $H_1$ continues to finish the execution as $H_0$. It is worth noting that although $\mcal{E}$ may extract a valid $(j, x_j)$ pair, it is not used in this hybrid. 


\begin{MyClaim}\label{claim:H0-H1}
The distribution of $(\view, \tilde{m})$ in $H_0$ is statistically close to that in $H_1$.
\end{MyClaim}
\begin{proof}
This claim follows directly from the witness-extended emulation property (\Cref{def:WEE}) of $\mcal{E}$, where the negligible error comes from \Cref{item:WEE:2}.% the failure of $\mcal{E}$ to extract a valid witness (when the simulated transcript is accepting). 

\xiao{Need to make a remark: \Cref{def:WEE} only requires emulation of the transcript. It doesn't say that $\mcal{M}$'s internal state can be simulated (such that when we continue the execution of after running $\mcal{E}^{\mcal{M}}$, $\mcal{M}$ will behave identically as in $H_0$). But this is actually true as long as $\mcal{M}$ is a classical machine.}
\end{proof}

\subpara{Hybrid $H_2$:} This hybrid is identical to the previous one, except that $H_2$ use the $(j, x_j)$ (extracted in $H_1$) to finish the \Cref{item:one-sided:step:WIPoK:2} $\WIPoK$ in the left execution.

\begin{MyClaim}\label{claim:H1-H2}
The distribution of $(\view, \tilde{m})$ in $H_1$ is computationally indistinguishable to that in $H_2$.
\end{MyClaim}
\begin{proof}
This claim follows directly from the (non-uniform) WI property of the \Cref{item:one-sided:step:WIPoK:2} $\WIPoK$ in the left execution.

\xiao{In more detail, ...}
\end{proof}

\subpara{Hybrid $H_3$:} This hybrid is identical to the previous one, except that in \Cref{item:one-sided:step:committing} of the left execution, $H_3$ sets (and sends) $\msf{com} =\Com_\rho(m_1;r)$ (instead of $\msf{com} = \Com_\rho(m_0;r)$).
\begin{MyClaim}\label{claim:H2-H3}
The distribution of $(\view, \tilde{m})$ in $H_2$ is computationally indistinguishable to that in $H_3$.
\end{MyClaim}
The proof of \Cref{claim:H2-H3} is the most involved part. We postpone it to \Cref{sec:one-sided:proof:claim:H2-H3}. For now, let us assume that \Cref{claim:H2-H3} is correct and proceed to finish the current proof of \Cref{thm:one-sided:non-malleability}. 


\subpara{Hybrid $H_4$:} This hybrid is identical to the previous one, except that $H_4$ use the $(m_1, r)$ to finish the \Cref{item:one-sided:step:WIPoK:2} $\WIPoK$ in the left execution.
\begin{MyClaim}\label{claim:H3-H4}
The distribution of $(\view, \tilde{m})$ in $H_3$ is computationally indistinguishable to that in $H_4$.
\end{MyClaim}
\begin{proof}
This proof is identical to that of \Cref{claim:H1-H2}. We omit the details.
\end{proof}


\subpara{Hybrid $H_5$:} This is the man-in-the-middle execution defined by $\msf{mim}^\mcal{M}_{\langle C, R \rangle}(\secpar, m_1, z)$. 
\begin{MyClaim}\label{claim:H4-H5}
The distribution of $(\view, \tilde{m})$ in $H_4$ is statistically close to that in $H_5$.
\end{MyClaim}
\begin{proof}
Note that the only difference between $H_4$ and $H_5$ is that $H_5$ does not run the emulation-extractor $\mcal{E}$ to finish \Cref{item:one-sided:step:WIPoK:1} of the left execution; instead, it is using the honest $C$'s algorithm. $H_5$ can do this because starting from $H_4$, we no longer need the $(j, x_j)$ pair extracted by $\mcal{E}$ from \Cref{item:one-sided:step:WIPoK:1} of the left execution. 

Thus, the switch between $H_4$ and $H_5$ is analogous to that between $H_0$ and $H_1$. Similar to the proof of \Cref{claim:H0-H1}, the statistical indistinguishability follows from the witness-extended emulation property (\Cref{def:WEE}) of the \Cref{item:one-sided:step:WIPoK:1} $\WIPoK$.
\end{proof}

Combining \Cref{claim:H0-H1,claim:H1-H2,claim:H2-H3,claim:H3-H4,claim:H4-H5} shows that \Cref{eq:one-sided:goal} holds. This finishes the proof of \Cref{thm:one-sided:non-malleability}.



\subsection{Proof of \Cref{claim:H2-H3} \red{(Old Stuff)}}
\label{sec:one-sided:proof:claim:H2-H3}

\begin{xiaoenv}
May need to define the output of each $H_i$ as $\View_{H_i}$, and the corresponding committed value as $\tilde{m}(\View_{H_i})$. which is defined as: 
\begin{itemize}
\item
If $\View_{H_i}$ is accepting, $\tilde{m}(\View_{H_i})$ is defined to be the value (statistically) committed in \Cref{item:one-sided:step:committing} of the right execution;
Otherwise, $\tilde{m}(\View_{H_i}) \coloneqq \bot$. 
\end{itemize}
\end{xiaoenv}



\xiao{In the following need to specify $\epsilon$ and $\epsilon'$.}

% \begin{lemma}\label{lem:one-sided:proof:bad1}
% \xiao{Define prefix $\tau$ and $p_{\tau(\View_{H_2})}$ the probability that $H_2$ conditnues to output an accepting view conditioned on the prefix $\tau$. }
% $$\Pr[
% \View_{H_2}~\text{is accepting}~\wedge~p_{\tau(\View_{H_2})} \le \epsilon(\secpar): \View_{H_2} \gets H_2] \le \epsilon(\secpar).$$
% \end{lemma}
% \begin{proof}
%  This lemma follows from the definition of $p_{\tau(\View_{H_2})}$: 
% \begin{align*}
% \Pr_{H_2}[
% \View_{H_2}~\text{is accepting}~\wedge~p_{\tau(\View_{H_2})} \le \epsilon(\secpar)] 
% &= \Pr_{H_2}[p_{\tau(\View_{H_2})} \le \epsilon(\secpar)] \cdot \Pr_{H_2}[ \View_{H_2}~\text{is accepting}~|~p_{\tau(\View_{H_2})} \le \epsilon(\secpar)]\\
% & \le 1 \cdot \Pr_{H_2}[ \View_{H_2}~\text{is accepting}~|~p_{\tau(\View_{H_2})} \le \epsilon(\secpar)]\\
% & = 1 \cdot \epsilon(\secpar).
% \end{align*}
% \end{proof}



\begin{xiaoenv}{}
Define $H^{\mcal{M}}[m]$ and $G^{\mcal{M}}[m]$. Note that $H^{\mcal{M}}[m_0] = H_2$ and $H^{\mcal{M}}[m_1] = H_3$.

\para{Game $H^{\mcal{M}}[m]$:} Identical to $H_2$ except that \Cref{item:one-sided:step:committing} is $\Com_\rho(m;r)$.

\para{Game $G^{\mcal{M}}[m]$:} It first execute $\View_H \gets H^{\mcal{M}}[m]$. It sets $\View_G \coloneqq \View_H$. Next, it sets $\msf{Val}$ in the following way:
\begin{itemize}
\item
If $\View_H$ is not accepting, let $\msf{Val} \coloneqq \bot$;
\item
Otherwise, it executes $\mcal{E}$ on input $\tau(\View_H)$, and sets $\msf{Val}$ to the output of $\mcal{E}(\tau)$.
\end{itemize}
\end{xiaoenv}


\begin{xiaoenv}{Define the simulation-extractor}

\para{Extractor $\mcal{E}(\tau)$.} On input the prefix , it first continues to finish the execution as $H^\mcal{M}[m]$ to learn the view $\View$ of $\mcal{M}$. If $\View$ is not accepting, it outputs $\View$ and $\msf{Val} = \bot$; Otherwise, it rewinds the execution up to $\red{XXX}$ times. for $\red{j \in [XXX]}$, do the following:
\begin{itemize}
\item
to do...
\end{itemize} 
\end{xiaoenv}

\begin{xiaoenv}{finishing }
Note that assuming \Cref{lem:one-sided:proof:statsitcally-close} is true, \Cref{claim:H2-H3} follows from the computationally-hiding property of Naor's commitment. To do...

\end{xiaoenv}

\begin{lemma}\label{lem:one-sided:proof:statsitcally-close}
For any $m \in \bits^\secpar$ and any PPT machine $\mcal{M}$, 
\begin{equation}\label[Expression]{eq:one-sided:proof:statsitcally-close}
\big\{\big(\View_{H}, \tilde{m}(\View_{H})\big):\View_{H} \gets H^{\mcal{M}}[m] \big\} \sind_\epsilon \big\{(\View_G, \msf{Val}):(\View_G, \msf{Val}) \gets G^{\mcal{M}}[m] \big\}.
\end{equation}
\end{lemma}
\begin{proof}
It follows from the definition of $G^\mcal{M}[m]$ that 
$$\big\{\big(\View_{H}, \tilde{m}(\View_{H})\big):\View_{H} \gets H^{\mcal{M}}[m] \big\} \idind \big\{\big(\View_G, \tilde{m}(\View_{G})\big):(\View_G, \msf{Val}) \gets G^{\mcal{M}}[m] \big\}.$$
Thus, to establish \Cref{eq:one-sided:proof:statsitcally-close}, it suffices to show
\begin{equation}\label[Expression]{eq:one-sided:proof:statsitcally-close:goal}
\big\{\big(\View_G, \tilde{m}(\View_{G})\big):(\View_G, \msf{Val}) \gets G^{\mcal{M}}[m] \big\}\sind_\epsilon \big\{(\View_G, \msf{Val}):(\View_G, \msf{Val}) \gets G^{\mcal{M}}[m] \big\}.
\end{equation}
To establish \Cref{eq:one-sided:proof:statsitcally-close:goal}, it suffices to show
\begin{equation}\label[Inequality]{eq:one-sided:proof:statsitcally-close:inequality}
\Pr[\msf{Val}\ne \tilde{m}(\View_{G}):(\View_G, \msf{Val}) \gets G^{\mcal{M}}[m]] \le \epsilon(\secpar) + \negl(\secpar).
\end{equation}
We first define some events w.r.t.\ the random procedure $(\View_G, \Val) \gets G^\mcal{M}[m]$:
\begin{itemize}
\item
$E_1$: the event that $\View_G$ is an accepting view.
\item
$E_2$: the even that $p_{\tau(\View_G)} \le \epsilon(\secpar)$.
\end{itemize}
It follows by definition that the the probability for $(E_1 \wedge E_2)$ is upper-bounded by $\epsilon(\secpar)$. In more details,
\begin{equation}\label{eq:bounding-E1E2}
\Pr_{G^\mcal{M}[m]}[E_1 \wedge E_2] 
= \Pr_{G^\mcal{M}[m]}[E_1 ~|~ E_2] \cdot \Pr_{G^\mcal{M}[m]}[E_2] 
 \le \Pr_{G^\mcal{M}[m]}[E_1 ~|~ E_2] \cdot 1 = \epsilon(\secpar) \cdot 1.	
\end{equation}
Next, we upper-bound the LHS of \Cref{eq:one-sided:proof:statsitcally-close:inequality} by $\Pr[\Val = \tilde{m}(\View_G)~|~E_1 \wedge \neg E_2]$:

\begin{MyClaim}\label{bound:Val-ne-m}
It holds that	
$$\Pr[\msf{Val}\ne \tilde{m}(\View_{G})] \le \epsilon(\secpar) + \Pr[\Val = \tilde{m}(\View_G)~|~E_1 \wedge \neg E_2],$$ where both the probabilities are taken w.r.t.\ the random procedure ${(\View_G, \Val)\gets G^{\mcal{M}}[m]}$.
\end{MyClaim}
\begin{proof}
All the probabilities below are taken w.r.t.\ the same random procedure $(\View_G, \Val)\gets G^{\mcal{M}}[m]$. We thus omit it from the subscript.
\begin{align*}
\Pr[\msf{Val}\ne \tilde{m}(\View_{G})] 
& = \Pr[\msf{Val}\ne \tilde{m}(\View_{G}) \wedge E_1] + \Pr[\msf{Val}\ne \tilde{m}(\View_{G}) \wedge \neg E_1]	\\
& = \Pr[\msf{Val}\ne \tilde{m}(\View_{G}) \wedge E_1] \numberthis \label{bound:Val-ne-m:step:1}	\\
& = \Pr[\msf{Val}\ne \tilde{m}(\View_{G}) \wedge E_1 \wedge E_2] +\Pr[\msf{Val}\ne \tilde{m}(\View_{G}) \wedge E_1 \wedge \neg E_2]	\\
& \le \epsilon(\secpar) +  \Pr[\msf{Val}\ne \tilde{m}(\View_{G}) \wedge E_1 \wedge \neg E_2] \numberthis \label{bound:Val-ne-m:step:2}\\
&\le \epsilon(\secpar) +  \Pr[\msf{Val}\ne \tilde{m}(\View_{G}) ~|
~ E_1 \wedge \neg E_2],
\end{align*}
where \Cref{bound:Val-ne-m:step:1} follows from the fact that if $\View_G$ is not accepting then $\Val = \tilde{m}(\View_G) = \bot$, and \Cref{bound:Val-ne-m:step:2} follows from \Cref{eq:bounding-E1E2}.
\end{proof}
Recall that our goal is to establish \Cref{eq:one-sided:proof:statsitcally-close:inequality}. Because of \Cref{bound:Val-ne-m}, it is now sufficient to show 
\begin{equation}\label[Inequality]{bad:conditioned:E1-nE2}
\Pr_{(\View_G, \Val)\gets G^{\mcal{M}}[m]}[\msf{Val}\ne \tilde{m}(\View_{G}) ~|
~ E_1 \wedge \neg E_2] \le \negl(\secpar).
\end{equation} 
To prove \Cref{bad:conditioned:E1-nE2}, let us first interpret its LHS: 
\begin{itemize}
\item
Given $E_1$ (i.e., $\View_G$ is accepting), we know that $G^\mcal{M}[m]$ must have invoked the machine $\mcal{E}\big(\tau(\View_G)\big)$ and the value $\Val$ is defined to be its output.
\item
Given $\neg E_2$ (i.e., $p_{\tau(\View_G)} > \epsilon(\secpar)$), we know that $\mcal{E}$ must have been invoked on a prefix $\tau(\View_G)$ that has the following property: starting from this $\tau(\View_G)$, $G^\mcal{M}[m]$'s first output will be an accepting view with probability at least $\epsilon(\secpar)$. \xiao{May want to define the execution $G^\mcal{M}_{\tau(\View_G)}[m]$ to specify the prefix. Remark that for $(\View_G, \val)\gets G^\mcal{M}_{\tau}[m]$, we always have $\tau(\View_G) = \tau$.}
\end{itemize}
With the above understanding, it is easy to see that \Cref{bad:conditioned:E1-nE2} is equivalent to the following lemma.
\begin{lemma}\label{lemma:H2-H3:proof:final}
For any prefix $\tau$ corresponding to \Cref{item:one-sided:step:Naor-rho,item:one-sided:step:committing}, if 
\begin{equation}\label[Inequality]{lemma:H2-H3:proof:final:condition}
\Pr[\View_G~\text{is accepting} : \View_G \gets G^\mcal{M}_{\tau}[m]] \ge \epsilon(\secpar),
\end{equation} 
then it holds that 
\begin{equation}\label[Inequality]{lemma:H2-H3:proof:final:result}
\Pr[\Val \ne \tilde{m}(\tau): \Val \gets \mcal{E}(\tau)] \le \negl(\secpar),
\end{equation}
 where $\tilde{m}(\tau)$ denote the value (statistically) bounded in the right-side Naor's commitment (i.e.\ \Cref{item:one-sided:step:Naor-rho,item:one-sided:step:committing}) contained in $\tau$. 
\end{lemma}
We postpone the proof of \Cref{lemma:H2-H3:proof:final} to \Cref{sec:proof:lemma:H2-H3:proof:final}. Assuming that \Cref{lemma:H2-H3:proof:final} is true, it completes the current proof for \Cref{lem:one-sided:proof:statsitcally-close}. 
\end{proof}

\subsection{Proof of \Cref{lemma:H2-H3:proof:final} \red{(Old Stuff)}}
\label{sec:proof:lemma:H2-H3:proof:final}

We prove that under the promise of \Cref{lemma:H2-H3:proof:final:result}, it holds that

\begin{equation}\label[Inequality]{eq:lower-bound:E}
\Pr[\Val = \tilde{m}(\tau): \Val \gets \mcal{E}(\tau)] \ge \epsilon'(\secpar)/\tilde{t}.
\end{equation}
\xiao{need to state the running time of $\mcal{E}$ and the relation between $\epsilon'$ and $\epsilon$. Actually, the above $\mcal{E}$ is the one-shot execution of the $\mcal{E}$ we defined earlier. Will make this explicit later.}

\xiao{Define $\mcal{E}_{\tilde{i}}(\tau)$. By the relation between $\mcal{E}(\tau)$ and $\mcal{E}_{\tilde{i}}(\tau)$, to prove \Cref{eq:lower-bound:E}, it suffices to prove the following lemma.}
\begin{lemma}\label{lem:lower-bound:Ei}
For any prefix $\tau$ corresponding to \Cref{item:one-sided:step:Naor-rho,item:one-sided:step:committing}, if 
\begin{equation}\label[Inequality]{lem:lower-bound:Ei:condition}
\Pr[\View_G~\text{is accepting} : \View_G \gets G^\mcal{M}_{\tau}[m]] \ge \epsilon(\secpar),
\end{equation} 
then
there exists $\tilde{i} \in [\tilde{t}]$ s.t.\ $$\Pr[\Val = \tilde{m}(\tau): \Val \gets \mcal{E}_{\tilde{i}}(\tau)] \ge \epsilon'(\secpar).$$
\end{lemma}
\para{Proving \Cref{lem:lower-bound:Ei}.} In the remainder of this section, we prove \Cref{lem:lower-bound:Ei}, which eventually finishes the proof of \Cref{lemma:H2-H3:proof:final}.

We prove this lemma by contradiction. Under the condition of \Cref{lem:lower-bound:Ei:condition}, we assume for contradiction that 
$$\forall \tilde{i} \in [\tilde{t}], ~\Pr[\Val = \tilde{m}(\tau): \Val \gets \mcal{E}_{\tilde{i}}(\tau)] < \epsilon'(\secpar).$$


\begin{MyClaim}
For any $\tau$ satisfying the assumption of \Cref{lem:lower-bound:Ei:condition}, the following holds:
$$\forall \tilde{i}\in [\tilde{t}], ~\Pr[\Val = \tilde{X}_{\tilde{i}} : \Val \gets\mcal{E}_{\tilde{i}}(\tau)] \ge \epsilon(\secpar)/\tilde{t} - \epsilon'(\secpar) - \negl(\secpar).$$
\end{MyClaim}
\begin{proof}
\begin{xiaoenv}{Proof sketch}
\begin{itemize}
\item
Define $\mcal{E}^*_{\tilde{i}}(\tau)$, which is identical to $\mcal{E}_{\tilde{i}}(\tau)$ except that it plays the final \WIPoK in the right execution as the honest receiver, instead of running the emulation-extractor. $\mcal{E}^*_{\tilde{i}}(\tau)$ outputs a view $\View_{\tilde{i}}$.
\item
By the property of the \WIPoK emulation-extractor, it holds that 
$$\forall \tilde{i} \in [\tilde{t}], ~\Pr[\Val\ne \bot:\Val\gets\mcal{E}_{\tilde{i}}(\tau)] \ge \Pr[\View_{\tilde{i}}~\text{is accepting}:\View_{\tilde{i}}\gets\mcal{E}^*_{\tilde{i}}(\tau)] -\negl(\secpar).$$
where $\Val \ne \bot$ means that the extracted $\Val$ is a valid witness for the statement $\tilde{\com} \vee (\tilde{y}_1, \ldots, \tilde{y}_{\tilde{t}})$.
\item
We define the following machine $\mcal{E}^*(\tau)$ that on any prefix $\tau$:	
\begin{itemize}
\item
sample a random $\tilde{i} \pick [\tilde{t}]$;
\item
Run $\View\gets\mcal{E}_{\tilde{i}}(\tau)$, and outputs $\View$.
\end{itemize}
It is obvious that 
$$\Pr[\View~\text{is accepting}:\View\gets\mcal{E}^*(\tau)] = \Pr[\View_G~\text{is accepting} : \View_G \gets G^\mcal{M}_{\tau}[m]].$$
\item
Since $\tau$ satisfying \Cref{lem:lower-bound:Ei:condition}, we know that for such a $\tau$, 
$$\Pr[\View~\text{is accepting}:\View\gets\mcal{E}^*(\tau)] \ge \epsilon(\secpar).$$
\item
By the definition of $\mcal{E}^*(\cdot)$, we know that for such a $\tau$, 
$$\exists \tilde{j} \in [\tilde{t}]~s.t.~\Pr[\View~\text{is accepting}:\View\gets\mcal{E}^*_{\tilde{j}}(\tau)] \ge \epsilon(\secpar)/\tilde{t}.$$
\end{itemize}
\end{xiaoenv}
\end{proof}

==> sections/one-sided-_old-stuff_.tex <==

\subsection{Proving Non-Malleability \red{(Old Stuff)}}
\label{one-sided:non-malleability:proof:classical}

\begin{theorem}\label{thm:one-sided:non-malleability}
The commitment scheme $\langle C, R \rangle$ in \Cref{prot:one-sided:classical} is a one-sided non-malleable commitment scheme secure against synchronous PPT adversaries.
\end{theorem}	
% To prove \Cref{thm:one-sided:non-malleability}, we show that
% \begin{equation}\label[Expression]{eq:one-sided:goal}
% \Set{\msf{mim}^\mcal{M}_{\langle C, R \rangle}(\secpar, m_0, z)}_{\secpar, m_0, m_1, z} \cind \Set{\msf{mim}^\mcal{M}_{\langle C, R \rangle}(\secpar, m_1, z)}_{\secpar, m_0, m_1, z},
% \end{equation}
% where $\secpar \in \Naturals$, $m_0, m_1 \in \bits^{\secpar}$, and $z \in \bits^*$.

To prove \Cref{thm:one-sided:non-malleability}, let us first define the game that captures the man-in-the-middle execution corresponding to $\msf{mim}^\mcal{M}_{\langle C, R \rangle}(\secpar, m, z)$ with the $\langle C, R \rangle$ defined in \Cref{prot:one-sided:classical}.

\para{Game $H^{\mcal{M}}(\secpar,m,z)$:\label{gameH:description}} (Illustrated in \Cref{figure:one-sided:H}.) This is the man-in-the-middle execution of the commit stage of the $\langle C, R \rangle$ defined in \Cref{prot:one-sided:classical}, where the left committer commits to $m$ and $\mcal{M}$'s non-uniform advice is $z$. The output of this game is defined as the view of $\mcal{M}$ resulted from this execution, which we denote as $\View_H$. \xiao{It seems more convenient to define the output of game to be the output of $\mcal{M}$, instead of its view.}

\para{Notation.} For any $\View_H$ output by $H^{\mcal{M}}(\secpar,m,z)$, we say that $\View_H$ is an {\em accepting} view if the honest receiver $R$ in the right session accepts at the end of the commit stage. \xiao{(here, it seems we can assume w.l.o.g.\ that we can tell if $\View_H$ is accepting or not efficiently.)} We use $\tilde{m}(\View_H)$ to denote the value committed by $\mcal{M}$: if $\View_H$ is accepting, $\tilde{m}(\View_H) \coloneqq \bot$; otherwise, $\tilde{m}(\View_H)$ is defined to be the value (statistically) bounded in \Cref{item:one-sided:step:Naor-rho,item:one-sided:step:committing} of the right execution (i.e., the right-side Naor's commitment). In particular, it holds that:
\begin{equation}\label{eq:classical:mim-H}
\big\{\msf{mim}^\mcal{M}_{\langle C, R \rangle}(\secpar, m, z)\big\} \idind \big\{\big(\View_H, \tilde{m}(\View_H)\big):\View_H \gets H^{\mcal{M}}(\secpar,m,z) \big\},
\end{equation}
where both ensembles are index by $\secpar \in \Naturals$, $m \in \bits^\secpar$, and $z \in \bits^*$. \xiao{Need to modify the length of the message to $\ell(\secpar)$.}

Therefore, to prove that \Cref{prot:one-sided:classical} satisfies \Cref{def:NMCom:classical}, it suffices to show the following:
\begin{equation}
\label{eq:classical:H:m-0:m-1}
\big\{\big(\View^0_H, \tilde{m}(\View^0_H)\big):\View^0_H \gets H^{\mcal{M}}(\secpar,m_0,z) \big\} \cind \big\{\big(\View^1_H, \tilde{m}(\View^1_H)\big):\View^1_H \gets H^{\mcal{M}}(\secpar,m_1,z) \big\},
\end{equation}
where both ensembles are index by $\secpar \in \Naturals$, $m_0, m_1 \in \bits^\secpar$, and $z \in \bits^*$.

\para{Proof by Contradiction.} Our high-level strategy is proof by contradiction. We assume for contradiction that there are a PPT machine $\mcal{D}$ and a function $\epsilon(\secpar) = 1/\poly(\secpar)$ such that for infinitely many $\secpar \in \Naturals$,
\begin{equation}\label[Inequality]{eq:one-sided:proof:contra-assump}
\bigg|\Pr[\mcal{D}\big(1^\secpar, \View^0_H, \tilde{m}(\View^0_H)\big)] - \Pr[\mcal{D}\big(1^\secpar,\View^1_H, \tilde{m}(\View^1_H)\big)] \bigg|\ge 3 \cdot \epsilon(\secpar),
\end{equation}
where the first probability is taken over the random procedure $\View^0_H \gets H^{\mcal{M}}(\secpar,m_0,z)$ and the second probability is taken over the random procedure $\View^1_H \gets H^{\mcal{M}}(\secpar,m_1,z)$.

We then show the following lemma:
\begin{lemma}\label{lem:one-sided:proof:core}
For the above $\epsilon(\secpar)$,
there exits a hybrid $G$ such that for any PPT $\mcal{M}$, the following holds
\begin{enumerate}
\item\label[Property]{item:lem:one-sided:proof:core:1}
$\big\{(\View_0, \Val_0):(\View_0, \Val_0) \gets G^{\mcal{M}}(\secpar,m_0,z) \big\} \cind \big\{(\View_1, \Val_1):(\View_1, \Val_1) \gets G^{\mcal{M}}(\secpar,m_1,z) \big\}$, where both ensembles are index by $\secpar \in \Naturals$, $m_0, m_1 \in \bits^\secpar$, and $z \in \bits^*$.
\item\label[Property]{item:lem:one-sided:proof:core:2}
$\big\{(\View_G, \Val):(\View_G, \Val) \gets G^{\mcal{M}}(\secpar,m,z) \big\} \sind_{\epsilon(\secpar)} \big\{\big(\View_H, \tilde{m}(\View_H)\big):\View_H \gets H^{\mcal{M}}(\secpar,m,z) \big\}$,  where both ensembles are index by $\secpar \in \Naturals$, $m \in \bits^\secpar$, and $z \in \bits^*$.
\end{enumerate}
\end{lemma}
It is easy to see that if \Cref{lem:one-sided:proof:core} is true, it will contradict our assumption in \Cref{eq:one-sided:proof:contra-assump}. Thus, it will finish the proof of non-malleability. Indeed, this lemma is the most technically involved part. We prove it in \Cref{sec:one-sided:core-lemma:proof}.



\subsection{Proof of \Cref{lem:one-sided:proof:core} \red{(Old Stuff)}}
\label{sec:one-sided:core-lemma:proof}

We first describe the hybrid $G$ mentioned in \Cref{lem:one-sided:proof:core}, and then prove that it has the desired properties. Note that $G$ depends on $\epsilon$, though we does not make $\epsilon$ an explicit input parameter for $G$. In \Cref{item:hyb:G:runK} below, We will need an extra parameter $\epsilon'$ which is defined as $\epsilon'(\secpar) \coloneqq \frac{\epsilon(\secpar)}{t^2}$. The reason for this setup will become clear later in the proof. For now, we want to remark that this notation is not really necessary---We can always write $\frac{\epsilon(\secpar)}{t^2}$ (and with potential simplifications) whenever we need $\epsilon'(\secpar)$. We choose to define $\epsilon'(\secpar)$ as a separate parameter because it helps make our presentation conceptually cleaner.

Also, the hybrid $G$ will invoke a machine $\mcal{K}$ as a sub-procedure, which will be defined and constructed in \Cref{lem:extractorK}.

\begin{AlgorithmBox}[label={hybrid:G}]{Hybrid \textnormal{$G^{\mcal{M}}(\secpar,m,z)$}} 
\red{Once I finish the quantum version, I'll modify this algorithm slightly. There is no need to run the ``main-thread'' for the first time. We can simply obtain the prefix $\tau$, and start running $\mcal{K}$ directly. This is more consistent with the quantum version.} This hybrid proceeds as follows:
\begin{enumerate}
\item
Execute $\View_H \gets H^{\mcal{M}}(\secpar,m,z)$. 
\item
Set $\View_G \coloneqq \View_H$. 
\item
If $\View_G$ is {\em not} an accepting view \red{(here, it seems we can assume w.l.o.g.\ that we can tell if $\View_H$ is accepting or not efficiently.)}, set $\Val \coloneqq \bot$ and then jump directly to \Cref{item:hyb:G:final}; Otherwise (i.e., $\View_G$ is an accepting view), go to the next step (i.e., \Cref{item:hyb:G:runK}).
\item \label[Step]{item:hyb:G:runK}
Let $\tau(\View_G)$ denote the prefix of the view $\View_G$ that corresponds to \Cref{item:one-sided:step:Naor-rho,item:one-sided:step:committing} of the man-in-the-middle execution. Namely, it contains all the information of the execution right before the beginning of \Cref{item:one-sided:step:OWFs}. Therefore, a PPT procedure can resume $\tau(\View_G)$ to finish the main-in-the-middle execution corresponding to $\View_G$.

$G^{\mcal{M}}(\secpar,m,z)$ then loops the following procedure for $\frac{\tilde{t}}{\epsilon'(\secpar)} \cdot \secpar$ times, where $\epsilon'(\secpar) \coloneqq \frac{\epsilon(\secpar)}{t^2}$:
\begin{itemize}
\item
Execute $\Val_{\mcal{K}} \gets \mcal{K}\big(\tau(\View_G)\big)$, where $\mcal{K}$ is defined in \Cref{lem:extractorK}.  If $\Val_{\mcal{K}} = \tilde{m}(\View_G)$ \red{(This is not efficient in general. But we are using Naor's $\Com$, which has is efficiently testable. Need to explain this explicitly. Put it in another way, what $\mcal{K}$ extracted is not only the message, but also the decommitment information.)}, set $\Val \coloneqq \Val_{\mcal{K}}$ and jump to \Cref{item:hyb:G:final}; otherwise, go to the next loop.
\end{itemize}
\item
Set $\Val \coloneqq \bot$.
\item \label[Step]{item:hyb:G:final}
Output $(\View_G, \Val)$.
\end{enumerate}
\end{AlgorithmBox}

Before talking about the extractor $\mcal{K}$, let us first define a variable that captures the probability that the man-in-the-middle yields an accepting view conditioned on a given prefix $\tau$.
\begin{definition}[Accepting Probability from Prefix $\tau$]\label{def:p-tau:1}
For any prefix $\tau$ corresponding to the first two steps of the man-in-the-middle execution (see also \Cref{item:hyb:G:runK} of \Cref{hybrid:G}), let $p_\tau$ denote the probability that continuing from this particular prefix $\tau$, the man-in-the-middle execution will yield an accepting view.
\end{definition}

\begin{lemma}[Extractor $\mcal{K}$]\label{lem:extractorK}
There exists a machine $\mcal{K}$ that takes as input a prefix $\tau$ corresponding to \Cref{item:one-sided:step:Naor-rho,item:one-sided:step:committing} of the man-in-the-middle execution, and tries to output $\tilde{m}(\tau)$, which is defined to be the value committed in the right Naor's commitment in $\tau$. Machine $\mcal{K}$ satisfies the following requirements:
\begin{enumerate}
\item\label[Property]{item:extractorK:efficiency}
On any input $\tau$, $\mcal{K}(\tau)$ runs in expected polynomial time on the security parameter $\secpar$ (contained implicitly in $\tau$).
\item\label[Property]{item:extractorK:extractability}
Let $\epsilon(\secpar) = \frac{1}{\poly(\secpar)}$ and $\epsilon'(\secpar) = \frac{\epsilon(\secpar)}{t^2}$. For any $\tau$, if $p_\tau\ge \epsilon(\secpar)$ (where $p_\tau$ is defined in \Cref{def:p-tau:1}), then 
$$\Pr[\Val = \tilde{m}(\tau) :\Val \gets \mcal{K}(\tau)] \ge \epsilon'(\secpar)/\tilde{t}.$$
\xiao{Need to modify this part: what $\mcal{K}$ extracted is not only the message, but also the decommitment information. See the red text in \Cref{item:hyb:G:runK}.}
\end{enumerate}
\end{lemma}
The proof of \Cref{lem:extractorK} is the most involved part for the current proof of \Cref{lem:one-sided:proof:core}. We will do that in \Cref{sec:lem:extractorK:proof}. For now, let us first use \Cref{lem:extractorK} to finish the current proof of \Cref{lem:one-sided:proof:core}, assuming that the former is correct.


\para{Proving \Cref{item:lem:one-sided:proof:core:1} in \Cref{lem:one-sided:proof:core}.\label{para:lem:one-sided:proof:core:1}} Observe that hybrid $G^{\mcal{M}}(\secpar,m,z)$ is an efficient machine \xiao{This argument is not accurate. $G$ is not efficient yet. See the red text in \Cref{item:hyb:G:runK}.} (this makes use of \Cref{item:extractorK:efficiency} in \Cref{lem:extractorK}). Moreover, it does not rewind \Cref{item:one-sided:step:Naor-rho,item:one-sided:step:committing} of the man-in-the-middle execution. Therefore, \Cref{item:lem:one-sided:proof:core:1} in \Cref{lem:one-sided:proof:core} follows immediately from the computationally hiding property of the left Naor's commitment (i.e., \Cref{item:one-sided:step:Naor-rho,item:one-sided:step:committing} in the left execution).

Now, to finish the proof of \Cref{lem:one-sided:proof:core}, we only need to prove \Cref{item:lem:one-sided:proof:core:2}.


\para{Proving \Cref{item:lem:one-sided:proof:core:2} in \Cref{lem:one-sided:proof:core}.\label{para:lem:one-sided:proof:core:2}} We first observe that, by the definition of $G^{\mcal{M}}(\secpar,m,z)$, the following holds 
$$\big\{\big(\View_{H}, \tilde{m}(\View_{H})\big):\View_{H} \gets H^{\mcal{M}}(\secpar,m,z) \big\} \idind \big\{\big(\View_G, \tilde{m}(\View_{G})\big):(\View_G, \msf{Val}) \gets G^{\mcal{M}}(\secpar,m,z) \big\},$$
where both ensembles are index by $\secpar \in \Naturals$, $m \in \bits^\secpar$, and $z \in \bits^*$.
Thus, to establish \Cref{item:lem:one-sided:proof:core:2} in \Cref{lem:one-sided:proof:core}, it suffices to show
\begin{equation}\label[Expression]{eq:one-sided:proof:statsitcally-close:goal}
\big\{\big(\View_G, \tilde{m}(\View_{G})\big):(\View_G, \msf{Val}) \gets G^{\mcal{M}}(\secpar,m,z)  \big\}\sind_\epsilon \big\{(\View_G, \msf{Val}):(\View_G, \msf{Val}) \gets G^{\mcal{M}}(\secpar,m,z)  \big\},
\end{equation}
where both ensembles are index by $\secpar \in \Naturals$, $m \in \bits^\secpar$, and $z \in \bits^*$.

To establish \Cref{eq:one-sided:proof:statsitcally-close:goal}, it suffices to show
\begin{equation}\label[Inequality]{eq:one-sided:proof:statsitcally-close:inequality}
\Pr[\msf{Val}\ne \tilde{m}(\View_{G}):(\View_G, \msf{Val}) \gets G^{\mcal{M}}(\secpar,m,z)] \le \epsilon(\secpar) + \negl(\secpar).
\end{equation}
To do that, let us first define two events w.r.t.\ the random procedure $(\View_G, \msf{Val}) \gets G^{\mcal{M}}(\secpar,m,z)$:
\begin{itemize}
\item
$E_{\msf{acc}}$: the event that $\View_G$ is an accepting view.
\item
$E_{\le \epsilon}$: the even that $p_{\tau(\View_G)} \le \epsilon(\secpar)$.
\end{itemize}
We first show that the the probability for $(E_{\msf{acc}} \wedge E_{\le \epsilon})$ is upper-bounded by $\epsilon(\secpar)$. 

\begin{MyClaim} 
It holds that
$\Pr[E_{\msf{acc}} \wedge E_{\le \epsilon}:(\View_G, \msf{Val}) \gets G^{\mcal{M}}(\secpar,m,z)]  \le \epsilon(\secpar)$.
\end{MyClaim}
\begin{proof}
This is an immediate result following from the definitions of these two events. In more details,
\begin{equation}\label[Inequality]{eq:bounding-E1E2}
\Pr[E_{\msf{acc}} \wedge E_{\le \epsilon}] 
= \Pr[E_{\msf{acc}} ~|~ E_{\le \epsilon}] \cdot \Pr[E_{\le \epsilon}] 
 \le \Pr[E_{\msf{acc}} ~|~ E_{\le \epsilon}] \cdot 1 = \epsilon(\secpar) \cdot 1,	
\end{equation}
where all the probabilities are taken over the random procedure $(\View_G, \msf{Val}) \gets G^{\mcal{M}}(\secpar,m,z)$.
\end{proof}

Next, we upper-bound the LHS of \Cref{eq:one-sided:proof:statsitcally-close:inequality} by $\Pr[\Val = \tilde{m}(\View_G)~|~E_{\msf{acc}} \wedge \neg E_{\le \epsilon}]$:

\begin{MyClaim}\label{bound:Val-ne-m}
It holds that	
$$\Pr[\msf{Val}\ne \tilde{m}(\View_{G})] \le \epsilon(\secpar) + \Pr[\Val = \tilde{m}(\View_G)~|~E_{\msf{acc}} \wedge \neg E_{\le \epsilon}],$$ where both the probabilities are taken w.r.t.\ the random procedure $(\View_G, \msf{Val}) \gets G^{\mcal{M}}(\secpar,m,z)$.
\end{MyClaim}
\begin{proof}
All the probabilities below are taken w.r.t.\ the random procedure $(\View_G, \msf{Val}) \gets G^{\mcal{M}}(\secpar,m,z)$. We thus omit it from the subscript.
\begin{align*}
\Pr[\msf{Val}\ne \tilde{m}(\View_{G})] 
& = \Pr[\msf{Val}\ne \tilde{m}(\View_{G}) \wedge E_{\msf{acc}}] + \Pr[\msf{Val}\ne \tilde{m}(\View_{G}) \wedge \neg E_{\msf{acc}}]	\\
& = \Pr[\msf{Val}\ne \tilde{m}(\View_{G}) \wedge E_{\msf{acc}}] \numberthis \label{bound:Val-ne-m:step:1}	\\
& = \Pr[\msf{Val}\ne \tilde{m}(\View_{G}) \wedge E_{\msf{acc}} \wedge E_{\le \epsilon}] +\Pr[\msf{Val}\ne \tilde{m}(\View_{G}) \wedge E_{\msf{acc}} \wedge \neg E_{\le \epsilon}]	\\
& \le \epsilon(\secpar) +  \Pr[\msf{Val}\ne \tilde{m}(\View_{G}) \wedge E_{\msf{acc}} \wedge \neg E_{\le \epsilon}] \numberthis \label[Inequality]{bound:Val-ne-m:step:2}\\
&\le \epsilon(\secpar) +  \Pr[\msf{Val}\ne \tilde{m}(\View_{G}) ~|
~ E_{\msf{acc}} \wedge \neg E_{\le \epsilon}],
\end{align*}
where \Cref{bound:Val-ne-m:step:1} follows from the fact that if $\View_G$ is not accepting then $\Val = \tilde{m}(\View_G) = \bot$, and \Cref{bound:Val-ne-m:step:2} follows from \Cref{eq:bounding-E1E2}.
\end{proof}
Recall that our goal is to establish \Cref{eq:one-sided:proof:statsitcally-close:inequality}. Because of \Cref{bound:Val-ne-m}, it is now sufficient to show 
\begin{equation}\label{bad:conditioned:E1-nE2}
\Pr_{(\View_G, \Val)\gets G^{\mcal{M}}(\secpar,m,z)}[\msf{Val}\ne \tilde{m}(\View_{G}) ~|
~ E_{\msf{acc}} \wedge \neg E_{\le \epsilon}] = \negl(\secpar).
\end{equation}
\begin{proof}[Proof of \Cref{bad:conditioned:E1-nE2}]
Given $E_{\msf{acc}}$ (i.e., $\View_G$ is accepting), we know that $G^{\mcal{M}}(\secpar,m,z)$ must have entered \Cref{item:hyb:G:runK} to execute the machine $\mcal{K}\big(\tau(\View_G)\big)$ for at most $\frac{\tilde{t}}{\epsilon'(\secpar)} \cdot \secpar$ times, with early termination only if the event $\Val_{\mcal{K}} = \tilde{m}\big(\tau(\View_G)\big)$ happens (see \Cref{hybrid:G}).\footnote{Technically speaking, in \Cref{item:hyb:G:runK} of \Cref{hybrid:G}, $G$ loops until $\Val_{\mcal{K}} = \tilde{m}(\View_G)$ happens. But it is obvious that $\tilde{m}\big(\tau(\View_G)\big) \equiv\tilde{m}(\View_G)$.}

Given $\neg E_{\le \epsilon}$ (i.e., $p_{\tau(\View_G)} > \epsilon(\secpar)$), it follows from \Cref{item:extractorK:extractability} in \Cref{lem:extractorK} that each time $\mcal{K}$ is invoked on $\tau(\View_G)$, it holds that $\Pr[\Val = \tilde{m}\big(\tau(\View_G)\big) :\Val \gets \mcal{K}\big(\tau(\View_G) \big)] \ge \epsilon'(\secpar)/\tilde{t}$.

Therefore, we have 
\begin{equation*}
\Pr_{(\View_G, \Val)\gets G^{\mcal{M}}(\secpar,m,z)}[\msf{Val}\ne \tilde{m}(\View_{G}) ~|
~ E_{\msf{acc}} \wedge \neg E_{\le \epsilon}] = (1 - \frac{\epsilon'(\secpar)}{\tilde{t}})^{\frac{\tilde{t}}{\epsilon'(\secpar)}\cdot \secpar} = 2^{-O(\secpar)} = \negl(\secpar).
\end{equation*}
%that has the following property: starting from this $\tau(\View_G)$, $G^{\mcal{M}}(\secpar,m,z)$'s first output will be an accepting view with probability at least $\epsilon(\secpar)$. %\xiao{May want to define the execution $G^\mcal{M}_{\tau(\View_G)}[m]$ to specify the prefix. Remark that for $(\View_G, \val)\gets G^\mcal{M}_{\tau}[m]$, we always have $\tau(\View_G) = \tau$.}
This finishes the proof of \Cref{bad:conditioned:E1-nE2}.
\end{proof} 
This eventually finishes the proof of \Cref{item:lem:one-sided:proof:core:2} in \Cref{lem:one-sided:proof:core} (and thus \Cref{lem:one-sided:proof:core}). 


\subsection{Extractor $\mcal{K}$ (Proof of \Cref{lem:extractorK})}
\label{sec:lem:extractorK:proof}

In this section, we prove \Cref{lem:extractorK}. We will construct the extractor $\mcal{K}$ prescribed by \Cref{lem:extractorK}, and show that it enjoys the stipulated properties. We will build the extractor $\mcal{K}$
gradually, starting by defining several intermediate machines.
The description of $\mcal{K}$ will appear toward the end of this subsection (on \Cpageref{extractorK:description}). We found this arrangement most reader-friendly. Moreover, we illustrate all the intermediate machines in \Cref{figure:one-sided:games}.


\para{Machine $\mcal{G}_{i}$ ($i \in [\tilde{t}]$):\label{machine:Gi}} (Illustrated in \Cref{figure:one-sided:Gi}.)
Recall the man-in-the-middle execution $H^{\mcal{M}}(\secpar,m,z)$ defined on \Cpageref{gameH:description} (and depicted in \Cref{figure:one-sided:H}). We can re-interpret $H^{\mcal{M}}(\secpar,m,z)$ as consisting of the following two steps:
\begin{enumerate}
\item
It first executes the \Cref{item:one-sided:step:Naor-rho,item:one-sided:step:committing} of the man-in-the-middle execution. Let $\tau$ denote the states and transcripts of all the parties $C$, $R$, and $\mcal{M}$ at the end of \Cref{item:one-sided:step:committing}. Recall that  we refer to this $\tau$ as the prefix of the man-in-the-middle execution.
\item\label[Step]{item:H:re-interp:2}
It then resumes the execution from $\tau$ to finish the remaining steps as $H^{\mcal{M}}(\secpar,m,z)$.
\end{enumerate}
We now define $\mcal{G}_1(\tau)$ as the machine corresponding to the  \Cref{item:H:re-interp:2} above. That is, on input the prefix $\tau$, $\mcal{G}_1(\tau)$ finishes the remaining part of the man-in-the-middle execution identically as $H^{\mcal{M}}(\secpar,m,z)$. In particular, $\mcal{G}_1(\tau)$ uses the witness $\tilde{x}_1$ to go through the right {\bf WIPoK-1} (the subscript ``1'' is meant to signal this fact), and at the end, $\mcal{G}_1(\tau)$ output the view of $\mcal{M}$ (same as $H^{\mcal{M}}(\secpar,m,z)$).

Then, for any $i \in [\tilde{t}]\setminus \Set{1}$, we define $\mcal{G}_{i}(\tau)$ as the machine that behaves identically to $\mcal{G}_1(\tau)$, except that $\mcal{G}_i(\tau)$ uses the witness $\tilde{x}_{i}$ in the right {\bf WIPoK-1}.

For a prefix $\tau$, let us (re-)define the probability that $\tau$ leads to an accepting execution. Recall that we actually already defined this term in \Cref{def:p-tau:1}. The following definition is equivalent to \Cref{def:p-tau:1}, but is formalized w.r.t.\ the machine $\mcal{G}_1$. This version turns out to be more suitable for the rest of the proof.
\begin{definition}\label{def:p-tau:2}
For any $\tau$ that corresponds to \Cref{item:one-sided:step:Naor-rho,item:one-sided:step:committing} of the execution $H^{\mcal{M}}(\secpar,m,z)$, we define
\begin{equation}\label{eq:def:p-tau}
p_\tau \coloneqq \Pr[\View~\text{is accepting}: \View \gets \mcal{G}_1(\tau)].
\end{equation}
\end{definition}
We first claim that the accepting probabilities for $\mcal{G}_i(\tau)$'s with different $i \in [\tilde{t}]$  are almost the same.
\begin{figure}[!tb]
     \begin{subfigure}[t]{0.47\textwidth}
         \centering
         \fbox{
         \includegraphics[width=\textwidth]{figures/figure01.pdf}
         }
         \caption{}
         \label{figure:one-sided:H}
     \end{subfigure}
     \hspace{6.5pt}
     \begin{subfigure}[t]{0.47\textwidth}
         \centering
         \fbox{
         \includegraphics[width=\textwidth]{figures/figure02.pdf}
         }
         \caption{}
         \label{figure:one-sided:Gi}
     \end{subfigure}
     \vskip\baselineskip
      \begin{subfigure}[t]{0.47\textwidth}
         \centering
         \fbox{
         \includegraphics[width=\textwidth]{figures/figure03.pdf}
         }
         \caption{}
         \label{figure:one-sided:G'i}
     \end{subfigure}
     \hspace{6.5pt}
     \begin{subfigure}[t]{0.47\textwidth}
         \centering
         \fbox{
         \includegraphics[width=\textwidth]{figures/figure04.pdf}
         }
         \caption{}
         \label{figure:one-sided:G''i}
     \end{subfigure}
     \vskip\baselineskip
     \begin{subfigure}[t]{0.47\textwidth}
         \centering
         \fbox{
         \includegraphics[width=\textwidth]{figures/figure05.pdf}
         }
         \caption{}
         \label{figure:one-sided:Ki}
     \end{subfigure}
     \hspace{6.5pt}
     \begin{subfigure}[t]{0.47\textwidth}
         \centering
         \fbox{
         \includegraphics[width=\textwidth]{figures/figure06.pdf}
         }
         \caption{}
         \label{figure:one-sided:K}
     \end{subfigure}
     \caption{Different Hybrids/Machines \scriptsize{(Changes between adjacent machines are highlighted by red color)}}
     \label{figure:one-sided:games}
\end{figure}

\begin{MyClaim}\label{claim:bound:Gi}
% For any $\tau$, if $p_\tau \ge \epsilon(\secpar)$, then it holds that  
$\forall i \in [\tilde{t}], ~\Pr[\View~\text{is accepting}:\View \gets \mcal{G}_i(\tau)] \ge p_\tau - \negl(\secpar)$.
\end{MyClaim}
\begin{proof}
Note that the machine $\mcal{G}_i(\tau)$ does not rewind the right {\bf WIPoK-1}, and for any $i \in [\tilde{t}] \setminus \Set{1}$, $\mcal{G}_i(\tau)$ differs from $\mcal{G}_1(\tau)$ only by the witness used in the right {\bf WIPoK-1}. Therefore, it follows from the WI property of the right {\bf WIPoK-1} that for any $i \in [\tilde{t}]$,
$$\big| \Pr[\View~\text{is accepting}:\View \gets \mcal{G}_i(\tau)] - \Pr[\View~\text{is accepting}:\View \gets \mcal{G}_1(\tau)]\big| \le \negl(\secpar).$$
Then, by the definition of $p_\tau$ (\Cref{eq:def:p-tau}), \Cref{claim:bound:Gi} follows.
\end{proof}

\para{Machine $\mcal{G}'_i$ ($i\in [\tilde{t}]$):} (Illustrated in \Cref{figure:one-sided:G'i}.) On any input $\tau$, $\mcal{G}'_i(\tau)$ behaves identically to $\mcal{G}_i(\tau)$, except the following change. Instead of executing the left {\bf WIPoK-1} (i.e., \Cref{item:one-sided:step:WIPoK:1} in the left) honestly, $\mcal{G}'_i$ invokes the emulation-extractor $\SimExt$ to emulate the left {\bf WIPoK-1} while extracting a value $(j, x_j)$ \xiao{need to make a new notation: the extracted value could be $\bot$}. Recall that the existence of $\SimExt$ is guaranteed by the PoK property of $\WIPoK$ (see \Cref{def:WEE}). If  $(j, x_j) \notin \Relation_{\Lang^t_f}(Y)$ \xiao{change the notation} (see \Cref{eq:one-sided:Lang:OWF})---namely, the extraction fails---$\mcal{G}'_i(\tau)$ aborts; Otherwise, it continues to finish the execution identically as $\mcal{G}_i(\tau)$. It is worth noting that although $\SimExt$ may extract a valid $(j, x_j)$ pair, $\mcal{G}'_i(\tau)$ does {\em not} use it.  

\begin{MyClaim}\label{claim:bound:G'i}
% For any $\tau$, if $p_\tau \ge \epsilon(\secpar)$, then it holds that  
$\forall i \in [\tilde{t}], ~\Pr[\View~\text{is accepting}:\View \gets \mcal{G}'_i(\tau)] \ge p_\tau - \negl(\secpar)$.
\end{MyClaim}
\begin{proof}
This claim follows immediately from \Cref{claim:bound:Gi} and the witness-extended emulation property (as per \Cref{def:WEE}) of the left {\bf WIPoK-1}.
\end{proof}

\para{Machine $\mcal{G}''_i$ ($i\in [\tilde{t}]$):} (Illustrated in \Cref{figure:one-sided:G''i}.) On any input $\tau$, $\mcal{G}''_i(\tau)$ behaves identically to $\mcal{G}'_i(\tau)$, except that $\mcal{G}''_i(\tau)$ use the $(j, x_j)$ (extracted in $\mcal{G}'_i(\tau)$) to finish the left {\bf WIPoK-2} (i.e., \Cref{item:one-sided:step:WIPoK:2} in the left execution).

\begin{MyClaim}\label{claim:bound:G''i}
% For any $\tau$, if $p_\tau \ge \epsilon(\secpar)$, then it holds that  
$\forall i \in [\tilde{t}], ~\Pr[\View~\text{is accepting}:\View \gets \mcal{G}''_i(\tau)] \ge p_\tau - \negl(\secpar)$.
\end{MyClaim}
\begin{proof}
This claim follows immediately from \Cref{claim:bound:G'i} and the WI property of the left {\bf WIPoK-2}.
\end{proof}

\para{Machine $\mcal{K}_i$ ($i\in [\tilde{t}]$):} (Illustrated in \Cref{figure:one-sided:Ki}.) On any input $\tau$, $\mcal{K}_i(\tau)$ behaves identically to $\mcal{G}''_i(\tau)$, except for the following difference. Machine $\mcal{K}_i(\tau)$ uses the witness-extended emulator $\SimExt$ to finish the right {\bf WIPoK-2}, instead of playing the role of the honest receiver. Let $\Val$ denote the witness extracted by $\SimExt$. We use $\Val = \bot$ to denote the situation where $\Val$ is not a valid witness for the statement $\big(\tilde{\com}, (\tilde{y}_1, \ldots, \tilde{y}_{\tilde{t}})\big)$. (Recall that  $\big(\tilde{\com}, (\tilde{y}_1, \ldots, \tilde{y}_{\tilde{t}})\big)$ is supposed to be an instance in the language $\Lang_{\tilde{\rho}} \vee \Lang^{\tilde{t}}_{\tilde{f}}$.) %If $\Val = \bot$, $\mcal{K}_i(\tau)$ aborts and outputs a special symbol $\msf{Fail}_{\mcal{K}}$. 
\begin{MyClaim}\label{claim:bound:Ki}
% For any $\tau$, if $p_\tau \ge \epsilon(\secpar)$, then it holds that
$\forall i \in [\tilde{t}], ~\Pr[\Val \ne \bot :\Val \gets \mcal{K}_i(\tau)] \ge p_\tau - \negl(\secpar)$.
\end{MyClaim}
\begin{proof}
This claim follows immediately from \Cref{claim:bound:G''i} and the witness-extended emulation property (as per \Cref{def:WEE}) of the right {\bf WIPoK-2}.
\end{proof}

Finally, we are ready to define the extractor $\mcal{K}$. Intuitively, it can be considered as an average-case version of $\Set{\mcal{K}_i}_{i\in[\tilde{t}]}$:

\para{Extractor $\mcal{K}$:\label{extractorK:description}} (Illustrated in \Cref{figure:one-sided:K}.)  one any input $\tau$, $\mcal{K}(\tau)$ samples uniformly at random an $i \pick [\tilde{t}]$, executes $\mcal{K}_i(\tau)$, and outputs whatever $\mcal{K}_i(\tau)$ outputs.

\para{Proving \Cref{item:extractorK:efficiency} in \Cref{lem:extractorK}.} Recall that we need to show that $\mcal{K}$ satisfies the two properties listed in \Cref{lem:extractorK}. First, observe that \Cref{item:extractorK:efficiency} follows simply from the description of $\mcal{K}$---Indeed, each $\mcal{K}_i(\tau)$ is the same as the real man-in-the-middle execution conditioned on the prefix $\tau$, except that $\tilde{x}_i$ is used in the right {\bf WIPoK-1} and the witness-extended emulator $\SimExt$ is used in the right {\bf WIPoK-2} and the left {\bf WIPoK-1}. Since  $\SimExt$ runs in expected PPT, so does $\mcal{K}_i(\tau)$. Therefore, $\mcal{K}(\tau)$ also runs in expected PPT.


\para{Proving \Cref{item:extractorK:extractability} in \Cref{lem:extractorK}.} Now, the only thing left is to prove \Cref{item:extractorK:extractability}.
Recall that \Cref{item:extractorK:extractability} requires that 
for any $\tau$, if $p_\tau \ge \epsilon(\secpar)$, then it holds that
\begin{equation}\label[Inequality]{eq:bound:averageK}
\Pr[\Val = \tilde{m}(\tau) :\Val \gets \mcal{K}(\tau)] \ge \epsilon'(\secpar)/\tilde{t}.
\end{equation}
Also recall that $\mcal{K}(\tau)$ is defined to execute the machine $\mcal{K}_i(\tau)$  with  $i$ uniformly sampled from $[\tilde{t}]$. Therefore, \Cref{eq:bound:averageK} can be reduced to the following \Cref{lem:bound:Ki}. We will prove \Cref{lem:bound:Ki} in \Cref{sec:lem:bound:Ki:proof}, which will eventually finish the current proof of \Cref{lem:extractorK}.
\begin{lemma}\label{lem:bound:Ki}
Let $\epsilon(\secpar) = \frac{1}{\poly(\secpar)}$ and $\epsilon'(\secpar) = \frac{\epsilon(\secpar)}{t^2}$.
For any $\tau$, if $p_\tau \ge \epsilon(\secpar)$, then there exists an $i \in [\tilde{t}]$ such that 
$$\Pr[\Val = \tilde{m}(\tau) :\Val \gets \mcal{K}_i(\tau)] \ge \epsilon'(\secpar).$$
\end{lemma}
% \begin{lemma}\label{lem:bound:averageK}
% for any $\tau$, if $p_\tau \ge \epsilon(\secpar)$, then it holds that
% $$\Pr[\Val = \tilde{m}(\tau) :\Val \gets \mcal{K}(\tau)] \ge \epsilon'(\secpar)/\tilde{t}.$$
% \xiao{Need to define $\tilde{m}(\tau)$; also need to specify $\epsilon'$ (w.r.t.\ $\epsilon$)..}
% \end{lemma}
% \xiao{Say that we postpone the proof of \Cref{lem:bound:averageK} to \Cref{sec:proof:lem:bound:averageK}}

% \xiao{Assume \Cref{lem:bound:averageK} is true, finish the proof of non-malleability.}


% To prove \Cref{lem:bound:averageK}, it suffices to show that if $\tau$ satisfying $p_\tau \ge \epsilon(\secpar)$, then there exists an $i \in [\tilde{t}]$ such that $\Pr[\Val = \tilde{m}(\tau) :\Val \gets \mcal{K}_i(\tau)] \ge \epsilon'(\secpar)$.

\subsection{Proof of \Cref{lem:bound:Ki}}
\label{sec:lem:bound:Ki:proof}
We assume for contradiction that for some $\tau$ satisfying $p_\tau \ge \epsilon(\secpar)$, it holds that 
\begin{equation}\label[Inequality]{eq:proof:averageK:contra-assump}
\forall i \in [\tilde{t}], ~\Pr[\Val = \tilde{m}(\tau) :\Val \gets \mcal{K}_i(\tau)] < \epsilon'(\secpar).
\end{equation}

\begin{MyClaim}\label{cliam:bound:Ki-xi}
%For any $\tau$, if $p_\tau \ge \epsilon(\secpar)$, then it holds that
Under the assumption in \Cref{eq:proof:averageK:contra-assump}, it holds that 
$$\forall i \in [\tilde{t}], ~\Pr[\Val = \tilde{x}_i:\Val \gets \mcal{K}_i(\tau)] \ge p_\tau - \epsilon'(\secpar) - \negl(\secpar).$$
\end{MyClaim}
\begin{proof}
First, recall that the event $\Val \ne \bot$ (i.e., $\Val$ is a valid witness) can be partitioned into the following {\em disjoint} events: $\Val = \tilde{m}(\tau)$, $\Val = \tilde{x}_1$, \ldots, $\Val = \tilde{x}_{\tilde{t}}$. Therefore, we have 
\begin{equation}\label{eq:bound:Ki-xi:1}
\forall i \in [\tilde{t}], ~\Pr[\Val \ne \bot] = \Pr[\Val = \tilde{m}(\tau)] + \Pr[\Val = \tilde{x}_i] + \sum_{j \in [\tilde{t}]\setminus \Set{i}} \Pr[\Val = \tilde{x}_j],
\end{equation}
where all the probabilities are taken over the random procedure $\Val \gets \mcal{K}_i(\tau)$.

% Combining \Cref{claim:bound:Ki}, our assumption of \Cref{eq:proof:averageK:contra-assump}, and \Cref{eq:bound:Ki-xi:1}, we have the following inequality 
% $$\forall i \in [\tilde{t}], ~\Pr[\Val \red{\ne \bot}:\Val \gets \mcal{K}_i(\tau)] \ge p_\tau - \epsilon'(\secpar) - \sum_{j \in [\tilde{t}]\setminus \Set{i}} \Pr[\Val = \tilde{x}_j:\Val \gets \mcal{K}_i(\tau)].$$

Then, the following holds
(all the probabilities below are taken w.r.t.\ the random procedure $\Val \gets \mcal{K}_i(\tau)$):
\begin{align}
\forall i \in [\tilde{t}], ~\Pr[\Val = \tilde{x}_i] 
& = 
\Pr[\Val \ne \bot] - \Pr[\Val = \tilde{m}(\tau)] -  \bigg(\sum_{j \in [\tilde{t}]\setminus \Set{i}} \Pr[\Val = \tilde{x}_j] \bigg)  \label{eq:bound:Ki-xi:derive:1} \\
& \ge p_\tau - \negl(\secpar) - \Pr[\Val = \tilde{m}(\tau)] -  \bigg(\sum_{j \in [\tilde{t}]\setminus \Set{i}} \Pr[\Val = \tilde{x}_j] \bigg)  \label[Inequality]{eq:bound:Ki-xi:derive:2}\\
& \ge p_\tau - \negl(\secpar) - \epsilon'(\secpar) -  \bigg(\sum_{j \in [\tilde{t}]\setminus \Set{i}} \Pr[\Val = \tilde{x}_j] \bigg) \label[Inequality]{eq:bound:Ki-xi:derive:3}
\end{align}
where \Cref{eq:bound:Ki-xi:derive:1} follows from \Cref{eq:bound:Ki-xi:1}, \Cref{eq:bound:Ki-xi:derive:2} follows from \Cref{claim:bound:Ki}, and \Cref{eq:bound:Ki-xi:derive:3} follows from \Cref{eq:proof:averageK:contra-assump}.


Now, to prove \Cref{cliam:bound:Ki-xi}, it suffices to show that 
\begin{equation}
\forall i \in [\tilde{t}],~\forall j \in [\tilde{t}]\setminus \Set{i}, ~\Pr[\Val = \tilde{x}_j:\Val \gets \mcal{K}_i(\tau)] = \negl(\secpar).
\end{equation}
This can be reduced via standard techniques to the one-wayness of the OWF $\tilde{f}$ in \Cref{item:one-sided:step:OWFs} of the right execution. In more details, we assume for contradiction that there exit $i^*, j^* \in [\tilde{t}]$ such that $i^* \ne j^*$ and that the probability $\Pr[\Val = \tilde{x}_{j^*}: \Val \gets \mcal{K}_{i^*}(\tau)]$ is non-negligible, where, by definition, $\tilde{x}_{j^*}$ is the preimage of $\tilde{y}_{j^*}$ under the right OWF $\tilde{f}$. Then, we can build an adversary $\Adv_\textsc{owf}$ breaking one-wayness in the following way: $\Adv_\textsc{owf}$ obtains the challenge $y^*$ from the external one-wayness challenger; it then runs the machine $\mcal{K}_{i^*}(\tau)$ internally, for which $\Adv_\textsc{owf}$ uses $y^*$ in place of $\tilde{y}_{j^*}$ when executing \Cref{item:one-sided:step:OWFs} in the right. Note that the internal execution $\mcal{K}_{i^*}(\tau)$ is identically to the stand-alone execution of $\mcal{K}_{i^*}$, thus the extracted $\tilde{x}_{j^*}$ will be a valid preimage for $y^*$ ($= \tilde{y}_j^*$) with non-negligible probability, breaking one-wayness. 
\end{proof}


\para{Machine $\mcal{K}'_i$ ($i \in [\tilde{t}]$):\label{machineK':description}} (Illustrated in \Cref{figure:one-sided:K'i}.) On an input $\tau$ that corresponds to the first 2 steps of the man-in-the-middle execution, $\mcal{K}'_i(\tau)$ proceeds as follows:
\begin{enumerate}
\item
$\mcal{K}'_i(\tau)$ first finish \Cref{item:one-sided:step:OWFs} of the man-in-the-middle execution in the same way as $\mcal{K}_i(\tau)$. In particular, it will see in the left execution the values $Y = (y_1, \ldots, y_t)$ sent from $\mcal{M}$; 
\item
$\mcal{K}'_i(\tau)$ recovers $(x_1, \ldots, x_t)$ by brute-force: Namely, for each $y_i$, it inverts the OWF $f$ to find $x_i$ s.t.\ $f(x_i) = y_i$. It is possible that there exist some ``bad'' $y_i$'s that are not in the range of $f$. For such bad $i$'s, it sets $x_i = \bot$. If all the $x_i$'s are bad, $\mcal{K}'_i(\tau)$ halts and outputs $\bot$;
\item \label[Step]{item:machineK':3}
If this step is reached, we know that $(x_1, \ldots, x_t)$ cannot be all $\bot$. $\mcal{K}'_i(\tau)$ then picks a $x^*_j$ uniformly at random from the good (i.e.\ non-$\bot$) $x_i$'s.
\item
$\mcal{K}'_i(\tau)$ continues to finish the execution in the same way as $\mcal{K}_i(\tau)$, except that it uses $x^*_j$ as the witness when executing the left {\bf WIPoK-2}. 
\end{enumerate}
It is worth noting that the $(j, x_j)$ extracted (in $\mcal{K}_i(\tau)$, inherited from $\mcal{G}'_i(\tau)$) by the witness-extended emulator for the left {\bf WIPoK-1} is not used any more by $\mcal{K}'_i(\tau)$. 

It is easy to see that if the $x^*_j$ picked by $\mcal{K}'_i(\tau)$ is the equal to the $x_j$ extracted by $\mcal{K}_i(\tau)$ from its left {\bf WIPoK-1}, then $\mcal{K}'_i(\tau)$ and $\mcal{K}_i(\tau)$ are identical\footnote{In this step, we rely on the injectiveness of the OWF $f$ in the right. That is, there is a unique preimage for each image. Thus, if both the $x^*_j$ (sampled by $\mcal{K}'_i(\tau)$) and the extracted $x_j$ (in $\mcal{K}_i(\tau)$) are a valid preimage for the same $y_j$, then $x^*_j$ must equal $x_j$.}. Since $\mcal{K}'_i(\tau)$ samples $x^*_j$ uniformly, then $x^*_j = x_j$ with probability at least $1/t$. Therefore, the following must holds: 
\begin{equation}\label[Inequality]{eq:bound:K'i}
\forall i \in [\tilde{t}], ~\Pr[\Val = \tilde{x}_i:\Val \gets \mcal{K}'_i(\tau)] \ge \frac{1}{t}\cdot \Pr[\Val = \tilde{x}_i:\Val \gets \mcal{K}_i(\tau)].
\end{equation}

\begin{figure}[!tb]
     \begin{subfigure}[t]{0.47\textwidth}
         \centering
         \fbox{
         \includegraphics[width=\textwidth]{figures/figure07.pdf}
         }
         \caption{}
         \label{figure:one-sided:K'i}
     \end{subfigure}
     \hspace{6.5pt}
     \begin{subfigure}[t]{0.47\textwidth}
         \centering
         \fbox{
         \includegraphics[width=\textwidth]{figures/figure08.pdf}
         }
         \caption{}
         \label{figure:one-sided:K''i}
     \end{subfigure}
     \caption{Machines $\mcal{K}'_i(\tau)$ and $\mcal{K}''_i(\tau)$ \scriptsize{(Changes between adjacent machines are highlighted by red color)}}
     \label{figure:one-sided:K'i-K''i}
\end{figure}

\para{Machine $\mcal{K}''_i$ ($i\in [\tilde{t}]$):} (Illustrated in \Cref{figure:one-sided:K''i}.) On any input $\tau$,  $\mcal{K}''_i(\tau)$ behaves identically to $\mcal{K}'_i(\tau)$ except that it plays as the honest committer in the left {\bf WIPoK-1}, instead of running the witness-extended emulator. Recall that starting from $\mcal{K}'_i$, the witness $(j, x_j)$ extracted by the witness-extended emulator for the left {\bf WIPoK-1} is not used any more. Thus, machine $\mcal{K}''_i$ does not need to perform this witness-extended emulation.

By the witness-extended emulation property (as per \Cref{def:WEE}) of the left {\bf WIPoK-1}, it is easy to see that 
\begin{equation}\label[Inequality]{eq:relation:K'-K''}
\forall i \in [\tilde{t}], ~\Pr[\Val = \tilde{x}_i:\Val \gets \mcal{K}''_i(\tau)] \ge \Pr[\Val = \tilde{x}_i:\Val \gets \mcal{K}'_i(\tau)] -\negl(\secpar).
\end{equation}
Moreover, by the WI property of the right {\bf WIPoK-1}, the following must hold
\begin{equation}\label[Inequality]{eq:relation:K:WI}
\forall i \in [\tilde{t}], ~\big|\Pr[\Val = \tilde{x}_i:\Val \gets \mcal{K}''_i(\tau)] - \Pr[\Val = \tilde{x}_i:\Val \gets \mcal{K}''_1(\tau)]\big|  \le \negl(\secpar).
\end{equation}

\begin{MyClaim}\label{claim:bound:K''1}
% For any $\tau$, if $p_\tau \ge \epsilon(\secpar)$, then it holds that
$\forall i \in [\tilde{t}], ~\Pr[\Val = \tilde{x}_i:\Val \gets \mcal{K}''_1(\tau)] \ge \frac{1}{t} \cdot \big(p_\tau - \epsilon'(\secpar)\big) - \negl(\secpar)$.
\end{MyClaim}
\begin{proof} 
This claim following from \Cref{cliam:bound:Ki-xi} and \Cref{eq:bound:K'i,eq:relation:K'-K'',eq:relation:K:WI}. Formally,
\begin{align}
\forall i \in [\tilde{t}], ~\Pr[\Val = \tilde{x}_i:\Val \gets \mcal{K}''_1(\tau)] 
 & \ge \Pr[\Val = \tilde{x}_i:\Val \gets \mcal{K}''_i(\tau)]  - \negl(\secpar)
\label[Inequality]{claim:bound:K''1:proof:1}\\
 & \ge 
\Pr[\Val = \tilde{x}_i:\Val \gets \mcal{K}'_i(\tau)]  - \negl(\secpar) 
\label[Inequality]{claim:bound:K''1:proof:2}\\
 & \ge 
\frac{1}{t}\cdot\Pr[\Val = \tilde{x}_i:\Val \gets \mcal{K}_i(\tau)]  - \negl(\secpar) 
\label[Inequality]{claim:bound:K''1:proof:3}\\
& \ge 
\frac{1}{t} \cdot \big(p_\tau - \epsilon'(\secpar)\big) - \negl(\secpar), \label[Inequality]{claim:bound:K''1:proof:4}
\end{align}
where \Cref{claim:bound:K''1:proof:1} follows from \Cref{eq:relation:K:WI}, \Cref{claim:bound:K''1:proof:2} follows from \Cref{eq:relation:K'-K''}, \Cref{claim:bound:K''1:proof:3} follows from \Cref{eq:bound:K'i}, and \Cref{claim:bound:K''1:proof:4} follows from \Cref{cliam:bound:Ki-xi}.
\end{proof}

Now, we show the last claim which, together with \Cref{claim:bound:K''1}, will lead to the desired contradiction.
\begin{MyClaim}\label{claim:K'':non-abort}
%For any $\tau$, if $p_\tau \ge \epsilon(\secpar)$, then it holds that
$\Pr[\Val \ne \bot:\Val \gets \mcal{K}''_1(\tau)] \le p_\tau + \negl(\secpar)$.
\end{MyClaim}

\para{Deriving the contradiction.} Before proving \Cref{claim:K'':non-abort}, we first show why \Cref{claim:bound:K''1,claim:K'':non-abort} are contradicting. In the following, all the probabilities are taken over the random procedure $\Val \gets \mcal{K}''_1(\tau)$:
\begin{align*}
\Pr[\Val \ne \bot] 
& = \Pr[\Val = \tilde{m}(\tau) ~\vee~ \Val = \tilde{x}_1 ~\vee~ \ldots ~\vee~ \Val = \tilde{x}_{\tilde{t}}] \\
& \ge \Pr[\Val = \tilde{x}_1 ~\vee~ \ldots ~\vee~ \Val = \tilde{x}_{\tilde{t}}] = \sum_{i =1 }^{\tilde{t}} \Pr[\Val = \tilde{x}_i] \\
&\ge \tilde{t} \cdot \frac{1}{t} \cdot \big(p_\tau - \epsilon'(\secpar)\big) - \negl(\secpar) \numberthis \label[Inequality]{eq:bound:Ki:final-contradiction:1}\\
& \ge (1+\frac{1}{t}) \cdot (p_\tau - \epsilon'(\secpar)) - \negl(\secpar) \numberthis \label[Inequality]{eq:bound:Ki:final-contradiction:2}\\
& = p_\tau + \bigg(\frac{p_\tau}{t} - \epsilon'(\secpar) - \frac{\epsilon'(\secpar)}{t}\bigg) - \negl(\secpar)\\
& \ge p_\tau + \frac{t^2 - t -1}{t^3}\cdot \epsilon(\secpar) - \negl(\secpar) \numberthis \label[Inequality]{eq:bound:Ki:final-contradiction:3}\\
\end{align*}
where \Cref{eq:bound:Ki:final-contradiction:1} follows from \Cref{claim:bound:K''1}, \Cref{eq:bound:Ki:final-contradiction:2} follows from the assumption that $\tilde{t} \ge t+1$, and \Cref{eq:bound:Ki:final-contradiction:3} follows from the assumption that $p_\tau \ge \epsilon(\secpar)$ and our parameter setting $\epsilon'(\secpar) = \frac{\epsilon(\secpar)}{t^2}$.

Recall that $t$ is the tag taking value from $[2n]$ where $n$ is a polynomial of $\secpar$. Also recall that $\epsilon(\secpar)$ is an inverse polynomial on $\secpar$. Therefore, \Cref{eq:bound:Ki:final-contradiction:2} can be written as:
$$\Pr[\Val \ne \bot:\Val \gets \mcal{K}''_1(\tau)] \ge p_\tau + \frac{1}{\poly(\secpar)} - \negl(\secpar),$$
which contradicts \Cref{claim:K'':non-abort}.

This eventually finishes the proof of \Cref{lem:bound:Ki} (modulo the proof of \Cref{claim:K'':non-abort} which we will show next).



\begin{proof}[Proof of {\Cref{claim:K'':non-abort}}]
We first define two extra machines $\mcal{K}^{**}_1$ and $\mcal{K}^*_1$. 

\para{Machine $\mcal{K}^{**}_1$:} (Illustrated in \Cref{figure:one-sided:K**i}.) On any input $\tau$, $\mcal{K}^{**}_1(\tau)$ behaves identically as $\mcal{K}''_1(\tau)$ except that $\mcal{K}^{**}_1(\tau)$ finishes the right {\bf WIPoK-2} using the honest receiver's algorithm, instead of using the witness-extended emulator. $\mcal{K}^{**}_1(\tau)$ simply outputs the view of $\mcal{M}$ during the execution. By the witness-extended emulation property (as per \Cref{def:WEE}), it holds that
\begin{equation}\label{eq:K''1-K**1}
\Pr[\Val \ne \bot :\Val\gets \mcal{K}''_1(\tau)] = \Pr[\View~\text{is accepting}:\View\gets \mcal{K}^{**}_1(\tau)] \pm \negl(\secpar).
\end{equation}


\para{Machine $\mcal{K}^{*}_1$:} (Illustrated in \Cref{figure:one-sided:K*i}.) On any input $\tau$, $\mcal{K}^{*}_1(\tau)$ behaves identically as $\mcal{K}^{**}_1(\tau)$ except for the witness used in the left {\bf WIPoK-2}: $\mcal{K}^{*}_1(\tau)$ use the $(m, r)$ used to generated $\com = \Com_\rho(m;r)$ as the witness to finish the left {\bf WIPoK-2}. (Note that this witness pair $(m,r)$ must be contained in $\tau$---because $\tau$ is corresponding to the first steps of the man-in-the-middle execution, and the left execution is done by the honest committer.) It is worth noting that machine $\mcal{K}^*_1$ is actually identical to the machine $\mcal{G}_1$ we defined on \Cpageref{machine:Gi}. Therefore, it follows immediately that
\begin{equation}\label{eq:K*1-G1}
\Pr[\View~\text{is accepting}:\View\gets \mcal{K}^{*}_1(\tau)] = \Pr[\View~\text{is accepting}:\View\gets \mcal{G}_1(\tau)] = p_\tau, 
\end{equation}
where the last equivalence follows by definition (see \Cref{def:p-tau:2}).

\begin{figure}[!tb]
     \begin{subfigure}[t]{0.47\textwidth}
         \centering
         \fbox{
         \includegraphics[width=\textwidth]{figures/figure09.pdf}
         }
         \caption{}
         \label{figure:one-sided:K**i}
     \end{subfigure}
     \hspace{6.5pt}
     \begin{subfigure}[t]{0.47\textwidth}
         \centering
         \fbox{
         \includegraphics[width=\textwidth]{figures/figure10.pdf}
         }
         \caption{}
         \label{figure:one-sided:K*i}
     \end{subfigure}
     \caption{Machines $\mcal{K}^{**}_1(\tau)$ and $\mcal{K}^*_1(\tau)$ \scriptsize{(Changes between adjacent machines are highlighted by red color)}}
     \label{figure:one-sided:K**1-K*1}
\end{figure}

Next, let us recall the witness used by $\mcal{K}^{**}_1$ for the left {\bf WIPoK-2}. By definition, machine $\mcal{K}^{**}_1(\tau)$ performs brute-force to extract $(x_1, \ldots, x_t)$ from $\tau$,\footnote{This brute-forcing was there starting from $\mcal{K}'_1$ (defined on \Cpageref{machineK':description}), and was inherited by $\mcal{K}''_1$, $\mcal{K}^{**}_1$, and eventually by $\mcal{K}^{*}_1$.} and samples a random {\em good}\footnote{Recall from \Cref{item:machineK':3}
 of $\mcal{K}'_i(\tau)$ (\Cpageref{machineK':description}) that ``good'' means that $x^*_j$ is a valid pre-image of $y_j$.} $x^*_j$ as the witness to go through the left {\bf WIPoK-2}. In summary, the only difference between $\mcal{K}^{*}_1$ and $\mcal{K}^{**}_1$ is the witness used in the left {\bf WIPoK-2}. Also, note that neither $\mcal{K}^{*}_1$ nor $\mcal{K}^{**}_1$ rewinds the {\bf WIPoK-2} because we already get rid of the witness-extended emulation starting from $\mcal{K}^{**}_1$. Therefore, 
by the WI property of the left {\bf WIPoK-2}, it holds that
\begin{equation}\label{eq:K**1-K*1}
\Pr[\View~\text{is accepting}:\View\gets \mcal{K}^{**}_1(\tau)] = \Pr[\View~\text{is accepting}:\View\gets \mcal{K}^{*}_1(\tau)] \pm \negl(\secpar).
\end{equation}
Combining \Cref{eq:K''1-K**1,eq:K*1-G1,eq:K**1-K*1}, we have
$$\Pr[\Val \ne \bot :\Val\gets \mcal{K}''_1(\tau)] = p_\tau \pm \negl(\secpar).$$
This in particular implies \Cref{claim:K'':non-abort}.
\end{proof}

==> sections/tag-amp.tex <==
%!TEX root = ../main.tex
\section{Tag Amplification}

\takashi{I moved BLS theorem to the post-quantum section. I believe you will not use that in the classical case.}

\takashi{It may be fine to omit the details of the tag-amplification in the classical case given that the post-quantum case is the main result.}

